Real-time optimal quantum control for atomic magnetometers with decoherence

Quantum entanglement, in the form of spin squeezing, is known to improve the sensitivity of atomic sensors to static or slowly varying fields. Sensing transient events presents a distinct challenge, requires different analysis tools, and has not been shown to benefit from entanglement in practically important scenarios such as spin-precession magnetometry. To address this, we apply concepts from continuous quantum measurements and estimation theory to optical atomic magnetometers, aiming to accurately model these devices, interpret their measurement data, control their dynamics, and achieve optimal sensitivity. Quantifying this optimal performance requires determining a fundamental quantum limit on sensitivity. We derive this limit, imposed by noise, and show that it scales at best linearly with sensing time and atom number N, ruling out any super-classical scaling. This limit is independent of the initial state, measurement, estimator, and measurement-based feedback, and depends only on the decoherence model and the strength of field fluctuations. Thus, finding an estimator that attains this bound proves the sensing strategy optimal. To approach this limit, we develop a quantum dynamical model scalable with N, based on a co-moving Gaussian approximation of the stochastic master equation, which includes measurement backaction and decoherence. This enables a real-time estimation and control architecture integrating an extended Kalman filter with a linear quadratic regulator. Simulating the magnetometer with our model and EKF+LQR strategy shows that quantum-limited tracking of constant and fluctuating fields is within reach of current atomic magnetometers. Our sensing strategy can also track biologically relevant signals, such as heartbeat-like waveforms, and drive the atomic ensemble into an entangled state, even when the measurement record is used for feedback but later discarded.

==> tikzlibrary3dtools.code.tex <==
% Copyright 2021 by an anonymous marmot
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.
\ProvidesFileRCS{tikzlibrary3dtools.code.tex}
\usetikzlibrary{3d,decorations,fpu}% to do: ability to switch on and off
\usepackage{calculator}% maybe drop
\makeatletter%
\ifnum\month>10\relax
\typeout{Hibernation season has just started.}%
\fi
\ifnum\month<5\relax
\typeout{Hibernation season has not yet ended.}%
\fi
\ifnum\month=2\relax
\ifnum\day=2
\typeout{Yay! Groundhog Day!}%
\fi
\fi
\def\tikz@td@extractpgfversionaux#1.#2.#3|#4#5#6;{\def#4{#1}\def#5{#2}\def#6{#3}}%
\def\tikz@td@checkversion{%
\edef\pgfutil@tmp{\noexpand\tikz@td@extractpgfversionaux\pgfversion|\noexpand\pgfutil@tmpa\noexpand\pgfutil@tmpb\noexpand\pgfutil@tmpc;}%
\pgfutil@tmp%\typeout{a=\pgfutil@tmpa,b=\pgfutil@tmpb,c=\pgfutil@tmpc}%
\pgfmathtruncatemacro{\pgfutil@tmpe}{ifthenelse(10*\pgfutil@tmpa+\pgfutil@tmpb<31,0,1)}%
\ifnum\pgfutil@tmpe=0%
\message{You are using a too old version of pgf (\pgfversion). You need at least
version 3.1.1 to use the features of this library.}%
\fi
\edef\pgfutil@tmpd{\expandafter\@firstoftwo\pgfutil@tmpc\empty}%
\pgfmathtruncatemacro{\pgfutil@tmpe}{ifthenelse(100*\pgfutil@tmpa+10*\pgfutil@tmpb+\pgfutil@tmpc<313,0,1)}%
\ifnum\pgfutil@tmpe=0%
\message{Some routines of 3dtools may not work because they rely on the pushing
and popping techniques that were added in version 3.1.3 (but the current version
is \pgfversion).^^J}%
\fi
\pgfmathtruncatemacro{\pgfutil@tmpe}{ifthenelse(100*\pgfutil@tmpa+10*\pgfutil@tmpb+\pgfutil@tmpc<316,0,1)}%
\ifnum\pgfutil@tmpe=0%
\def\pgfutil@pushmacro##1{%
    \xdef\pgfutil@pushmacro@string{\string##1}%
    \ifcsname pgfutil@pushedmacro@\pgfutil@pushmacro@string\endcsname\else
        % \newcount is \outer in Plain
        \csname newcount\expandafter\endcsname\csname pgfutil@pushedmacro@\pgfutil@pushmacro@string\endcsname
    \fi
    \global\advance\csname pgfutil@pushedmacro@\pgfutil@pushmacro@string\endcsname 1\relax
    \global\expandafter\let\csname\the\csname pgfutil@pushedmacro@\pgfutil@pushmacro@string\endcsname\pgfutil@pushmacro@string\endcsname##1%
}
\message{pgfutil@pushmacro fixed because current pgf version \pgfversion\space is smaller than 3.1.6.^^J}%
\fi
}%

\newcommand{\orthmat}[3]{% the entries of this matrix keep track
\pgfmathparse{cos(#1)*cos(#2)}% of the current transformation
\xdef\tikz@td@matAA{\pgfmathresult}%
\pgfmathparse{sin(#1)*cos(#2)}% 
\xdef\tikz@td@matAB{\pgfmathresult}% 
\pgfmathparse{-sin(#2)}% 
\xdef\tikz@td@matAC{\pgfmathresult}%
\pgfmathparse{cos(#1)*sin(#2)*sin(#3)-sin(#1)*cos(#3)}%
\xdef\tikz@td@matBA{\pgfmathresult}%  
\pgfmathparse{sin(#1)*sin(#2)*sin(#3)+cos(#1)*cos(#3)}% 
\xdef\tikz@td@matBB{\pgfmathresult}%
\pgfmathparse{cos(#2)*sin(#3)}%
\xdef\tikz@td@matBC{\pgfmathresult}%
\pgfmathparse{cos(#1)*sin(#2)*cos(#3)+sin(#1)*sin(#3) }%
\xdef\tikz@td@matCA{\pgfmathresult}% 
\pgfmathparse{sin(#1)*sin(#2)*cos(#3)-cos(#1)*sin(#3)}% 
\xdef\tikz@td@matCB{\pgfmathresult}%
\pgfmathparse{cos(#2)*cos(#3)}%
\xdef\tikz@td@matCC{\pgfmathresult}}%
\tikzset{3d/.cd,phi/.initial=0,psi/.initial=0,theta/.initial=0,
install view/.style={/utils/exec=\tikzset{3d/.cd,#1}%
\orthmat{\pgfkeysvalueof{/tikz/3d/phi}}{%
\pgfkeysvalueof{/tikz/3d/psi}}{\pgfkeysvalueof{/tikz/3d/theta}},%
/tikz/x={({\tikz@td@matAA*1cm},{\tikz@td@matBA*1cm})},%
/tikz/y={({\tikz@td@matAB*1cm},{\tikz@td@matBB*1cm})},%
/tikz/z={({\tikz@td@matAC*1cm},{\tikz@td@matBC*1cm})}}}%
\def\pgfmathparse@td@FPU#1{\begingroup%
\pgfkeys{/pgf/fpu,/pgf/fpu/output format=fixed}%
\pgfmathparse{#1}%
\pgfmathsmuggle\pgfmathresult\endgroup}%
\def\pgfmathsetmacro@td@FPU#1#2{\begingroup%
\pgfkeys{/pgf/fpu,/pgf/fpu/output format=fixed}%
\pgfmathsetmacro#1{#2}%
\pgfmathsmuggle#1\endgroup}%
%
\xdef\tikz@td@type{0}%0=linear combination,1=vector product
\long\def\tikz@td@raw@coord(#1){\csname tikz@dcl@coord@#1\endcsname}% 
\long\def\tikz@td@makesenseof@coord#1{%
\expanded{\noexpand\pgfutil@in@{(}{#1}}% 
\ifpgfutil@in@% 
\tikz@td@parse@coord#1%
\else
\tikz@td@parse@coord(#1)%
\fi
}%
\long\def\tikz@td@parse@coord(#1){%
\pgfutil@tempcnta=0%
\pgfutil@for\pgf@tmp:={#1}\do{\advance\pgfutil@tempcnta by1}%
\ifnum\pgfutil@tempcnta=1\relax
\edef\pgfutil@tmp{\csname tikz@dcl@coord@#1\endcsname}% 
\fi
\ifcase\pgfutil@tempcnta
\or
\edef\pgfutil@tmp{\csname tikz@dcl@coord@#1\endcsname}% 
\or
\edef\pgfutil@tmp{#1,0}%
\or
\edef\pgfutil@tmp{#1}%
\fi%
\pgfmathparse@td@FPU{xcomp3(\pgfutil@tmp)}% 
\edef\pgf@X{\pgfmathresult pt}% 
\pgfmathparse@td@FPU{ycomp3(\pgfutil@tmp)}% 
\edef\pgf@Y{\pgfmathresult pt}% 
\pgfmathparse@td@FPU{zcomp3(\pgfutil@tmp)}% 
\edef\pgf@Z{\pgfmathresult pt}}%
\pgfmathdeclarefunction{TD}{1}{%
\begingroup%
\pgfmathtdparse{#1}%
\pgfmathsmuggle\pgfmathresult\endgroup%
}%
% projections 
\pgfmathdeclarefunction{xcomp3}{3}{% x component of a 3-vector 
\begingroup% 
\pgfmathparse@td@FPU{#1}% 
\pgfmathsmuggle\pgfmathresult\endgroup} 
\pgfmathdeclarefunction{ycomp3}{3}{% y component of a 3-vector 
\begingroup% 
\pgfmathparse@td@FPU{#2}% 
\pgfmathsmuggle\pgfmathresult\endgroup} 
\pgfmathdeclarefunction{zcomp3}{3}{% z component of a 3-vector 
\begingroup% 
\pgfmathparse@td@FPU{#3}% 
\pgfmathsmuggle\pgfmathresult\endgroup} 
\pgfmathdeclarefunction{TDx}{1}{% x component of a 3-vector 
\begingroup% 
\edef\mycoord{\tikz@td@raw@coord(#1)}%
\pgfmathparse@td@FPU{xcomp3\mycoord}% 
\pgfmathsmuggle\pgfmathresult\endgroup}%
\pgfmathdeclarefunction{TDy}{1}{% x component of a 3-vector 
\begingroup% 
\edef\mycoord{\tikz@td@raw@coord(#1)}%
\pgfmathparse@td@FPU{ycomp3\mycoord}% 
\pgfmathsmuggle\pgfmathresult\endgroup}%
\pgfmathdeclarefunction{TDz}{1}{% x component of a 3-vector 
\begingroup% 
\edef\mycoord{\tikz@td@raw@coord(#1)}%
\pgfmathparse@td@FPU{zcomp3\mycoord}% 
\pgfmathsmuggle\pgfmathresult\endgroup}%
\pgfmathdeclarefunction{TDunit}{1}{%normalized vector
\begingroup% 
\pgfmathsetmacro{\pgfutil@tmpv}{TD("#1")}%
\pgfmathsetmacro@td@FPU{\pgfutil@tmpn}{min(1,sqrt(TD("(\pgfutil@tmpv)o(\pgfutil@tmpv)")))}% changed May 23 2023
\ifdim\pgfutil@tmpn pt<0.002pt\relax
\PackageWarning{3dtools}{Vector too short, cannot normalize it.}%
\let\pgfmathresult\pgfutil@tmpv%
\else
\pgfmathsetmacro@td@FPU{\pgfutil@tmpn}{1/sqrt(TD("(\pgfutil@tmpv)o(\pgfutil@tmpv)"))}% % changed May 23 2023
\pgfmathparse{TD("\pgfutil@tmpn*(\pgfutil@tmpv)")}%
\fi
\pgfmathsmuggle\pgfmathresult\endgroup}%
% \pgfmathdeclarefunction{TDX}{1}{% x component of a 3-vector 
% \begingroup% 
% \edef\pgfmathresult{0}%
% % \typeout{#1}
% % \edef\temp{\noexpand\pgfmathparse@td@FPU{TDx#1}}%
% % \temp
% \typeout{\pgfmathresult}%
% \pgfmathsmuggle\pgfmathresult\endgroup}%
% \pgfmathdeclarefunction{TDY}{1}{% x component of a 3-vector 
% \begingroup% 
% \edef\mycoord{\tikz@td@raw@coord#1}%
% \pgfmathparse@td@FPU{ycomp3\mycoord}% 
% \pgfmathsmuggle\pgfmathresult\endgroup}%
% \pgfmathdeclarefunction{TDZ}{1}{% x component of a 3-vector 
% \begingroup% 
% \edef\mycoord{\tikz@td@raw@coord#1}%
% \pgfmathparse@td@FPU{zcomp3\mycoord}% 
% \pgfmathsmuggle\pgfmathresult\endgroup}%
\tikzset{3d/record physical components/.code={%
\tikzset{every coordinate node/.append style={3d/store components}}},
3d/store components/.code={%
\edef\pgf@Z{\relax}%
\edef\pgfutil@tmpz{\relax}%
\expandafter\tikz@td@parse@coord\tikz@scan@point@coordinate%
\pgfmathsetmacro\pgfutil@tmpx{\the\pgf@x/1cm}%
\pgfmathsetmacro\pgfutil@tmpy{\the\pgf@y/1cm}%
\ifx\pgf@Z\pgfutil@tmpz
\pgfmathsetmacro\pgfutil@tmpz{screendepth(\pgfutil@tmpx,\pgfutil@tmpy,0)}%
\else
\pgfmathsetmacro\pgfutil@tmpz{screendepth(\pgf@X,\pgf@Y,\pgf@Z)}%
\fi
\expandafter\xdef\csname tikz@td@physical@x@\tikz@fig@name\endcsname{\pgfutil@tmpx}%
\expandafter\xdef\csname tikz@td@physical@y@\tikz@fig@name\endcsname{\pgfutil@tmpy}%
\expandafter\xdef\csname tikz@td@physical@z@\tikz@fig@name\endcsname{\pgfutil@tmpz}%
}}
\pgfmathdeclarefunction{TDphysx}{1}{%
\begingroup%
\ifcsname tikz@td@physical@x@#1\endcsname
\expandafter\edef\expandafter\pgfmathresult\expandafter{\csname tikz@td@physical@x@#1\endcsname}%
\else
\PackageWarning{3dtools}{Physical x component of #1 not stored. Setting it to 0.}%
\edef\pgfmathresult{0}%
\fi
\pgfmathsmuggle\pgfmathresult\endgroup%
}%
\pgfmathdeclarefunction{TDphysy}{1}{%
\begingroup%
\ifcsname tikz@td@physical@y@#1\endcsname
\expandafter\edef\expandafter\pgfmathresult\expandafter{\csname tikz@td@physical@y@#1\endcsname}%
\else
\PackageWarning{3dtools}{Physical y component of #1 not stored. Setting it to 0.}%
\edef\pgfmathresult{0}%
\fi
\pgfmathsmuggle\pgfmathresult\endgroup%
}%
\pgfmathdeclarefunction{TDphysz}{1}{%
\begingroup%
\ifcsname tikz@td@physical@z@#1\endcsname
\expandafter\edef\expandafter\pgfmathresult\expandafter{\csname tikz@td@physical@z@#1\endcsname}%
\else
\PackageWarning{3dtools}{Physical y component of #1 not stored. Setting it to 0.}%
\edef\pgfmathresult{0}%
\fi
\pgfmathsmuggle\pgfmathresult\endgroup%
}%
\pgfmathdeclarefunction{TDphys}{1}{%
\begingroup%
\pgfmathsetmacro{\pgfutil@tmpx}{TDphysx("#1")}%
\pgfmathsetmacro{\pgfutil@tmpy}{TDphysy("#1")}%
\pgfmathsetmacro{\pgfutil@tmpz}{TDphysz("#1")}%
\edef\pgfmathresult{\pgfutil@tmpx,\pgfutil@tmpy,\pgfutil@tmpz}%
\pgfmathsmuggle\pgfmathresult\endgroup%
}%
\tikzset{3d/.cd,local ex/.initial={localex},local ey/.initial={localey},
local ez/.initial={localez},dual ex/.initial={dualex},dual ey/.initial={dualey},
dual ez/.initial={dualez},install dual basis/.code={%
% \path (1,0,0) coordinate (\pgfkeysvalueof{/tikz/3d/local ex})
% (0,1,0) coordinate (\pgfkeysvalueof{/tikz/3d/local ey})
% (0,0,1) coordinate (\pgfkeysvalueof{/tikz/3d/local ez});
% \pgfmathsetmacro{\pgfutil@tmpxx}{x2d("\pgfkeysvalueof{/tikz/3d/local ex}")/1cm}%
% \pgfmathsetmacro{\pgfutil@tmpxy}{y2d("\pgfkeysvalueof{/tikz/3d/local ex}")/1cm}%
% \pgfmathsetmacro{\pgfutil@tmpxz}{screendepth(1,0,0)}%
% \pgfmathsetmacro{\pgfutil@tmpyx}{x2d("\pgfkeysvalueof{/tikz/3d/local ey}")/1cm}%
% \pgfmathsetmacro{\pgfutil@tmpyy}{y2d("\pgfkeysvalueof{/tikz/3d/local ey}")/1cm}%
% \pgfmathsetmacro{\pgfutil@tmpyz}{screendepth(0,1,0)}%
% \pgfmathsetmacro{\pgfutil@tmpzx}{x2d("\pgfkeysvalueof{/tikz/3d/local ez}")/1cm}%
% \pgfmathsetmacro{\pgfutil@tmpzy}{y2d("\pgfkeysvalueof{/tikz/3d/local ez}")/1cm}%
% \pgfmathsetmacro{\pgfutil@tmpzz}{screendepth(0,0,1)}%
% \typeout{((\pgfutil@tmpxx,\pgfutil@tmpxy,\pgfutil@tmpxz),(\pgfutil@tmpyx,\pgfutil@tmpyy,\pgfutil@tmpyz),(\pgfutil@tmpzx,\pgfutil@tmpzy,\pgfutil@tmpzz))}%
% % ((\the\pgf@yx/1cm)*(\the\pgf@zy/1cm)-(\the\pgf@yy/1cm)*(\the\pgf@zx/1cm))*(#1)+%
% % ((\the\pgf@zx/1cm)*(\the\pgf@xy/1cm)-(\the\pgf@xx/1cm)*(\the\pgf@zy/1cm))*(#2)+%
% % ((\the\pgf@xx/1cm)*(\the\pgf@yy/1cm)-(\the\pgf@yx/1cm)*(\the\pgf@xy/1cm))*(#3)}%
\pgfmathsetmacro{\pgfutil@tmpxx}{\pgf@xx/1cm}%
\pgfmathsetmacro{\pgfutil@tmpxy}{\pgf@xy/1cm}%
\pgfmathsetmacro{\pgfutil@tmpxz}{nscreenx}%
\pgfmathsetmacro{\pgfutil@tmpyx}{\pgf@yx/1cm}%
\pgfmathsetmacro{\pgfutil@tmpyy}{\pgf@yy/1cm}%
\pgfmathsetmacro{\pgfutil@tmpyz}{nscreeny}%
\pgfmathsetmacro{\pgfutil@tmpzx}{\pgf@zx/1cm}%
\pgfmathsetmacro{\pgfutil@tmpzy}{\pgf@zy/1cm}%
\pgfmathsetmacro{\pgfutil@tmpzz}{nscreenz}%
\path (\pgfutil@tmpxx,\pgfutil@tmpxy,\pgfutil@tmpxz) coordinate (\pgfkeysvalueof{/tikz/3d/dual ex})
	(\pgfutil@tmpyx,\pgfutil@tmpyy,\pgfutil@tmpyz) coordinate (\pgfkeysvalueof{/tikz/3d/dual ey})
	(\pgfutil@tmpzx,\pgfutil@tmpzy,\pgfutil@tmpzz) coordinate (\pgfkeysvalueof{/tikz/3d/dual ez});
\typeout{((\pgfutil@tmpxx,\pgfutil@tmpxy,\pgfutil@tmpxz),(\pgfutil@tmpyx,\pgfutil@tmpyy,\pgfutil@tmpyz),(\pgfutil@tmpzx,\pgfutil@tmpzy,\pgfutil@tmpzz))}%
}}
\pgfmathdeclarefunction{TDlocalx}{1}{%
\begingroup%
\ifcsname tikz@td@physical@x@#1\endcsname
\expandafter\edef\expandafter\pgfutil@tmpx\expandafter{\csname tikz@td@physical@x@#1\endcsname}%
\expandafter\edef\expandafter\pgfutil@tmpy\expandafter{\csname tikz@td@physical@y@#1\endcsname}%
\expandafter\edef\expandafter\pgfutil@tmpz\expandafter{\csname tikz@td@physical@z@#1\endcsname}%
\pgfmathparse@td@FPU{(\pgfutil@tmpx)*(\pgf@xx/1cm)+(\pgfutil@tmpy)*(\pgf@xy/1cm)+(\pgfutil@tmpz)*(nscreenx)}% 
\else
\PackageWarning{3dtools}{Physical x component of #1 not stored. Setting result to 0.}%
\edef\pgfmathresult{0}%
\fi
\pgfmathsmuggle\pgfmathresult\endgroup%
}%
\pgfmathdeclarefunction{TDlocaly}{1}{%
\begingroup%
\ifcsname tikz@td@physical@y@#1\endcsname
\expandafter\edef\expandafter\pgfutil@tmpx\expandafter{\csname tikz@td@physical@x@#1\endcsname}%
\expandafter\edef\expandafter\pgfutil@tmpy\expandafter{\csname tikz@td@physical@y@#1\endcsname}%
\expandafter\edef\expandafter\pgfutil@tmpz\expandafter{\csname tikz@td@physical@z@#1\endcsname}%
\pgfmathparse@td@FPU{(\pgfutil@tmpx)*(\pgf@yx/1cm)+(\pgfutil@tmpy)*(\pgf@yy/1cm)+(\pgfutil@tmpz)*(nscreeny)}% 
\else
\PackageWarning{3dtools}{Physical y component of #1 not stored. Setting result to 0.}%
\edef\pgfmathresult{0}%
\fi
\pgfmathsmuggle\pgfmathresult\endgroup%
}%
\pgfmathdeclarefunction{TDlocalz}{1}{%
\begingroup%
\ifcsname tikz@td@physical@z@#1\endcsname
\expandafter\edef\expandafter\pgfutil@tmpx\expandafter{\csname tikz@td@physical@x@#1\endcsname}%
\expandafter\edef\expandafter\pgfutil@tmpy\expandafter{\csname tikz@td@physical@y@#1\endcsname}%
\expandafter\edef\expandafter\pgfutil@tmpz\expandafter{\csname tikz@td@physical@z@#1\endcsname}%
\pgfmathparse@td@FPU{(\pgfutil@tmpx)*(\pgf@zx/1cm)+(\pgfutil@tmpy)*(\pgf@zy/1cm)+(\pgfutil@tmpz)*(nscreenz)}% 
\else
\PackageWarning{3dtools}{Physical z component of #1 not stored. Setting result to 0.}%
\edef\pgfmathresult{0}%
\fi
\pgfmathsmuggle\pgfmathresult\endgroup%
}%
\pgfmathdeclarefunction{TDlocal}{1}{%
\begingroup%
\ifcsname tikz@td@physical@z@#1\endcsname
\expandafter\edef\expandafter\pgfutil@tmpx\expandafter{\csname tikz@td@physical@x@#1\endcsname}%
\expandafter\edef\expandafter\pgfutil@tmpy\expandafter{\csname tikz@td@physical@y@#1\endcsname}%
\expandafter\edef\expandafter\pgfutil@tmpz\expandafter{\csname tikz@td@physical@z@#1\endcsname}%
\pgfmathsetmacro@td@FPU{\pgfutil@tmpa}{(\pgfutil@tmpx)*(\pgf@xx/1cm)+(\pgfutil@tmpy)*(\pgf@xy/1cm)+(\pgfutil@tmpz)*(nscreenx)}% 
\pgfmathsetmacro@td@FPU{\pgfutil@tmpb}{(\pgfutil@tmpx)*(\pgf@yx/1cm)+(\pgfutil@tmpy)*(\pgf@yy/1cm)+(\pgfutil@tmpz)*(nscreeny)}% 
\pgfmathsetmacro@td@FPU{\pgfutil@tmpc}{(\pgfutil@tmpx)*(\pgf@zx/1cm)+(\pgfutil@tmpy)*(\pgf@zy/1cm)+(\pgfutil@tmpz)*(nscreenz)}% 
\edef\pgfmathresult{\pgfutil@tmpa,\pgfutil@tmpb,\pgfutil@tmpc}%
\else
\PackageWarning{3dtools}{Physical z component of #1 not stored. Setting result to 0.}%
\edef\pgfmathresult{(0,0,0)}%
\fi
\pgfmathsmuggle\pgfmathresult\endgroup%
}%
% \def\tizk@td@scalprod#1=#2.#3;{% 
% \edef\coordA{\tikz@td@raw@coord#2}% 
% \edef\coordB{\tikz@td@raw@coord#3}% 
% \pgfmathsetmacro\pgfutil@tmpa{scalarproduct({\coordA},{\coordB})}% 
% \edef#1{\pgfutil@tmpa}}% 
\def\tizk@td@spaux#1#2#3#4#5#6{(#1)*(#4)+(#2)*(#5)+(#3)*(#6)}% 
\pgfmathdeclarefunction{scalarproduct}{2}{% scalar product of two 3-vectors 
\begingroup% 
\pgfmathparse@td@FPU{\tizk@td@spaux#1#2}% 
\pgfmathsmuggle\pgfmathresult\endgroup} 
% vector product 
% vector product auxiliary functions 
\def\vpauxx#1#2#3#4#5#6{(#2)*(#6)-(#3)*(#5)}% 
\def\vpauxy#1#2#3#4#5#6{(#4)*(#3)-(#1)*(#6)}% 
\def\vpauxz#1#2#3#4#5#6{(#1)*(#5)-(#2)*(#4)}% 
% vector product pgf functions 
\pgfmathdeclarefunction{vpx}{2}{% x component of vector product 
\begingroup% 
\pgfmathparse@td@FPU{\vpauxx#1#2}% 
\pgfmathsmuggle\pgfmathresult\endgroup} 
\pgfmathdeclarefunction{vpy}{2}{% y component of vector product 
\begingroup% 
\pgfmathparse@td@FPU{\vpauxy#1#2}% 
\pgfmathsmuggle\pgfmathresult\endgroup} 
\pgfmathdeclarefunction{vpz}{2}{% z component of vector product 
\begingroup% 
\pgfmathparse@td@FPU{\vpauxz#1#2}% 
\pgfmathsmuggle\pgfmathresult\endgroup} 
%
% axisangles, usage \pgfmathsetmacro{\myaxisangles}{axisangles("(myn)")}
\pgfmathdeclarefunction{axisangles}{1}{% 
\begingroup% 
\pgfmathsetmacro{\pgfutil@tmpa}{sqrt(TD("#1o#1"))}%
\edef\pgfutil@tmpb{\tikz@td@raw@coord#1}%
\pgfmathsetmacro{\pgftemp@x}{xcomp3(\pgfutil@tmpb)/\pgfutil@tmpa}% 
\pgfmathsetmacro{\pgftemp@y}{ycomp3(\pgfutil@tmpb)/\pgfutil@tmpa}% 
\pgfmathsetmacro{\pgftemp@z}{zcomp3(\pgfutil@tmpb)/\pgfutil@tmpa}% 
\pgfmathtruncatemacro{\itest}{ifthenelse(abs(\pgftemp@z)==1,0,1)}%
\ifnum\itest=0%
	\pgfmathtruncatemacro{\jtest}{sign(\pgftemp@x)}%
	\ifnum\jtest=1%
		\edef\pgfutil@tmpc{0,0}%
	\else
		\edef\pgfutil@tmpc{180,0}%
	\fi	
\else
    % 1 1
	\pgfmathsetmacro{\pgfutil@tmpb}{acos(\pgftemp@z)}% 
    \pgfmathsetmacro{\pgfutil@tmpa}{acos(\pgftemp@x/sin(\pgfutil@tmpb))}% 
    \pgfmathsetmacro{\ntest}{abs(cos(\pgfutil@tmpa)*sin(\pgfutil@tmpb)-\pgftemp@x)%
		+abs(sin(\pgfutil@tmpa)*sin(\pgfutil@tmpb)-\pgftemp@y)+abs(cos(\pgfutil@tmpb)-\pgftemp@z)}%
    \ifdim\ntest pt<0.1pt
      \edef\pgfutil@tmpc{\pgfutil@tmpa,\pgfutil@tmpb}%
    \fi
	% 1 -1
	\pgfmathsetmacro{\pgfutil@tmpb}{acos(\pgftemp@z)}% 
    \pgfmathsetmacro{\pgfutil@tmpa}{-acos(\pgftemp@x/sin(\pgfutil@tmpb))}% 
    \pgfmathsetmacro{\ntest}{abs(cos(\pgfutil@tmpa)*sin(\pgfutil@tmpb)-\pgftemp@x)%
		+abs(sin(\pgfutil@tmpa)*sin(\pgfutil@tmpb)-\pgftemp@y)+abs(cos(\pgfutil@tmpb)-\pgftemp@z)}%
    \ifdim\ntest pt<0.1pt
      \edef\pgfutil@tmpc{\pgfutil@tmpa,\pgfutil@tmpb}%
    \fi
	% -1 1
	\pgfmathsetmacro{\pgfutil@tmpb}{-acos(\pgftemp@z)}% 
    \pgfmathsetmacro{\pgfutil@tmpa}{acos(\pgftemp@x/sin(\pgfutil@tmpb))}% 
    \pgfmathsetmacro{\ntest}{abs(cos(\pgfutil@tmpa)*sin(\pgfutil@tmpb)-\pgftemp@x)%
		+abs(sin(\pgfutil@tmpa)*sin(\pgfutil@tmpb)-\pgftemp@y)+abs(cos(\pgfutil@tmpb)-\pgftemp@z)}%
    \ifdim\ntest pt<0.1pt
      \edef\pgfutil@tmpc{\pgfutil@tmpa,\pgfutil@tmpb}%
    \fi
	% -1 -1
	\pgfmathsetmacro{\pgfutil@tmpb}{-acos(\pgftemp@z)}%
    \pgfmathsetmacro{\pgfutil@tmpa}{-acos(\pgftemp@x/sin(\pgfutil@tmpb))}% 
    \pgfmathsetmacro{\ntest}{abs(cos(\pgfutil@tmpa)*sin(\pgfutil@tmpb)-\pgftemp@x)%
		+abs(sin(\pgfutil@tmpa)*sin(\pgfutil@tmpb)-\pgftemp@y)+abs(cos(\pgfutil@tmpb)-\pgftemp@z)}%
    \ifdim\ntest pt<0.1pt
      \edef\pgfutil@tmpc{\pgfutil@tmpa,\pgfutil@tmpb}%
    \fi
	%
\fi
\edef\pgfmathresult{\pgfutil@tmpc}%
\pgfmathsmuggle\pgfmathresult\endgroup} 
% projection of a 3d coordinate on the normal of the screen
\pgfmathdeclarefunction{screendepth}{3}{%
\begingroup%
\pgfkeys{/pgf/fpu,/pgf/fpu/output format=fixed}%
\pgfmathparse{%
((\the\pgf@yx/1cm)*(\the\pgf@zy/1cm)-(\the\pgf@yy/1cm)*(\the\pgf@zx/1cm))*(#1)+%
((\the\pgf@zx/1cm)*(\the\pgf@xy/1cm)-(\the\pgf@xx/1cm)*(\the\pgf@zy/1cm))*(#2)+%
((\the\pgf@xx/1cm)*(\the\pgf@yy/1cm)-(\the\pgf@yx/1cm)*(\the\pgf@xy/1cm))*(#3)}%
\pgfmathsmuggle\pgfmathresult\endgroup%
}%
% returns the x, y and z coordinates of the normal on the screen
\pgfmathdeclarefunction*{nscreenx}{0}{%
\begingroup%
\pgfkeys{/pgf/fpu,/pgf/fpu/output format=fixed}%
\pgfmathparse{((\the\pgf@yx/1cm)*(\the\pgf@zy/1cm)-(\the\pgf@yy/1cm)*(\the\pgf@zx/1cm))}%
\pgfmathsmuggle\pgfmathresult\endgroup%
}%
\pgfmathdeclarefunction*{nscreeny}{0}{%
\begingroup%
\pgfkeys{/pgf/fpu,/pgf/fpu/output format=fixed}%
\pgfmathparse{((\the\pgf@zx/1cm)*(\the\pgf@xy/1cm)-(\the\pgf@xx/1cm)*(\the\pgf@zy/1cm))}%
\pgfmathsmuggle\pgfmathresult\endgroup%
}%
\pgfmathdeclarefunction*{nscreenz}{0}{%
\begingroup%
\pgfkeys{/pgf/fpu,/pgf/fpu/output format=fixed}%
\pgfmathparse{((\the\pgf@xx/1cm)*(\the\pgf@yy/1cm)-(\the\pgf@yx/1cm)*(\the\pgf@xy/1cm))}%
\pgfmathsmuggle\pgfmathresult\endgroup%
}%
% returns a vector that is orthogonal to the input vector
\pgfmathdeclarefunction{normalcandidate}{3}{%
\begingroup%
\pgfmathtruncatemacro{\icase}{(abs(#1)>0)+2*(abs(#2)>0)+4*(abs(#3)>0)}%
\ifcase\icase
\message{All three coordinates are zero. No normal can be computed.^^J}%
\edef\pgfmathresult{0,0,0}%
\or
\edef\pgfmathresult{0,1,0}%
\or
\edef\pgfmathresult{0,0,1}%
\or
\edef\pgfmathresult{0,0,1}%
\or
\edef\pgfmathresult{1,0,0}%
\or
\edef\pgfmathresult{0,1,0}%
\or
\edef\pgfmathresult{1,0,0}%
\or
\pgfmathsetmacro{\normalization}{(#1)*(#1)+(#2)*(#2)}%
\pgfmathsetmacro{\nx}{-1*(#2)/sqrt(\normalization)}%
\pgfmathsetmacro{\ny}{#1/sqrt(\normalization)}%
\edef\pgfmathresult{\nx,\ny,0}%
\fi
\pgfmathsmuggle\pgfmathresult\endgroup%
}%
\pgfmathdeclarefunction{randompermutation}{1}{%
\begingroup%	      
\c@pgf@counta=0%
\edef\pgfutil@tmpa{0}%
\loop
\advance\c@pgf@counta by1%
\edef\pgfutil@tmpa{\pgfutil@tmpa,\the\c@pgf@counta}%
\ifnum\c@pgf@counta<#1\relax
\repeat
\loop
\advance\c@pgf@counta by-1%
\pgfmathtruncatemacro{\pgfutil@tmpb}{1+rnd*\c@pgf@counta}%
\pgfmathtruncatemacro{\pgfutil@tmpc}{{\pgfutil@tmpa}[\pgfutil@tmpb]}%
\ifnum\c@pgf@counta=\numexpr#1-1\relax
\edef\pgfmathresult{\pgfutil@tmpc}%
\else
\edef\pgfmathresult{\pgfmathresult,\pgfutil@tmpc}%
\fi
\edef\pgfutil@tmpd{\pgfutil@tmpa}%
\edef\pgfutil@tmpa{0}%
\pgfutil@for\my@item:={\pgfutil@tmpd}\do{%
\unless\ifnum\pgfutil@tmpc=\my@item
\unless\ifnum\my@item=0\relax
\edef\pgfutil@tmpa{\pgfutil@tmpa,\my@item}%
\fi\fi}%
\ifnum\c@pgf@counta>0\relax
\repeat
\pgfmath@smuggleone\pgfmathresult%
\endgroup}
\pgfmathdeclarefunction{take}{2}{%
\begingroup%
\c@pgf@counta=0%
\pgfutil@for\my@item:={#1}\do{%
\advance\c@pgf@counta by1%
\ifnum\c@pgf@counta<#2\relax
\ifnum\c@pgf@counta=1\relax
\edef\pgfmathresult{\my@item}%
\else
\edef\pgfmathresult{\pgfmathresult,\my@item}%
\fi\fi}%
\pgfmath@smuggleone\pgfmathresult%
\endgroup}
%
%
% barycenter of a list of coordinates
\pgfmathdeclarefunction{barycenter}{1}{% barycentric coordinate 
\begingroup%
\edef\pgfutil@tmpb{0}%
\tikzset{3d/tmp/.code={\edef\pgfutil@tmpb{\the\numexpr\pgfutil@tmpb+1}%
\ifnum\pgfutil@tmpb=1
 \edef\pgfutil@tmpc{##1}%
\else
 \edef\pgfutil@tmpc{\pgfutil@tmpc+##1}%
\fi},3d/tmp/.list={#1}}%
\pgfmathsetmacro{\pgfutil@tmpc}{TD("\pgfutil@tmpc")}%
\pgfmathsetmacro{\pgfutil@tmpa}{1/\pgfutil@tmpb}%
\pgfmathparse{TD("\pgfutil@tmpa*(\pgfutil@tmpc)")}%   
\pgfmathsmuggle\pgfmathresult\endgroup}%
%
% position of a real in a list of reals
\pgfmathdeclarefunction*{pos}{2}{%
\begingroup%
\c@pgf@counta=1%
\pgfutil@for\my@item:={#2}\do{%
\ifdim\my@item pt<#1pt%
\advance\c@pgf@counta by1%
\fi}%
\edef\pgfmathresult{\the\c@pgf@counta}%
\pgfmathsmuggle\pgfmathresult\endgroup%
}
\pgfmathdeclarefunction*{x2d}{1}{%
\begingroup%
\pgf@process{\pgfpointanchor{#1}{center}}%
\pgfmathparse{\pgf@x}%
\pgfmathsmuggle\pgfmathresult\endgroup%
}%
\pgfmathdeclarefunction*{y2d}{1}{%
\begingroup%
\pgf@process{\pgfpointanchor{#1}{center}}%
\pgfmathparse{\pgf@y}%
\pgfmathsmuggle\pgfmathresult\endgroup%
}%
%
\tikzset{convex hull of/.code={% expects a list of points
\edef\pgfutil@tmpl{#1}% store the list for manipulations
\edef\pgfutil@tmpp{}% path to be constructed
\c@pgf@counta1%
\pgfutil@for\pgfutil@tmpa:={\pgfutil@tmpl}\do{%
\ifnum\c@pgf@counta=1\relax
\pgfmathsetmacro{\pgfutil@tmpb}{x2d("\pgfutil@tmpa")}% min
\edef\pgfutil@tmpd{\pgfutil@tmpa}% leftmost point
\else
\pgfmathsetmacro{\pgfutil@tmpc}{x2d("\pgfutil@tmpa")}% x coordinate
\ifdim\pgfutil@tmpc pt<\pgfutil@tmpb pt\relax
\edef\pgfutil@tmpb{\pgfutil@tmpc}% new min
\edef\pgfutil@tmpd{\pgfutil@tmpa}% new leftmost point
\fi
\fi
\advance\c@pgf@counta by1%
}
\edef\pgfutil@tmpp{(\pgfutil@tmpd)}%
\edef\pgfutil@tmpj{\pgfutil@tmpd}%
\edef\pgfutil@tmpe{90}% slope correction
\edef\pgfutil@tmpk{1}% first round flag
\loop
%\typeout{Removing  \pgfutil@tmpd}%
\edef\pgfutil@tmph{\noexpand\@removeelement{\pgfutil@tmpd}{\pgfutil@tmpl}{\noexpand\pgfutil@tmpl}}%
\pgfutil@tmph
%\typeout{List is now \pgfutil@tmpl}%
\c@pgf@countb1%
\pgfutil@for\pgfutil@tmpa:={\pgfutil@tmpl}\do{%
\pgfmathsetmacro{\pgfutil@tmpf}{Mod(atan2(y2d("\pgfutil@tmpa")-y2d("\pgfutil@tmpd"),
x2d("\pgfutil@tmpa")-x2d("\pgfutil@tmpd"))+\pgfutil@tmpe,360)}%
%\typeout{\the\c@pgf@countb: \pgfutil@tmpa\space has angle \pgfutil@tmpf.}%
\ifnum\c@pgf@countb=1\relax
\edef\pgfutil@tmpg{\pgfutil@tmpf}%
\edef\pgfutil@tmpi{\pgfutil@tmpa}%
\else
%\unless\ifdim\pgfutil@tmpf pt>180pt\relax
\ifdim\pgfutil@tmpf pt>\pgfutil@tmpg pt\relax
\edef\pgfutil@tmpg{\pgfutil@tmpf}%
\edef\pgfutil@tmpi{\pgfutil@tmpa}%
\fi
%\fi
\fi
\advance\c@pgf@countb by1%
}
%
\ifx\pgfutil@tmpi\pgfutil@tmpj\relax
\c@pgf@counta=2\relax
\else
\edef\pgfutil@tmpd{\pgfutil@tmpi}%
\edef\pgfutil@tmpp{\pgfutil@tmpp--(\pgfutil@tmpd)}%
\pgfmathsetmacro{\pgfutil@tmpe}{180+\pgfutil@tmpe-\pgfutil@tmpf}%
%\typeout{offset angle=\pgfutil@tmpe}%
\advance\c@pgf@counta by-1%
\fi
\ifnum\pgfutil@tmpk=1\relax
\edef\pgfutil@tmpl{\pgfutil@tmpl,\pgfutil@tmpj}% add the first point again
\edef\pgfutil@tmpk{0}%
\fi
\ifnum\c@pgf@counta>2\relax
\repeat
\edef\pgfutil@tmpp{\pgfutil@tmpp--cycle}%
%\typeout{hull path=\pgfutil@tmpp}%
\tikzset{insert path=\pgfutil@tmpp}%
}}
%
\tikzset{generous outside path/.style={overlay,insert path={[reset cm]
			(-16383.99999pt,-16383.99999pt) |-
			(16383.99999pt,16383.99999pt)|- cycle}},
		 generous outside path'/.style={overlay,insert path={[reset cm]
			(-16383.99999pt,-16383.99999pt) -|
			(16383.99999pt,16383.99999pt)-| cycle}}}
%			
\tikzset{even odd clip/.code={\pgfseteorule}}			
%
\tikzset{%
	save named path/.code={\tikz@addmode{\pgfsyssoftpath@getcurrentpath\pgfutil@tmpf
		\global\expandafter\let\csname tikz@td@named@path@#1\endcsname=\pgfutil@tmpf}},
	use named path/.code={%
		\expandafter\pgfsyssoftpath@setcurrentpath\expandafter{\csname tikz@td@named@path@#1\endcsname}}
}
%
\pgfkeys{% https://tex.stackexchange.com/a/20426
  /tikz/on layer/.code={
    \pgfonlayer{#1}\begingroup
    \aftergroup\endpgfonlayer
    \aftergroup\endgroup
  },
  /tikz/node on layer/.code={
    \gdef\node@@on@layer{%
      \setbox\tikz@tempbox=\hbox\bgroup\pgfonlayer{#1}\unhbox\tikz@tempbox\endpgfonlayer\egroup}
    \aftergroup\node@on@layer
  },
  /tikz/end node on layer/.code={
    \endpgfonlayer\endgroup\endgroup
  }
}
%
\def\node@on@layer{\aftergroup\node@@on@layer}
%
% the following is very much "inspired" by the calc library 
\long\def\pgfmathtdparse#1{% < and > really are placeholders for a later integration
\begingroup% into calc, which however requires changes both in
% tikzlibrarycalc.code.tex and in tikz.code.tex
% 
% tdparse main computation. It's a series of optional factors in front 
% of coordinates. It is very much copied from the calc library. 
% maybe one can implement groups via [ ... ]
% 
\edef\pgf@Xa{0pt}% We accumulate the result in here. 
\edef\pgf@Ya{0pt}% 
\edef\pgf@Za{0pt}% 
%\typeout{Got #1 to parse.}%
\tikz@td@cc@parse+#1% 
}% 
\def\tikz@td@cc@parse{% 
\pgfutil@ifnextchar>{% 
% Ok, we found the end... 
\tikz@td@cc@end% 
} 
{\pgfutil@ifnextchar+{% 
% Ok, we found a coordinate... 
\tikz@td@cc@add% 
}{% 
\pgfutil@ifnextchar-{% 
\tikz@td@cc@sub% 
}{% 
\pgfutil@ifnextchar x{% 
\tikz@td@cc@vecprod% 
}{% 
\pgfutil@ifnextchar o{% 
\tikz@td@cc@scalprod% 
}{% 
\pgfutil@ifnextchar[{% 
%\typeout{Found a [.}%
\tikz@td@cc@pgfparse% 
}{% \tikzerror{+ or - expected}% 
\tikz@td@cc@end%
}% 
}% 
}% 
}% 
}%
}%
}%
% 
% The end is reached with > at the moment but this should change 
% 
\def\tikz@td@cc@end{% 
\ifcase\tikz@td@type%
\pgfmathsetmacro{\pgftemp@x}{\pgf@Xa}% 
\pgfmathsetmacro{\pgftemp@y}{\pgf@Ya}% 
\pgfmathsetmacro{\pgftemp@z}{\pgf@Za}% 
\edef\pgfmathresult{\pgftemp@x,\pgftemp@y,\pgftemp@z}%
\or%
\pgfmathsetmacro{\myxa}{\pgf@Xa}%
\pgfmathsetmacro{\myya}{\pgf@Ya}%
\pgfmathsetmacro{\myza}{\pgf@Za}%
\pgfmathsetmacro{\myxb}{\pgf@Xb}%
\pgfmathsetmacro{\myyb}{\pgf@Yb}%
\pgfmathsetmacro{\myzb}{\pgf@Zb}%
\pgfmathsetmacro{\pgftemp@x}{\vpauxx{\myxb}{\myyb}{\myzb}{\myxa}{\myya}{\myza}}% 
\pgfmathsetmacro{\pgftemp@y}{\vpauxy{\myxb}{\myyb}{\myzb}{\myxa}{\myya}{\myza}}% 
\pgfmathsetmacro{\pgftemp@z}{\vpauxz{\myxb}{\myyb}{\myzb}{\myxa}{\myya}{\myza}}% 
%\typeout{P1=(\myxb,\myyb,\myzb),P2=(\myxa,\myya,\myza),P1xP2=(\pgftemp@x,\pgftemp@y,\pgftemp@z)}%
\edef\pgfmathresult{\pgftemp@x,\pgftemp@y,\pgftemp@z}%
\or%
\pgfmathsetmacro{\myxa}{\pgf@Xa}%
\pgfmathsetmacro{\myya}{\pgf@Ya}%
\pgfmathsetmacro{\myza}{\pgf@Za}%
\pgfmathsetmacro{\myxb}{\pgf@Xb}%
\pgfmathsetmacro{\myyb}{\pgf@Yb}%
\pgfmathsetmacro{\myzb}{\pgf@Zb}%
\pgfmathparse@td@FPU{\myxa*\myxb+\myya*\myyb+\myza*\myzb}%
%\typeout{P1=(\myxb,\myyb,\myzb),P2=(\myxa,\myya,\myza),P1.P2=(\pgmfmathresult)}%
\fi%
%\message{result = (\pgftemp@x,\pgftemp@y,\pgftemp@z)=\pgfmathresult^^J}%
\xdef\tikz@td@type{0}% reset type to linear combination
\pgfmathsmuggle\pgfmathresult\endgroup}% 
% 
\def\tikz@td@cc@add+{% 
\def\tikz@td@cc@factor{1}% 
\tikz@td@cc@factororcoordinate% 
}% 
\def\tikz@td@cc@sub-{% 
\def\tikz@td@cc@factor{-1}% 
\tikz@td@cc@factororcoordinate% 
}% 
\def\tikz@td@cc@vecprod x{% 
%\message{Ah, a vector product^^J}%
\xdef\tikz@td@type{1}%
\edef\pgf@Xb{\pgf@Xa}% store current vector in b
\edef\pgf@Yb{\pgf@Ya}%
\edef\pgf@Zb{\pgf@Za}%
\edef\pgf@Xa{0pt}% reset a
\edef\pgf@Ya{0pt}%
\edef\pgf@Za{0pt}%
\def\tikz@td@cc@factor{1}%
\tikz@td@cc@factororcoordinate% 
}%
\def\tikz@td@cc@scalprod o{% 
%\message{Ah, a scalar product^^J}%
\xdef\tikz@td@type{2}%
\edef\pgf@Xb{\pgf@Xa}% store current vector in b
\edef\pgf@Yb{\pgf@Ya}%
\edef\pgf@Zb{\pgf@Za}%
\edef\pgf@Xa{0pt}% reset a
\edef\pgf@Ya{0pt}%
\edef\pgf@Za{0pt}%
\def\tikz@td@cc@factor{1}%
\tikz@td@cc@factororcoordinate% 
}%
% 
% Check for a factor: If we see a (, its a coordinate... 
% 
\def\tikz@td@cc@factororcoordinate{% 
\pgfutil@ifnextchar({%) 
% Ok, found coordinate 
\tikz@td@cc@coordinate% 
}{% 
\pgfutil@ifnextchar[{%] 
% Ok, found ordinary expression to parse
\tikz@td@cc@pgfparse% 
}{% 
\tikz@td@cc@parse@factor% 
}% 
}% 
}% 
% 
% ... otherwise it's a factor. It ends at ...*( 
% 
\def\tikz@td@cc@pgfparse[#1]{% 
%\typeout{Parsing expression #1, previously the factor was \tikz@td@cc@factor.}%
\pgfmathsetmacro{\tikz@td@cc@factor}{\tikz@td@cc@factor*(#1)}%
%\typeout{Now the factor is \tikz@td@cc@factor.}%
\tikz@td@cc@factororcoordinate% 
}% 
%
\def\tikz@td@cc@parse@factor#1*({% 
%\typeout{Factor: got #1}.%
\pgfmathparse@td@FPU{#1*\tikz@td@cc@factor}% 
\let\tikz@td@cc@factor=\pgfmathresult% 
\tikz@td@cc@coordinate(%) 
}% 
\def\tikz@td@cc@coordinate(#1){% 
\tikz@td@parse@coord(#1)% 
\pgfmathsetmacro{\pgf@Xa}{\pgf@Xa+\tikz@td@cc@factor*\pgf@X}%
\pgfmathsetmacro{\pgf@Ya}{\pgf@Ya+\tikz@td@cc@factor*\pgf@Y}%
\pgfmathsetmacro{\pgf@Za}{\pgf@Za+\tikz@td@cc@factor*\pgf@Z}%
\tikz@td@cc@parse% 
}% 
\tikzset{declare function={torusx(\u,\v,\R,\r)=cos(\u)*(\R + \r*cos(\v)); 
torusy(\u,\v,\R,\r)=(\R + \r*cos(\v))*sin(\u);
torusz(\u,\v,\R,\r)=\r*sin(\v);
torusvcrit1(\u,\th)=atan(tan(\th)*sin(\u));% first critical v value
torusvcrit2(\u,\th)=180+atan(tan(\th)*sin(\u));% second critical v value
torusvtest(\u,\v,\az,\el)=sin(-vcrit1(\u-\az,\el)+\v);
torusdisc(\th,\R,\r)=((pow(\r,2)-pow(\R,2))*pow(cot(\th),2)+% 
pow(\r,2)*(2+pow(tan(\th),2)))/pow(\R,2);% discriminant
torusumax(\th,\R,\r)=ifthenelse(torusdisc(\th,\R,\r)>0,asin(sqrt(abs(torusdisc(\th,\R,\r)))),0);
}}%
%
\tikzset{3d parse/.style={%/utils/exec=\pgfmathtdparse{#1},%
insert path={\pgfextra{\pgfmathtdparse{#1}}(\pgfmathresult)}},
3d coordinate/.style args={#1=#2}{%
%/utils/exec=\pgfmathtdparse{#2},%
insert path={\pgfextra{\pgfmathtdparse{#2}}(\pgfmathresult) coordinate #1}}}%
\newcommand\pgfmathprintvector[2][]{%
\begingroup
\pgfkeys{#1}%
\pgfutil@tempcnta0%
\pgfutil@for\pgf@tmp:={#2}\do{\advance\pgfutil@tempcnta by1}%
\pgfutil@tempcntb1%
\pgfutil@for\pgf@tmp:={#2}\do{\advance\pgfutil@tempcntb by1%
\ifnum\pgfutil@tempcntb<\pgfutil@tempcnta
\pgfmathparse{\pgf@tmp}%
\pgfmathprintnumber{\pgfmathresult},%
\else
\pgfmathparse{\pgf@tmp}%
\pgfmathprintnumber{\pgfmathresult}%
\fi}%
\endgroup
}%
% 
% projection of a point on a line
\tikzset{3d/projection precomputations/.code n args={3}{%
\pgfmathsetmacro{\pgfutil@tmpa}{TD("#2-#3o#1-#3")/TD("#2-#3o#2-#3")}%
\pgfmathsetmacro{\pgfutil@tmpb}{TD("#3+\pgfutil@tmpa*#2-\pgfutil@tmpa*#3")}%
},3d/projection of/.style args={#1 on #2--#3}{%
3d/projection precomputations={#1}{#2}{#3},%
insert path={[3d parse={(\pgfutil@tmpb)}]}
}}
%
% define extended objects and project point on line or plane
\tikzset{3d/.cd,
plane through/.code args={#1 and #2 and #3 named #4}{%
%\typeout{#2-#1x#3-#1}%
\pgfmathsetmacro{\pgfutil@tmpa}{TD("#2-#1x#3-#1")}%
\pgfmathsetmacro{\pgfutil@tmpb}{TD("(\pgfutil@tmpa)o(\pgfutil@tmpa)")}%
\ifdim\pgfutil@tmpb pt<0.01pt\relax
\PackageWarning{3dtools}{The points #1 and #2 and #3 are either too close to each other or almost
on one line, so not suited to define a plane.}%
\else
\pgfmathsetmacro{\pgfutil@tmpc}{1/sqrt(\pgfutil@tmpb)}%
\pgfmathsetmacro{\pgfutil@tmpd}{TD("\pgfutil@tmpc*(\pgfutil@tmpa)")}%
\pgfmathsetmacro{\pgfutil@tmpe}{TD("#1")}%
%\typeout{normal=(\pgfutil@tmpd),point=(\pgfutil@tmpe),name=#4}%
\expandafter\xdef\csname tikz@td@plane@normal@#4\endcsname{\pgfutil@tmpd}%
\expandafter\xdef\csname tikz@td@plane@point@#4\endcsname{\pgfutil@tmpe}%
\expandafter\xdef\csname tikz@td@dim@#4\endcsname{2}%
\fi
},%
plane with normal/.code args={#1 through #2 named #3}{%
\pgfmathsetmacro{\pgfutil@tmpn}{sqrt(TD("#1o#1"))}%
\ifdim\pgfutil@tmpn pt<0.02pt\relax
\PackageWarning{3dtools}{Normal (\pgfutil@tmpn) is too short.}%
\else
\pgfmathsetmacro{\pgfutil@tmpn}{1/\pgfutil@tmpn}%
\pgfmathsetmacro{\pgfutil@tmpd}{TD("\pgfutil@tmpn*#1")}%
\pgfmathsetmacro{\pgfutil@tmpe}{TD("#2")}%
\expandafter\xdef\csname tikz@td@plane@normal@#3\endcsname{\pgfutil@tmpd}%
\expandafter\xdef\csname tikz@td@plane@point@#3\endcsname{\pgfutil@tmpe}%
\expandafter\xdef\csname tikz@td@dim@#3\endcsname{2}%
\fi
},%
line through/.code args={#1 and #2 named #3}{%
\pgfmathsetmacro{\pgfutil@tmpd}{TD("#1")}%
\pgfmathsetmacro{\pgfutil@tmpe}{TD("#2")}%
\pgfmathsetmacro{\pgfutil@tmpf}{TD("#1-#2o#1-#2")}%
\ifdim\pgfutil@tmpf pt<0.001pt\relax
\PackageWarning{3dtools}{The points #1 and #2 are too close to each other. No line defined.}%
\else
\expandafter\xdef\csname tikz@td@line@A@#3\endcsname{\pgfutil@tmpd}%
\expandafter\xdef\csname tikz@td@line@B@#3\endcsname{\pgfutil@tmpe}%
\expandafter\xdef\csname tikz@td@dim@#3\endcsname{1}%
\fi
},%
line with direction/.code args={#1 through #2 named #3}{%
\pgfmathsetmacro{\pgfutil@tmpd}{TD("#2")}%
\pgfmathsetmacro{\pgfutil@tmpe}{TD("#1+#2")}%
\pgfmathsetmacro{\pgfutil@tmpf}{TD("#1o#1")}%
\ifdim\pgfutil@tmpf pt<0.001pt\relax
\PackageWarning{3dtools}{The points #1 and #2 are too close to each other. No line defined.}%
\else
\expandafter\xdef\csname tikz@td@line@A@#3\endcsname{\pgfutil@tmpd}%
\expandafter\xdef\csname tikz@td@line@B@#3\endcsname{\pgfutil@tmpe}%
\expandafter\xdef\csname tikz@td@dim@#3\endcsname{1}%
\fi
},%
sphere with center/.code args={#1 and radius #2 named #3}{%
\pgfmathsetmacro{\pgfutil@tmpd}{TD("#1")}%
\expandafter\xdef\csname tikz@td@sphere@C@#3\endcsname{\pgfutil@tmpd}%
\expandafter\xdef\csname tikz@td@sphere@r@#3\endcsname{#2}%
\expandafter\xdef\csname tikz@td@dim@#3\endcsname{3}% reserve 3 for sphere...
},
project/.code args={#1 on #2}{%
\expandafter\edef\expandafter\pgfutil@tmpd{\csname tikz@td@dim@#2\endcsname}%
\ifcase\pgfutil@tmpd
\PackageWarning{3dtools}{It is not particularly meaningful to project a point on a point.}
\or% line
\expandafter\edef\expandafter\pgfutil@tmpa{\csname tikz@td@line@A@#2\endcsname}%
\expandafter\edef\expandafter\pgfutil@tmpb{\csname tikz@td@line@B@#2\endcsname}%
\pgfmathsetmacro{\pgfutil@tmpd}{TD("(\pgfutil@tmpa)-(\pgfutil@tmpb)o#1-(\pgfutil@tmpb)")/TD("(\pgfutil@tmpa)-(\pgfutil@tmpb)o(\pgfutil@tmpa)-(\pgfutil@tmpb)")}%
\pgfmathsetmacro{\pgfutil@tmpc}{TD("(\pgfutil@tmpb)+\pgfutil@tmpd*(\pgfutil@tmpa)-\pgfutil@tmpd*(\pgfutil@tmpb)")}%
%\typeout{alpha=\pgfutil@tmpd,projection=(\pgfutil@tmpc)}%
\tikzset{insert path={(\pgfutil@tmpc)}}%
\or% plane
\expandafter\edef\expandafter\pgfutil@tmpn{\csname tikz@td@plane@normal@#2\endcsname}%
\expandafter\edef\expandafter\pgfutil@tmpa{\csname tikz@td@plane@point@#2\endcsname}%
\pgfmathsetmacro{\pgfutil@tmpb}{TD("(\pgfutil@tmpn)o(\pgfutil@tmpa)-#1")}%
\pgfmathsetmacro{\pgfutil@tmpc}{TD("#1+\pgfutil@tmpb*(\pgfutil@tmpn)")}%
%\typeout{alpha=\pgfutil@tmpb,projection=(\pgfutil@tmpc)}%
\tikzset{insert path={(\pgfutil@tmpc)}}%
\fi
}}
%%
%% intersections in 3d (so far: intersection of line with line, plane, or sphere)
\tikzset{3d/intersection of/.code args={#1 with #2}{%
\expandafter\edef\expandafter\pgfutil@tmpd{\csname tikz@td@dim@#1\endcsname}%
\expandafter\edef\expandafter\pgfutil@tmpe{\csname tikz@td@dim@#2\endcsname}%
\edef\pgfutil@tmpde{\pgfutil@tmpd\pgfutil@tmpe}%
\edef\pgfutil@tmpf{0}% flag
\ifnum\pgfutil@tmpde=11\relax% line with line
 \expandafter\edef\expandafter\pgfutil@tmpa{\csname tikz@td@line@B@#1\endcsname}%
 \expandafter\edef\expandafter\pgfutil@tmpb{\csname tikz@td@line@B@#2\endcsname}%
 \expandafter\edef\expandafter\pgfutil@tmpc{\csname tikz@td@line@A@#1\endcsname}%
 \expandafter\edef\expandafter\pgfutil@tmpd{\csname tikz@td@line@A@#2\endcsname}%
\edef\pgfutil@tmpf{3}% 
\else
\ifnum\pgfutil@tmpde=21\relax% plane with line
 \expandafter\edef\expandafter\pgfutil@tmpa{\csname tikz@td@line@A@#2\endcsname}%
 \expandafter\edef\expandafter\pgfutil@tmpb{\csname tikz@td@line@B@#2\endcsname}%
 \expandafter\edef\expandafter\pgfutil@tmpn{\csname tikz@td@plane@normal@#1\endcsname}%
 \expandafter\edef\expandafter\pgfutil@tmpc{\csname tikz@td@plane@point@#1\endcsname}%
 \edef\pgfutil@tmpf{1}%
 \else
  \ifnum\pgfutil@tmpde=12\relax% line with plane
   \expandafter\edef\expandafter\pgfutil@tmpa{\csname tikz@td@line@A@#1\endcsname}%
   \expandafter\edef\expandafter\pgfutil@tmpb{\csname tikz@td@line@B@#1\endcsname}%
   \expandafter\edef\expandafter\pgfutil@tmpn{\csname tikz@td@plane@normal@#2\endcsname}%
   \expandafter\edef\expandafter\pgfutil@tmpc{\csname tikz@td@plane@point@#2\endcsname}%
   \edef\pgfutil@tmpf{1}% flag
  \else
   \ifnum\pgfutil@tmpde=13\relax% line with sphere
	\expandafter\edef\expandafter\pgfutil@tmpa{\csname tikz@td@line@A@#1\endcsname}%
	\expandafter\edef\expandafter\pgfutil@tmpb{\csname tikz@td@line@B@#1\endcsname}%
	\expandafter\edef\expandafter\pgfutil@tmpc{\csname tikz@td@sphere@C@#2\endcsname}%
	\expandafter\edef\expandafter\pgfutil@tmpr{\csname tikz@td@sphere@r@#2\endcsname}%
	\edef\pgfutil@tmpf{2}%
	%\typeout{line with sphere}%
   \else
	\ifnum\pgfutil@tmpde=31\relax% sphere with line
	\expandafter\edef\expandafter\pgfutil@tmpa{\csname tikz@td@line@A@#2\endcsname}%
	\expandafter\edef\expandafter\pgfutil@tmpb{\csname tikz@td@line@B@#2\endcsname}%
	\expandafter\edef\expandafter\pgfutil@tmpc{\csname tikz@td@sphere@C@#1\endcsname}%
	\expandafter\edef\expandafter\pgfutil@tmpr{\csname tikz@td@sphere@r@#1\endcsname}%
	\edef\pgfutil@tmpf{2}%
    %\typeout{sphere with line}%
	\else
	 \PackageWarning{3dtools}{Currently, one intersection object has to be a plane and the other 
  	   one a line. However, #1 has dimension \pgfutil@tmpd\space and 
	   #2 has dimension \pgfutil@tmpe.}%
	\fi
   \fi	
  \fi
 \fi
\fi
\ifnum\pgfutil@tmpf=1\relax% reasonable input, stored in a, b, c and n
%\typeout{debug: A=(\pgfutil@tmpa), B=(\pgfutil@tmpb), C=(\pgfutil@tmpc), n=(\pgfutil@tmpn)}%
\pgfmathsetmacro{\pgfutil@tmpg}{TD("(\pgfutil@tmpn)o(\pgfutil@tmpb)-(\pgfutil@tmpa)")}%
\pgfmathtruncatemacro{\pgfutil@tmph}{abs(\pgfutil@tmpg)>0.01?1:0}% 
\ifnum\pgfutil@tmph=1\relax%
\pgfmathsetmacro{\pgfutil@tmpi}{TD("(\pgfutil@tmpn)o(\pgfutil@tmpc)-(\pgfutil@tmpa)")/\pgfutil@tmpg}%
\pgfmathsetmacro{\pgfutil@tmpj}{TD("(\pgfutil@tmpa)+\pgfutil@tmpi*(\pgfutil@tmpb)-\pgfutil@tmpi*(\pgfutil@tmpa)")}%
\tikzset{insert path={(\pgfutil@tmpj)}}%
%\typeout{debug: intersection is at (\pgfutil@tmpj)}%
\else
\PackageWarning{3dtools}{The plane and line do not intersect within the uncertainties. Returning (0,0,0) instead.}%
\fi
\fi
\ifnum\pgfutil@tmpf=2\relax% line and sphere
\pgfmathsetmacro@td@FPU{\pgfutil@tmpg}{TD("(\pgfutil@tmpb)-(\pgfutil@tmpa)o(\pgfutil@tmpb)-(\pgfutil@tmpa)")}%
\pgfmathsetmacro@td@FPU{\pgfutil@tmph}{2*TD("(\pgfutil@tmpa)-(\pgfutil@tmpc)o(\pgfutil@tmpb)-(\pgfutil@tmpa)")}%
\pgfmathsetmacro@td@FPU{\pgfutil@tmpi}{TD("(\pgfutil@tmpa)-(\pgfutil@tmpc)o(\pgfutil@tmpa)-(\pgfutil@tmpc)")-\pgfutil@tmpr*\pgfutil@tmpr}%
\pgfmathsetmacro@td@FPU{\pgfutil@tmpj}{sign(\pgfutil@tmph*\pgfutil@tmph-4*\pgfutil@tmpg*\pgfutil@tmpi)}%
\ifdim\pgfutil@tmpj pt<0pt\relax
\PackageWarning{3dtools}{The sphere and line do not intersect within the uncertainties. Returning (0,0,0) instead.}%
\else
\pgfmathsetmacro@td@FPU{\pgfutil@tmpk}{-1*(\pgfutil@tmph+sqrt(\pgfutil@tmph*\pgfutil@tmph-4*\pgfutil@tmpg*\pgfutil@tmpi))/2/\pgfutil@tmpg}%
%\typeout{k=\pgfutil@tmpk}
\edef\pgfutil@tmpm{0}%
\ifdim\pgfutil@tmpk pt>0pt\relax
 \ifdim\pgfutil@tmpk pt<1pt\relax
  \edef\pgfutil@tmpm{1}%
  \pgfmathsetmacro{\pgfutil@tmpn}{TD("(\pgfutil@tmpa)+\pgfutil@tmpk*(\pgfutil@tmpb)-\pgfutil@tmpk*(\pgfutil@tmpa)")}%
  \tikzset{insert path={(\pgfutil@tmpn) coordinate (\pgfkeysvalueof{/tikz/3d/aux keys/intersection 1})}}%
  %\typeout{first intersection inserted.}%
 \fi
\fi
\pgfmathsetmacro@td@FPU{\pgfutil@tmpk}{-1*(\pgfutil@tmph-sqrt(\pgfutil@tmph*\pgfutil@tmph-4*\pgfutil@tmpg*\pgfutil@tmpi))/2/\pgfutil@tmpg}%
%\typeout{k=\pgfutil@tmpk}
\ifdim\pgfutil@tmpk pt>0pt\relax
 \ifdim\pgfutil@tmpk pt<1pt\relax
  \pgfmathsetmacro{\pgfutil@tmpn}{TD("(\pgfutil@tmpa)+\pgfutil@tmpk*(\pgfutil@tmpb)-\pgfutil@tmpk*(\pgfutil@tmpa)")}%
  \ifnum\pgfutil@tmpm=1
   \tikzset{insert path={(\pgfutil@tmpn) coordinate (\pgfkeysvalueof{/tikz/3d/aux keys/intersection 2})}}%
  \else
   \tikzset{insert path={(\pgfutil@tmpn) coordinate (\pgfkeysvalueof{/tikz/3d/aux keys/intersection 1})}}%
  \fi
 \fi
\fi
% cont
\fi
\fi
\ifnum\pgfutil@tmpf=3\relax% intersection between two lines, follow https://math.stackexchange.com/a/271366
 \pgfmathsetmacro{\pgfutil@tmpC}{TD("(\pgfutil@tmpc)")}%
 \pgfmathsetmacro{\pgfutil@tmpD}{TD("(\pgfutil@tmpd)")}%
 \pgfmathsetmacro{\pgfutil@tmpi}{sqrt(TD("(\pgfutil@tmpC)-(\pgfutil@tmpD)o(\pgfutil@tmpC)-(\pgfutil@tmpD)"))}%
 \ifdim\pgfutil@tmpi pt<0.05pt\relax
  \tikzset{insert path={(\pgfutil@tmpC) coordinate (\pgfkeysvalueof{/tikz/3d/aux keys/intersection 1})}}%
 \else
  \pgfmathsetmacro{\pgfutil@tmpE}{TD("(\pgfutil@tmpc)-(\pgfutil@tmpa)")}%
  \pgfmathsetmacro{\pgfutil@tmpF}{TD("(\pgfutil@tmpd)-(\pgfutil@tmpb)")}%
  \pgfmathsetmacro{\pgfutil@tmpG}{TD("(\pgfutil@tmpD)-(\pgfutil@tmpC)")}%
  \pgfmathsetmacro{\pgfutil@tmpH}{TD("(\pgfutil@tmpF)x(\pgfutil@tmpG)")}%
  \pgfmathsetmacro{\pgfutil@tmpK}{TD("(\pgfutil@tmpF)x(\pgfutil@tmpE)")}%
  \pgfmathsetmacro@td@FPU{\pgfutil@tmph}{sqrt(TD("(\pgfutil@tmpH)o(\pgfutil@tmpH)"))}%
  \pgfmathsetmacro@td@FPU{\pgfutil@tmpk}{sqrt(TD("(\pgfutil@tmpK)o(\pgfutil@tmpK)"))}%
  \ifdim\pgfutil@tmph pt<0.01pt\relax
   \PackageWarning{3dtools}{The lines do not intersect within the uncertainties. Returning (0,0,0) instead.}%
  \else
   \ifdim\pgfutil@tmpk pt<0.01pt\relax
	\PackageWarning{3dtools}{The lines do not intersect within the uncertainties. Returning (0,0,0) instead.}%
   \else
	\pgfmathsetmacro@td@FPU{\pgfutil@tmpl}{sign(TD("(\pgfutil@tmpH)o(\pgfutil@tmpK)"))*\pgfutil@tmph/\pgfutil@tmpk}%
	\pgfmathsetmacro{\pgfutil@tmpM}{TD("(\pgfutil@tmpC)+\pgfutil@tmpl*(\pgfutil@tmpE)")}%
	\tikzset{insert path={(\pgfutil@tmpM) coordinate (\pgfkeysvalueof{/tikz/3d/aux keys/intersection 1})}}%
   \fi 
  \fi
 \fi
\fi
}}
%%
%% circumsphere center
\tikzset{3d/circumsphere center/.code={%
\tikzset{3d/aux keys/.cd,#1}%
\edef\pgfutil@tmpA{\pgfkeysvalueof{/tikz/3d/aux keys/A}}%
\edef\pgfutil@tmpB{\pgfkeysvalueof{/tikz/3d/aux keys/B}}%
\edef\pgfutil@tmpC{\pgfkeysvalueof{/tikz/3d/aux keys/C}}%
\edef\pgfutil@tmpD{\pgfkeysvalueof{/tikz/3d/aux keys/D}}%
% shifting to A=0 by redefining B, C and D
\pgfmathsetmacro{\pgfutil@tmpB}{TD("\pgfutil@tmpB-\pgfutil@tmpA")}%
\pgfmathsetmacro{\pgfutil@tmpC}{TD("\pgfutil@tmpC-\pgfutil@tmpA")}%
\pgfmathsetmacro{\pgfutil@tmpD}{TD("\pgfutil@tmpD-\pgfutil@tmpA")}%
% 
\pgfmathsetmacro{\pgfutil@tmpBxC}{TD("(\pgfutil@tmpB)x(\pgfutil@tmpC)")}%
\pgfmathsetmacro{\pgfutil@tmpCxD}{TD("(\pgfutil@tmpC)x(\pgfutil@tmpD)")}%
\pgfmathsetmacro{\pgfutil@tmpDxB}{TD("(\pgfutil@tmpD)x(\pgfutil@tmpB)")}%
% determinant (times 2)
\pgfmathsetmacro{\pgfutil@tmpd}{2*TD("(\pgfutil@tmpB)o(\pgfutil@tmpCxD)")}%
%\typeout{Determinant is \pgfutil@tmpd.}
\pgfmathtruncatemacro{\pgfutil@tmpi}{abs(\pgfutil@tmpd)>0.02?1:0}%
\ifnum\pgfutil@tmpi=0\relax
\PackageWarning{3dtools}{The points approximately sit on a common plane. The circumsphere cannot
be determined.}%
\else
\pgfmathsetmacro{\pgfutil@tmpnB}{TD("(\pgfutil@tmpB)o(\pgfutil@tmpB)")/\pgfutil@tmpd}%
\pgfmathsetmacro{\pgfutil@tmpnC}{TD("(\pgfutil@tmpC)o(\pgfutil@tmpC)")/\pgfutil@tmpd}%
\pgfmathsetmacro{\pgfutil@tmpnD}{TD("(\pgfutil@tmpD)o(\pgfutil@tmpD)")/\pgfutil@tmpd}%
\pgfmathsetmacro{\pgfutil@tmpI}{TD("\pgfutil@tmpA+\pgfutil@tmpnB*(\pgfutil@tmpCxD)+\pgfutil@tmpnC*(\pgfutil@tmpDxB)+\pgfutil@tmpnD*(\pgfutil@tmpBxC)")}%
\tikzset{insert path={(\pgfutil@tmpI)}}%
\fi
}}%
\tikzset{3d/circumcircle center/.code={%
\tikzset{3d/aux keys/.cd,#1}%
\edef\pgfutil@tmpA{\pgfkeysvalueof{/tikz/3d/aux keys/A}}%
\edef\pgfutil@tmpB{\pgfkeysvalueof{/tikz/3d/aux keys/B}}%
\edef\pgfutil@tmpC{\pgfkeysvalueof{/tikz/3d/aux keys/C}}%
% shifting to A=0 by redefining B and C
\pgfmathsetmacro{\pgfutil@tmpB}{TD("\pgfutil@tmpB-\pgfutil@tmpA")}%
\pgfmathsetmacro{\pgfutil@tmpC}{TD("\pgfutil@tmpC-\pgfutil@tmpA")}%
%\typeout{\pgfutil@tmpB,\pgfutil@tmpC}%
% 
\pgfmathsetmacro{\pgfutil@tmpBB}{TD("(\pgfutil@tmpB)o(\pgfutil@tmpB)")}%
\pgfmathsetmacro{\pgfutil@tmpBC}{TD("(\pgfutil@tmpB)o(\pgfutil@tmpC)")}%
\pgfmathsetmacro{\pgfutil@tmpCC}{TD("(\pgfutil@tmpC)o(\pgfutil@tmpC)")}%
%\typeout{\pgfutil@tmpBB,\pgfutil@tmpBC,\pgfutil@tmpCC}%
% determinant (times 2)
\pgfmathparse@td@FPU{2*(\pgfutil@tmpBB*\pgfutil@tmpCC-\pgfutil@tmpBC*\pgfutil@tmpBC)}%
\let\pgfutil@tmpd\pgfmathresult%
%\typeout{debug: determinant is \pgfutil@tmpd.}%
%\pgfmathtruncatemacro{\pgfutil@tmpi}{abs(\pgfutil@tmpd)>0.02?1:0}%
\pgfmathparse@td@FPU{int(abs(\pgfutil@tmpd)>0.02?1:0)}%
\pgfmathtruncatemacro{\pgfutil@tmpi}{\pgfmathresult}%
%\typeout{debug: i is \pgfutil@tmpi.}%
\ifnum\pgfutil@tmpi=0\relax
\PackageWarning{3dtools}{The points approximately sit on a common line. The circumcircle cannot
be determined.}%
\else
%\pgfmathsetmacro{\pgfutil@tmpb}{(\pgfutil@tmpBB-\pgfutil@tmpBC)*\pgfutil@tmpCC/\pgfutil@tmpd}%
\pgfmathparse@td@FPU{(\pgfutil@tmpBB-\pgfutil@tmpBC)*\pgfutil@tmpCC/\pgfutil@tmpd}%
\let\pgfutil@tmpb\pgfmathresult
%\typeout{debug: b is \pgfutil@tmpb.}%
%\pgfmathsetmacro{\pgfutil@tmpc}{(\pgfutil@tmpCC-\pgfutil@tmpBC)*\pgfutil@tmpBB/\pgfutil@tmpd}%
\pgfmathparse@td@FPU{(\pgfutil@tmpCC-\pgfutil@tmpBC)*\pgfutil@tmpBB/\pgfutil@tmpd}%
\let\pgfutil@tmpc\pgfmathresult
%\typeout{debug: c is \pgfutil@tmpc.}%
%\typeout{debug: b=\pgfutil@tmpb,c=\pgfutil@tmpc,(B)=(\pgfutil@tmpB),(C)=(\pgfutil@tmpC)}%
\pgfmathsetmacro{\pgfutil@tmpI}{TD("\pgfutil@tmpA+\pgfutil@tmpb*(\pgfutil@tmpB)+\pgfutil@tmpc*(\pgfutil@tmpC)")}%
%\typeout{debug: (I)=((\pgfutil@tmpI))}%
\tikzset{insert path={(\pgfutil@tmpI)}}%
\fi
}}%
\tikzset{3d/define orthonormal dreibein/.code={%
\tikzset{3d/aux keys/.cd,#1}%
\edef\pgfutil@tmpA{\pgfkeysvalueof{/tikz/3d/aux keys/A}}%
\edef\pgfutil@tmpB{\pgfkeysvalueof{/tikz/3d/aux keys/B}}%
\edef\pgfutil@tmpC{\pgfkeysvalueof{/tikz/3d/aux keys/C}}%
\pgfmathsetmacro{\pgfutil@tmpB}{TD("\pgfutil@tmpB-\pgfutil@tmpA")}%
\pgfmathsetmacro{\pgfutil@tmpC}{TD("\pgfutil@tmpC-\pgfutil@tmpA")}%
\pgfmathsetmacro{\pgfutil@tmpD}{TD("(\pgfutil@tmpB)x(\pgfutil@tmpC)")}%
\pgfmathsetmacro@td@FPU{\pgfutil@tmpd}{min(1,TD("(\pgfutil@tmpD)o(\pgfutil@tmpD)"))}% changed May 23 2023
\ifdim\pgfutil@tmpd pt<0.01pt\relax
\PackageWarning{3dtools}{The vectors \pgfutil@tmpA, \pgfutil@tmpB\space and 
\pgfutil@tmpC are too collinear. Cannot determine appropriate plane.}%
\else
\pgfmathsetmacro{\pgfutil@tmpB}{TDunit("(\pgfutil@tmpB)")}% changed May 23 2023
\pgfmathsetmacro{\pgfutil@tmpD}{TDunit("(\pgfutil@tmpD)")}% changed May 23 2023
\pgfmathsetmacro{\pgfutil@tmpC}{TD("(\pgfutil@tmpD)x(\pgfutil@tmpB)")}%
% \typeout{3d coordinate={\pgfkeysvalueof{/tikz/3d/aux keys/ex}=(\pgfutil@tmpB)},
% 	3d coordinate={\pgfkeysvalueof{/tikz/3d/aux keys/ey}=(\pgfutil@tmpC)},
% 	3d coordinate={\pgfkeysvalueof{/tikz/3d/aux keys/ez}=(\pgfutil@tmpD)}}%
\expanded{\noexpand\path[overlay,
	3d coordinate={\pgfkeysvalueof{/tikz/3d/aux keys/ex}=(\pgfutil@tmpB)},
	3d coordinate={\pgfkeysvalueof{/tikz/3d/aux keys/ey}=(\pgfutil@tmpC)},
	3d coordinate={\pgfkeysvalueof{/tikz/3d/aux keys/ez}=(\pgfutil@tmpD)}];}%
\fi
},3d/aux keys/.cd,A/.initial={(A)},B/.initial={(B)},
C/.initial={(C)},D/.initial={(D)},
intersection 1/.initial={I-1},intersection 2/.initial={I-2},
ex/.initial={(ex)},
ey/.initial={(ey)},ez/.initial={(ez)},
i1/.initial=i1,i2/.initial=i2,
rA/.initial=1,rB/.initial=1,rC/.initial=1,
tmpcoord1/.initial=3dtoolstmp-1}
\tikzset{3d/screen coords/.style={x={(1cm,0cm)},y={(0cm,1cm)},z={(-1cm,-1cm)}}}%
%%
%% predefined pics
\makeatletter
\tikzset{pics/3d/dim line/.style={code={%
  \tikzset{3d/dim line/.cd,#1}%
  \pgfmathsetmacro{\pgfutil@tmpa}{tddistance("\pgfkeysvalueof{/tikz/3d/dim line/A}","\pgfkeysvalueof{/tikz/3d/dim line/B}")}%
  \ifdim\pgfutil@tmpa pt<0.02pt\relax 
   \message{The points A=\pgfkeysvalueof{/tikz/3d/dim line/A} and B=\pgfkeysvalueof{/tikz/3d/dim line/B} are too close. Cannot draw dim line.}%
  \else 
    \pgfmathsetmacro{\pgfutil@tmpa}{TD("\pgfkeysvalueof{/tikz/3d/dim line/A}-\pgfkeysvalueof{/tikz/3d/dim line/B}x\pgfkeysvalueof{/tikz/3d/dim line/n}")}%
    \pgfmathsetmacro{\pgfutil@tmpb}{TD("(\pgfutil@tmpa)o(\pgfutil@tmpa)")}%
    \ifdim\pgfutil@tmpb pt<0.02pt\relax
      \message{The normal n=\pgfkeysvalueof{/tikz/3d/dim line/n} is either too short or too collinear with A-B=\pgfkeysvalueof{/tikz/3d/dim line/A}-\pgfkeysvalueof{/tikz/3d/dim line/B}. Cannot draw dim line.}%
    \else 
      % \pgfmathsetmacro{\pgfutil@tmpC}{TD("\pgfkeysvalueof{/tikz/3d/dim line/B}-\pgfkeysvalueof{/tikz/3d/dim line/A}x\pgfkeysvalueof{/tikz/3d/dim line/n}")}%
      % \pgfmathsetmacro{\pgfutil@tmpC}{TD("\pgfkeysvalueof{/tikz/3d/dim line/B}+(\pgfutil@tmpC)")}%
      % %\typeout{C=(\pgfutil@tmpC)}%
      % \tikzset{3d/define orthonormal dreibein={%
      %   A=\pgfkeysvalueof{/tikz/3d/dim line/A},%
      %   B=\pgfkeysvalueof{/tikz/3d/dim line/B},%
      %   C={(\pgfutil@tmpC)},%
      %   ex={(\pgfkeysvalueof{/tikz/3d/dim line/auxiliary coordinate prefix}ex)},%
      %   ey={(\pgfkeysvalueof{/tikz/3d/dim line/auxiliary coordinate prefix}ey)},%
      %   ez={(\pgfkeysvalueof{/tikz/3d/dim line/auxiliary coordinate prefix}ez)}%
      % }}%
      \pgfmathsetmacro{\pgfutil@tmpa}{TDunit("(\pgfutil@tmpa)")}%
      \pgfmathsetmacro{\pgfutil@tmpb}{\pgfkeysvalueof{/tikz/3d/dim line/d}/1cm}%
      \pgfmathsetmacro{\pgfutil@tmpex}{TDunit("\pgfkeysvalueof{/tikz/3d/dim line/B}-\pgfkeysvalueof{/tikz/3d/dim line/A}")}%
      \expanded{\noexpand\path[overlay]
        (\pgfutil@tmpex) coordinate (\pgfkeysvalueof{/tikz/3d/dim line/auxiliary coordinate prefix}ex);}
      \pgfmathtruncatemacro{\pgfutil@tmpf}{ifthenelse(x2d("\pgfkeysvalueof{/tikz/3d/dim line/auxiliary coordinate prefix}ex")<0,1,0)}%
      \ifnum\pgfutil@tmpf=1\relax 
        \pgfmathsetmacro{\pgfutil@tmpex}{TDunit("\pgfkeysvalueof{/tikz/3d/dim line/A}-\pgfkeysvalueof{/tikz/3d/dim line/B}")}%
      \fi
      \pgfmathsetmacro{\pgfutil@tmpey}{TDunit("\pgfkeysvalueof{/tikz/3d/dim line/n}x(\pgfutil@tmpex)")}%
      \expanded{\noexpand\path[overlay]
        (\pgfutil@tmpey) coordinate (\pgfkeysvalueof{/tikz/3d/dim line/auxiliary coordinate prefix}ey);}
      \pgfmathtruncatemacro{\pgfutil@tmpf}{ifthenelse(y2d("\pgfkeysvalueof{/tikz/3d/dim line/auxiliary coordinate prefix}ey")<0,1,0)}%
      \ifnum\pgfutil@tmpf=1\relax 
        \pgfmathsetmacro{\pgfutil@tmpey}{TDunit("(\pgfutil@tmpex)x\pgfkeysvalueof{/tikz/3d/dim line/n}")}%
      \fi
      \pgfmathsetmacro{\pgfutil@tmpez}{TDunit("\pgfkeysvalueof{/tikz/3d/dim line/n}")}%
      \pgfmathsetmacro{\pgfutil@tmpA}{TD("\pgfkeysvalueof{/tikz/3d/dim line/A}+\pgfutil@tmpb*(\pgfutil@tmpa)")}%
      \pgfmathsetmacro{\pgfutil@tmpB}{TD("\pgfkeysvalueof{/tikz/3d/dim line/B}+\pgfutil@tmpb*(\pgfutil@tmpa)")}%
      \pgfmathsetmacro{\pgfutil@tmpC}{TD("0.5*\pgfkeysvalueof{/tikz/3d/dim line/A}+0.5*\pgfkeysvalueof{/tikz/3d/dim line/B}+\pgfutil@tmpb*(\pgfutil@tmpa)")}%
      \expanded{\noexpand\path[overlay]
      % (\pgfutil@tmpa) coordinate (\pgfkeysvalueof{/tikz/3d/dim line/auxiliary coordinate prefix}D)
      (\pgfutil@tmpex) coordinate (\pgfkeysvalueof{/tikz/3d/dim line/auxiliary coordinate prefix}ex)
      (\pgfutil@tmpey) coordinate (\pgfkeysvalueof{/tikz/3d/dim line/auxiliary coordinate prefix}ey)
      (\pgfutil@tmpez) coordinate (\pgfkeysvalueof{/tikz/3d/dim line/auxiliary coordinate prefix}ez)
      (\pgfutil@tmpA) coordinate (\pgfkeysvalueof{/tikz/3d/dim line/auxiliary coordinate prefix}A')
      (\pgfutil@tmpB) coordinate (\pgfkeysvalueof{/tikz/3d/dim line/auxiliary coordinate prefix}B')
      (\pgfutil@tmpC) coordinate (\pgfkeysvalueof{/tikz/3d/dim line/auxiliary coordinate prefix}AB')
      ;}%
      \begin{scope}[x={(\pgfkeysvalueof{/tikz/3d/dim line/auxiliary coordinate prefix}ex)},
          y={(\pgfkeysvalueof{/tikz/3d/dim line/auxiliary coordinate prefix}ey)},
          z={(\pgfkeysvalueof{/tikz/3d/dim line/auxiliary coordinate prefix}ez)},canvas is xy plane at z=0]          
          \path (\pgfkeysvalueof{/tikz/3d/dim line/auxiliary coordinate prefix}AB') node[3d/dim line/dim label](\pgfkeysvalueof{/tikz/3d/dim line/node name}){\tikz@td@dim@line@label};
          \fill let \p1=($(\pgfkeysvalueof{/tikz/3d/dim line/node name}.west)-(\pgfkeysvalueof{/tikz/3d/dim line/node name}.east)$),\n1={0.5*sqrt((\x1)*(\x1)+(\y1)*(\y1))},\p2=($(\pgfkeysvalueof{/tikz/3d/dim line/node name})-(\pgfkeysvalueof{/tikz/3d/dim line/auxiliary coordinate prefix}A')$),\n2={sqrt((\x2)*(\x2)+(\y2)*(\y2))-\n1-0.4pt} in (\pgfkeysvalueof{/tikz/3d/dim line/node name}) ++ (\n1,0) -- ++ (0,0.2pt) -- ++ (\n2-3pt,0pt)
          -- ++ (0pt,1.3pt) -- ++ (3pt,-1.5pt) -- ++ (-3pt,-1.5pt)  -- ++ (0pt,1.3pt) -- ++ (3pt-\n2,0pt) -- cycle
          (\pgfkeysvalueof{/tikz/3d/dim line/node name}) ++ (-\n1,0) -- ++ (0,-0.2pt) -- ++ (3pt-\n2,0pt)
          -- ++ (0pt,-1.3pt) -- ++ (-3pt,1.5pt) -- ++ (3pt,1.5pt)  -- ++ (0pt,-1.3pt) -- ++ (\n2-3pt,0pt) -- cycle
          (\pgfkeysvalueof{/tikz/3d/dim line/node name}) ++ (\n1+\n2,1.5pt) -- ++ (0.4pt,0pt) -- ++ (0pt,-3pt) -- ++ (-0.4pt,0pt) -- cycle
          (\pgfkeysvalueof{/tikz/3d/dim line/node name}) ++ (0pt-\n1-\n2,-1.5pt) -- ++ (-0.4pt,0pt) -- ++ (0pt,3pt) -- ++ (0.4pt,0pt) -- cycle;
      \end{scope}
    \fi 
  \fi  
}},3d/dim line/.cd,A/.initial={(0,0,0)},B/.initial={(1,0,0)},n/.initial={(0,0,1)},
l/.store in=\tikz@td@dim@line@label,
l=\empty,
auxiliary coordinate prefix/.initial=tmp,d/.initial=2mm,
dim label/.style={transform shape,circle,inner sep=1pt},
node name/.initial=dim label}
% based on https://en.wikipedia.org/wiki/Circumscribed_circle
\tikzset{pics/3d circle through 3 points/.style={code={%
 \tikzset{3d/circle through 3 points/.cd,#1}%
 \expanded{\noexpand\path[overlay,
3d coordinate={(\pgfkeysvalueof{/tikz/3d/circle through 3 points/auxiliary coordinate prefix}b)=\pgfkeysvalueof{/tikz/3d/circle through 3 points/A}-\pgfkeysvalueof{/tikz/3d/circle through 3 points/C}},
 3d coordinate={(\pgfkeysvalueof{/tikz/3d/circle through 3 points/auxiliary coordinate prefix}a)=\pgfkeysvalueof{/tikz/3d/circle through 3 points/B}-\pgfkeysvalueof{/tikz/3d/circle through 3 points/C}},
 3d coordinate={(\pgfkeysvalueof{/tikz/3d/circle through 3 points/auxiliary coordinate prefix}c)=\pgfkeysvalueof{/tikz/3d/circle through 3 points/A}-\pgfkeysvalueof{/tikz/3d/circle through 3 points/B}},
 3d coordinate={(\pgfkeysvalueof{/tikz/3d/circle through 3 points/auxiliary coordinate prefix}n)=(\pgfkeysvalueof{/tikz/3d/circle through 3 points/auxiliary coordinate prefix}a)x(\pgfkeysvalueof{/tikz/3d/circle through 3 points/auxiliary coordinate prefix}b)}
 ];}%
 \pgfmathsetmacro@td@FPU{\lengthn}{sqrt(TD("(\pgfkeysvalueof{/tikz/3d/circle through 3 points/auxiliary coordinate prefix}n)o(\pgfkeysvalueof{/tikz/3d/circle through 3 points/auxiliary coordinate prefix}n)"))}
 \ifdim\lengthn pt<0.02pt\relax
   \message{The points are (almost) on a line. Circle cannot be determined.}
  \else
   \pgfmathsetmacro@td@FPU{\tmpradius}{sqrt(TD("(\pgfkeysvalueof{/tikz/3d/circle through 3 points/auxiliary coordinate prefix}a)o(\pgfkeysvalueof{/tikz/3d/circle through 3 points/auxiliary coordinate prefix}a)"))*%
   	sqrt(TD("(\pgfkeysvalueof{/tikz/3d/circle through 3 points/auxiliary coordinate prefix}b)o(\pgfkeysvalueof{/tikz/3d/circle through 3 points/auxiliary coordinate prefix}b)"))*sqrt(TD("(\pgfkeysvalueof{/tikz/3d/circle through 3 points/auxiliary coordinate prefix}c)o(\pgfkeysvalueof{/tikz/3d/circle through 3 points/auxiliary coordinate prefix}c)"))/%
		(2*\lengthn)}
   \pgfmathsetmacro@td@FPU{\coeffa}{-1*TD("(\pgfkeysvalueof{/tikz/3d/circle through 3 points/auxiliary coordinate prefix}b)o(\pgfkeysvalueof{/tikz/3d/circle through 3 points/auxiliary coordinate prefix}b)")/(2*TD("(\pgfkeysvalueof{/tikz/3d/circle through 3 points/auxiliary coordinate prefix}n)o(\pgfkeysvalueof{/tikz/3d/circle through 3 points/auxiliary coordinate prefix}n)"))}		
   \pgfmathsetmacro@td@FPU{\coeffb}{TD("(\pgfkeysvalueof{/tikz/3d/circle through 3 points/auxiliary coordinate prefix}a)o(\pgfkeysvalueof{/tikz/3d/circle through 3 points/auxiliary coordinate prefix}a)")/(2*TD("(\pgfkeysvalueof{/tikz/3d/circle through 3 points/auxiliary coordinate prefix}n)o(\pgfkeysvalueof{/tikz/3d/circle through 3 points/auxiliary coordinate prefix}n)"))}
   \expanded{%
   \noexpand\path[overlay,3d coordinate={(\pgfkeysvalueof{/tikz/3d/circle through 3 points/auxiliary coordinate prefix}u)=\coeffa*(\pgfkeysvalueof{/tikz/3d/circle through 3 points/auxiliary coordinate prefix}a)x(\pgfkeysvalueof{/tikz/3d/circle through 3 points/auxiliary coordinate prefix}n)},
     3d coordinate={(\pgfkeysvalueof{/tikz/3d/circle through 3 points/auxiliary coordinate prefix}v)=\coeffb*(\pgfkeysvalueof{/tikz/3d/circle through 3 points/auxiliary coordinate prefix}b)x(\pgfkeysvalueof{/tikz/3d/circle through 3 points/auxiliary coordinate prefix}n)}];
   \noexpand\path[3d coordinate={(\pgfkeysvalueof{/tikz/3d/circle through 3 points/center name})=\pgfkeysvalueof{/tikz/3d/circle through 3 points/C}+(\pgfkeysvalueof{/tikz/3d/circle through 3 points/auxiliary coordinate prefix}u)+(\pgfkeysvalueof{/tikz/3d/circle through 3 points/auxiliary coordinate prefix}v)}];
   }%
   \pgfmathsetmacro{\normalizationa}{1/sqrt(TD("(\pgfkeysvalueof{/tikz/3d/circle through 3 points/auxiliary coordinate prefix}a)o(\pgfkeysvalueof{/tikz/3d/circle through 3 points/auxiliary coordinate prefix}a)"))}
   \pgfmathsetmacro{\normalizationn}{1/sqrt(TD("(\pgfkeysvalueof{/tikz/3d/circle through 3 points/auxiliary coordinate prefix}n)o(\pgfkeysvalueof{/tikz/3d/circle through 3 points/auxiliary coordinate prefix}n)"))}
   \expanded{%
   \noexpand\path[overlay,3d coordinate={(\pgfkeysvalueof{/tikz/3d/circle through 3 points/auxiliary coordinate prefix}a)=\normalizationa*(\pgfkeysvalueof{/tikz/3d/circle through 3 points/auxiliary coordinate prefix}a)},
   3d coordinate={(\pgfkeysvalueof{/tikz/3d/circle through 3 points/auxiliary coordinate prefix}n)=\normalizationn*(\pgfkeysvalueof{/tikz/3d/circle through 3 points/auxiliary coordinate prefix}n)},
   3d coordinate={(\pgfkeysvalueof{/tikz/3d/circle through 3 points/auxiliary coordinate prefix}c)=(\pgfkeysvalueof{/tikz/3d/circle through 3 points/auxiliary coordinate prefix}a)x(\pgfkeysvalueof{/tikz/3d/circle through 3 points/auxiliary coordinate prefix}n)}];
   }%
   \expanded{%
	\noexpand\begin{scope}[plane x={(\pgfkeysvalueof{/tikz/3d/circle through 3 points/auxiliary coordinate prefix}a)},plane y={(\pgfkeysvalueof{/tikz/3d/circle through 3 points/auxiliary coordinate prefix}c)},canvas is plane]
	 \noexpand\draw[pic actions] (\pgfkeysvalueof{/tikz/3d/circle through 3 points/center name}) circle[radius=\tmpradius];
	 \noexpand\pgfkeys{/tikz/3d/circle through 3 points/extra}
	\noexpand\end{scope}}%
  \fi 
}},3d/circle through 3 points/.cd,A/.initial={(1,0,0)},B/.initial={(0,1,0)},
C/.initial={(0,0,1)},
auxiliary coordinate prefix/.initial=tmp,center name/.initial=M,
extra/.code={}}%
% 
% incircle
\tikzset{pics/3d incircle/.style={code={%
\tikzset{3d/incircle/.cd,#1}%
\pgfmathsetmacro{\pgfutil@tmpa}{tddistance("\pgfkeysvalueof{/tikz/3d/incircle/B}","\pgfkeysvalueof{/tikz/3d/incircle/C}")}%
\pgfmathsetmacro{\pgfutil@tmpb}{tddistance("\pgfkeysvalueof{/tikz/3d/incircle/A}","\pgfkeysvalueof{/tikz/3d/incircle/C}")}%
\pgfmathsetmacro{\pgfutil@tmpc}{tddistance("\pgfkeysvalueof{/tikz/3d/incircle/A}","\pgfkeysvalueof{/tikz/3d/incircle/B}")}%
\pgfmathsetmacro{\pgfutil@tmpd}{(\pgfutil@tmpa+\pgfutil@tmpb+\pgfutil@tmpc)/2}%
\pgfmathsetmacro{\pgfutil@tmparea}{sqrt(\pgfutil@tmpd*(\pgfutil@tmpd-\pgfutil@tmpa)*(\pgfutil@tmpd-\pgfutil@tmpb)*(\pgfutil@tmpd-\pgfutil@tmpc))}%
\pgfmathsetmacro{\pgfutil@tmpr}{\pgfutil@tmparea/\pgfutil@tmpd}%
%\edef\pgfutil@tmpt{\noexpand\tikz@td@parse@coord\pgfkeysvalueof{/tikz/3d/incircle/A}}%
%\pgfutil@tmpt
\expanded{\noexpand\tikz@td@parse@coord\pgfkeysvalueof{/tikz/3d/incircle/A}}%
\pgfmathsetmacro{\pgfutil@tmp@Ax}{\pgf@X}%
\pgfmathsetmacro{\pgfutil@tmp@Ay}{\pgf@Y}%
\pgfmathsetmacro{\pgfutil@tmp@Az}{\pgf@Z}%
%\edef\pgfutil@tmpt{\noexpand\tikz@td@parse@coord\pgfkeysvalueof{/tikz/3d/incircle/B}}%
%\pgfutil@tmpt
\expanded{\noexpand\tikz@td@parse@coord\pgfkeysvalueof{/tikz/3d/incircle/B}}%
\pgfmathsetmacro{\pgfutil@tmp@Bx}{\pgf@X}%
\pgfmathsetmacro{\pgfutil@tmp@By}{\pgf@Y}%
\pgfmathsetmacro{\pgfutil@tmp@Bz}{\pgf@Z}%
%\edef\pgfutil@tmpt{\noexpand\tikz@td@parse@coord\pgfkeysvalueof{/tikz/3d/incircle/C}}%
%\pgfutil@tmpt
\expanded{\noexpand\tikz@td@parse@coord\pgfkeysvalueof{/tikz/3d/incircle/C}}%
\pgfmathsetmacro{\pgfutil@tmp@Cx}{\pgf@X}%
\pgfmathsetmacro{\pgfutil@tmp@Cy}{\pgf@Y}%
\pgfmathsetmacro{\pgfutil@tmp@Cz}{\pgf@Z}%
\pgfmathsetmacro{\pgfutil@tmpIx}{\pgfutil@tmp@Ax*\pgfutil@tmpa+\pgfutil@tmp@Bx*\pgfutil@tmpb+\pgfutil@tmp@Cx*\pgfutil@tmpc)/\pgfutil@tmpd/2}%
\pgfmathsetmacro{\pgfutil@tmpIy}{\pgfutil@tmp@Ay*\pgfutil@tmpa+\pgfutil@tmp@By*\pgfutil@tmpb+\pgfutil@tmp@Cy*\pgfutil@tmpc)/\pgfutil@tmpd/2}%
\pgfmathsetmacro{\pgfutil@tmpIz}{\pgfutil@tmp@Az*\pgfutil@tmpa+\pgfutil@tmp@Bz*\pgfutil@tmpb+\pgfutil@tmp@Cz*\pgfutil@tmpc)/\pgfutil@tmpd/2}%
\path (\pgfutil@tmpIx,\pgfutil@tmpIy,\pgfutil@tmpIz) 
  coordinate (\pgfkeysvalueof{/tikz/3d/incircle/center name})
  [3d/projection of={(\pgfkeysvalueof{/tikz/3d/incircle/center name}) on 
	\pgfkeysvalueof{/tikz/3d/incircle/A}--\pgfkeysvalueof{/tikz/3d/incircle/B}}] 
 coordinate (\pgfkeysvalueof{/tikz/3d/incircle/projection prefix}c)
 [3d/projection of={(\pgfkeysvalueof{/tikz/3d/incircle/center name}) on 
	\pgfkeysvalueof{/tikz/3d/incircle/A}--\pgfkeysvalueof{/tikz/3d/incircle/C}}] 
 coordinate (\pgfkeysvalueof{/tikz/3d/incircle/projection prefix}b)
 [3d/projection of={(\pgfkeysvalueof{/tikz/3d/incircle/center name}) on 
	\pgfkeysvalueof{/tikz/3d/incircle/B}--\pgfkeysvalueof{/tikz/3d/incircle/C}}] 
 coordinate (\pgfkeysvalueof{/tikz/3d/incircle/projection prefix}a);
 \path[pic actions] pic{3d circle through 3 points={%
   	A={(\pgfkeysvalueof{/tikz/3d/incircle/projection prefix}c)},%
   	B={(\pgfkeysvalueof{/tikz/3d/incircle/projection prefix}b)},%
  	C={(\pgfkeysvalueof{/tikz/3d/incircle/projection prefix}a)},%
  	center name=\pgfkeysvalueof{/tikz/3d/incircle/center name}}}
	;
}},3d/incircle/.cd,
center name/.initial=I,
A/.initial={(1,0,0)},B/.initial={(0,1,0)},C/.initial={(0,0,1)},
projection prefix/.initial=tmpp}
%
\tikzset{pics/3d/circle on sphere/.style={code={%
 \tikzset{3d/circle on sphere/.cd,#1}%
 \edef\pgfutil@tmpR{\pgfkeysvalueof{/tikz/3d/circle on sphere/R}}%
 \edef\pgfutil@tmpC{\pgfkeysvalueof{/tikz/3d/circle on sphere/C}}%
 \edef\pgfutil@tmpP{\pgfkeysvalueof{/tikz/3d/circle on sphere/P}}%
 \edef\pgfutil@tmpn{\pgfkeysvalueof{/tikz/3d/circle on sphere/n}}%
 \edef\pgfutil@tmpPname{\pgfkeysvalueof{/tikz/3d/circle on sphere/auxiliary coordinate prefix}P}%
 \pgfmathsetmacro{\pgfutil@tmpC}{TD("\pgfutil@tmpC")}%
 \pgfmathsetmacro{\pgfutil@tmpP}{TD("\pgfutil@tmpP")}%
 \pgfmathsetmacro{\pgfutil@tmpn}{TD("\pgfutil@tmpn")}%
 \pgfmathsetmacro{\pgfutil@tmpd}{sqrt(TD("(\pgfutil@tmpP)-(\pgfutil@tmpC)o(\pgfutil@tmpP)-(\pgfutil@tmpC)"))}%
 \ifdim\pgfutil@tmpd pt>0.02pt\relax
  % compute a new normal
  \pgfmathsetmacro{\pgfutil@tmpn}{TD("(\pgfutil@tmpP)-(\pgfutil@tmpC)")}%
 \fi
 % normalize the normal
 \pgfmathsetmacro{\pgfutil@tmpa}{sqrt(TD("(\pgfutil@tmpn)o(\pgfutil@tmpn)"))}%
 \ifdim\pgfutil@tmpa pt<0.02pt\relax
  \PackageWarning{3dtools}{Chosen normal is too short.}%    
 \else
 \pgfmathtruncatemacro{\pgfutil@tmpb}{(\pgfutil@tmpd<\pgfutil@tmpR?1:0)} 
 \ifnum\pgfutil@tmpb=0
  \PackageWarning{3dtools}{Circle center is not inside the sphere.}
 \else 
  \pgfmathsetmacro{\pgfutil@tmpr}{sqrt(\pgfutil@tmpR*\pgfutil@tmpR-\pgfutil@tmpd*\pgfutil@tmpd)}%
  \pgfmathsetmacro{\pgfutil@tmpa}{1/\pgfutil@tmpa}%
  \pgfmathsetmacro{\pgfutil@tmpz}{TD("\pgfutil@tmpa*(\pgfutil@tmpn)")}%
  \path[overlay] (nscreenx,nscreeny,nscreenz) coordinate (nscreen)
	[3d coordinate/.expanded={\pgfkeysvalueof{/tikz/3d/aux keys/ez}=(\pgfutil@tmpz)},
	3d coordinate/.expanded={(\pgfutil@tmpPname)=(\pgfutil@tmpP)}];%
  \pgfmathsetmacro{\pgfutil@tmpy}{TD("\pgfkeysvalueof{/tikz/3d/aux keys/ez}x(nscreen)")}%
  \pgfmathsetmacro{\pgfutil@tmpa}{sqrt(TD("(\pgfutil@tmpy)o(\pgfutil@tmpy)"))}%
  \ifdim\pgfutil@tmpa pt<0.04pt%
   %\typeout{(n) is (almost) parallel to normal on screen.}%
   \pgfmathsetmacro{\pgfutil@tmpx}{normalcandidate(\pgfutil@tmpz)}%
   \pgfmathsetmacro{\pgfutil@tmpy}{TD("(\pgfutil@tmpz)x(\pgfutil@tmpx)")}
   \path[overlay] 
	[3d coordinate/.expanded={\pgfkeysvalueof{/tikz/3d/aux keys/ex}=(\pgfutil@tmpx)},
	 3d coordinate/.expanded={\pgfkeysvalueof{/tikz/3d/aux keys/ey}=(\pgfutil@tmpy)}];
   \pgfmathtruncatemacro{\pgfutil@tmpa}{(TD("\pgfkeysvalueof{/tikz/3d/aux keys/ez}o(\pgfutil@tmpn)")<0?0:1)}%   
   \begin{scope}[x/.expanded={\pgfkeysvalueof{/tikz/3d/aux keys/ex}},%
   	y/.expanded={\pgfkeysvalueof{/tikz/3d/aux keys/ey}},%
	z/.expanded={\pgfkeysvalueof{/tikz/3d/aux keys/ez}},%
	shift={(\pgfutil@tmpPname)}]
	\ifcase\pgfutil@tmpa
	 % hidden
	 \begin{pgfonlayer}{\pgfkeysvalueof{/tikz/3d/circle on sphere/back layer}}%
	  \draw[3d/hidden]  circle[radius=\pgfutil@tmpr];
	 \end{pgfonlayer}%
	\or
	 % visible
	 \begin{pgfonlayer}{\pgfkeysvalueof{/tikz/3d/circle on sphere/fore layer}}%
	  \draw[3d/visible] circle[radius=\pgfutil@tmpr];
	 \end{pgfonlayer}% 
	\fi
   \end{scope}
  \else% normal not collinear with n_screen 
   \pgfmathsetmacro{\pgfutil@tmpa}{1/\pgfutil@tmpa}%
   \pgfmathsetmacro{\pgfutil@tmpy}{TD("\pgfutil@tmpa*(\pgfutil@tmpy)")}%
   \pgfmathsetmacro{\pgfutil@tmpx}{TD("(\pgfutil@tmpy)x(\pgfutil@tmpz)")}%
   \pgfmathsetmacro{\pgfutil@tmps}{TD("(nscreen)")}%
   \pgfmathsetmacro{\pgfutil@tmpp}{TD("\pgfkeysvalueof{/tikz/3d/aux keys/ez}o(nscreen)")}%
   \pgfmathsetmacro{\pgfutil@tmpo}{sqrt(1-\pgfutil@tmpp*\pgfutil@tmpp)}%
   \pgfmathsetmacro{\pgfutil@tmpa}{atan2(-1*\pgfutil@tmpp,\pgfutil@tmpo)}%
   \pgfmathsetmacro{\pgfutil@tmpb}{screendepth(\pgfutil@tmpP)}%
   \pgfmathsetmacro{\pgfutil@tmpc}{screendepth(\pgfutil@tmpC)}%
   \path[overlay,
		3d coordinate/.expanded={\pgfkeysvalueof{/tikz/3d/aux keys/ex}=(\pgfutil@tmpx)},
		3d coordinate/.expanded={\pgfkeysvalueof{/tikz/3d/aux keys/ey}=(\pgfutil@tmpy)}];%
%    \typeout{\pgfkeysvalueof{/tikz/3d/aux keys/ex}=(\pgfutil@tmpx), 
%    	\pgfkeysvalueof{/tikz/3d/aux keys/ey}=(\pgfutil@tmpy), 
% 	\pgfkeysvalueof{/tikz/3d/aux keys/ez}=(\pgfutil@tmpz), n_screen=(\pgfutil@tmps)}%
   \begin{scope}[x/.expanded={\pgfkeysvalueof{/tikz/3d/aux keys/ex}},%
   	 y/.expanded={\pgfkeysvalueof{/tikz/3d/aux keys/ey}},%
	 z/.expanded={\pgfkeysvalueof{/tikz/3d/aux keys/ez}},%
	 shift={(\pgfutil@tmpPname)}]  
    \pgfmathtruncatemacro{\pgfutil@tmpi}{(abs(\pgfutil@tmpr*cos(\pgfutil@tmpa))>abs(\pgfutil@tmpb-\pgfutil@tmpc)?1:0)}% 
 	\ifcase\pgfutil@tmpi
% 	  % only visible or only hidden
 	 \pgfmathtruncatemacro{\pgfutil@tmpj}{(\pgfutil@tmpb<\pgfutil@tmpc?0:1)}%
 	 \ifcase\pgfutil@tmpj
% 	   % hidden
      \begin{pgfonlayer}{\pgfkeysvalueof{/tikz/3d/circle on sphere/back layer}}%
 	   \draw[3d/hidden]  circle[radius=\pgfutil@tmpr];
	  \end{pgfonlayer}%	
 	 \or
% 	   % visible
	  \begin{pgfonlayer}{\pgfkeysvalueof{/tikz/3d/circle on sphere/fore layer}}%
 	   \draw[3d/visible]  circle[radius=\pgfutil@tmpr];
	  \end{pgfonlayer}%	
 	 \fi
 	\or
% 	  % mixed
	 \pgfmathsetmacro{\pgfutil@tmpf}{abs(acos((\pgfutil@tmpc-\pgfutil@tmpb)/\pgfutil@tmpr/cos(\pgfutil@tmpa))}%
	 \begin{pgfonlayer}{\pgfkeysvalueof{/tikz/3d/circle on sphere/back layer}}%
	  \draw[3d/hidden]  (\pgfutil@tmpf:\pgfutil@tmpr) arc[start angle=\pgfutil@tmpf,
	 	end angle=360-\pgfutil@tmpf,radius=\pgfutil@tmpr];
     \end{pgfonlayer}%
	 \begin{pgfonlayer}{\pgfkeysvalueof{/tikz/3d/circle on sphere/fore layer}}%
	  \draw[3d/visible]  (\pgfutil@tmpf:\pgfutil@tmpr) arc[start angle=\pgfutil@tmpf,
	 	end angle=-\pgfutil@tmpf,radius=\pgfutil@tmpr];
	 \end{pgfonlayer}%	
 	\fi
   \end{scope}
   \fi	
  \fi
 \fi  
}},3d/circle on sphere/.cd,C/.initial={(0,0,0)},
	P/.initial={(0,0,0)},R/.initial=1,%
	n/.initial={(0,0,1)},auxiliary coordinate prefix/.initial=tmp,%
	fore layer/.initial=main,back layer/.initial=main}
%
\tikzset{pics/3d/cone/.style={code={%
	\tikzset{3d/.cd,#1}%
	\def\pv##1{\pgfkeysvalueof{/tikz/3d/##1}}%
	\pgfmathsetmacro{\sdtip}{screendepth(0,0,\pv{h})}
	\pgfmathsetmacro{\aspectangle}{atan2(\sdtip,sqrt(\pv{h}*\pv{h}-\sdtip*\sdtip))}
	\path (0,0,\pv{h}) coordinate (-tip);
	\pgfmathsetmacro{\myey}{TDunit("(0,0,1)x(nscreenx,nscreeny,nscreenz)")}%
	\path (0,0,{tan(\aspectangle)}) coordinate (-tmpex)
		(\myey) coordinate (-tmpey);	
    \begin{scope}[x={(-tmpex)},y={(-tmpey)}]
	 \pgfmathtruncatemacro{\itest}{abs(tan(\aspectangle)*\pv{r}/\pv{h})<1}
	 \ifnum\itest=1
	  \pgfmathsetmacro{\alphacrit}{acos(tan(\aspectangle)*\pv{r}/\pv{h})}
	  \ifdim\sdtip pt>0pt
	   \path[/tikz/3d/hidden] (\alphacrit:\pv{r}) arc[start angle=\alphacrit,end
	   angle=-\alphacrit,radius=\pv{r}];
	   \path[/tikz/3d/visible,/tikz/3d/cone/outer] (\alphacrit:\pv{r}) 
	   arc[start angle=\alphacrit,end  angle=360-\alphacrit,radius=\pv{r}]
	   -- (-tip) -- cycle;
	  \else
	   \path[/tikz/3d/visible,/tikz/3d/cone/inner] (0,0) circle[radius=\pv{r}];
	   \path[/tikz/3d/visible,/tikz/3d/cone/outer] (\alphacrit:\pv{r}) 
	   arc[start angle=\alphacrit,end  angle=-\alphacrit,radius=\pv{r}]
	   -- (-tip) -- cycle;
	  \fi
	 \else
	  \path[/tikz/3d/visible] circle[radius=\pv{r}];	 
	 \fi
    \end{scope}
	}},3d/cone/.cd,outer/.style={},inner/.style={}}
%%
\tikzset{pics/3d/shaded cone/.style={code={%
	\tikzset{3d/.cd,#1}%
	\def\pv##1{\pgfkeysvalueof{/tikz/3d/##1}}%
	\pgfmathsetmacro{\sdtip}{screendepth(0,0,\pv{h})}
	\pgfmathsetmacro{\aspectangle}{atan2(\sdtip,sqrt(\pv{h}*\pv{h}-\sdtip*\sdtip))}
	\path (0,0,0) coordinate (-base) (0,0,\pv{h}) coordinate (-tip);
    \begin{scope}[x={(0,0,tan(\aspectangle))},y={($(0,0,0)!1cm!90:(0,0,\pv{h})$)}]
	 \pgfmathtruncatemacro{\itest}{abs(tan(\aspectangle)*\pv{r}/\pv{h})<1}
	 % zero means tip inside projection of the base
	 \ifnum\itest=1
	  \pgfmathsetmacro{\alphacrit}{acos(tan(\aspectangle)*\pv{r}/\pv{h})}
   	  \pgfmathtruncatemacro{\itest}{y2d("-tip")>y2d("-base")?1:0}
      \ifnum\itest=1 
	   \pgfmathsetmacro{\alphacritB}{-\alphacrit}
	   \pgfmathsetmacro{\alphacritC}{360-\alphacrit}
	  \else
	   \pgfmathsetmacro{\alphacritB}{360-\alphacrit}
	   \pgfmathsetmacro{\alphacritC}{-\alphacrit}
	  \fi
	  %\typeout{\sdtip,\itest,\alphacrit,\alphacritB,\alphacritC}
	  \ifdim\sdtip pt>0pt
	   \begin{scope}
	    \clip (\alphacrit:\pv{r}) 
	     arc[start angle=\alphacrit,end  angle=\alphacritC,radius=\pv{r}]
	     -- (-tip) -- cycle;
	    \path[3d/cone/outer shade,3d/screen coords]	
		 (-tip) circle[radius={abs(\pv{r})+abs(\pv{h})}];
	   \end{scope}
	   \path[/tikz/3d/hidden] (\alphacrit:\pv{r}) arc[start angle=\alphacrit,end
	    angle=\alphacritB,radius=\pv{r}];
	   \path[/tikz/3d/visible] (\alphacrit:\pv{r}) 
	    arc[start angle=\alphacrit,end  angle=\alphacritC,radius=\pv{r}]
	    -- (-tip) -- cycle;
	  \else
	   \begin{scope}
	    \clip (0,0) circle[radius=\pv{r}];
	    \path[3d/cone/inner shade,3d/screen coords]	
		 (-tip) circle[radius={abs(\pv{r})+abs(\pv{h})}];
	   \end{scope}
	   \path[/tikz/3d/visible,/tikz/3d/cone/inner] (0,0) circle[radius=\pv{r}];
	   \begin{scope}
	    \clip (\alphacrit:\pv{r}) 
	     arc[start angle=\alphacrit,end  angle=\alphacritB,radius=\pv{r}]
	    -- (-tip) -- cycle;
	    \path[3d/cone/outer shade,3d/screen coords]	
		 (-tip) circle[radius={abs(\pv{r})+abs(\pv{h})}];
	   \end{scope}
	   \path[/tikz/3d/visible,/tikz/3d/cone/outer] (\alphacrit:\pv{r}) 
	    arc[start angle=\alphacrit,end  angle=\alphacritB,radius=\pv{r}]
	    -- (-tip) -- cycle;
	  \fi
	 \else
      \ifdim\sdtip pt>0pt
	   \begin{scope}
		\clip (0,0) circle[radius=\pv{r}];	 
	     \path[3d/cone/outer shade,3d/screen coords]	
		  (-tip) circle[radius={abs(\pv{r})+abs(\pv{h})}];
	   \end{scope}
	  \else
	   \begin{scope}
		\clip (0,0) circle[radius=\pv{r}];	 
	     \path[3d/cone/inner shade,3d/screen coords]	
		  (-tip) circle[radius={abs(\pv{r})+abs(\pv{h})}];
	   \end{scope}
	  \fi
	  \path[/tikz/3d/visible] circle[radius=\pv{r}];	 
	 \fi
    \end{scope}
	}},3d/cone/.cd,outer shade/.style={3d/cone shading},
	inner shade/.style={3d/cone shading={brightness=0.3}}}	
%%
\tikzset{pics/3d/frustum/.style={code={%
  \tikzset{3d/.cd,#1}
  \def\pv##1{\pgfkeysvalueof{/tikz/3d/##1}}%
  \pgfmathtruncatemacro{\itest}{abs(\pv{R}-\pv{r})>0.02}
  \ifnum\itest=0
   %\PackageWarning{3dtools}{Radii R=\pv{R} and r=\pv{r} are too close.}%
   \path[overlay] (0,0,0) coordinate (-tdtmpo)
	(0,0,\pv{h}) coordinate (-tdtmpez)
	($(0,0,0)!1cm!90:(0,0,\pv{h})$) coordinate (-tdtmpey);
   \pgfmathsetmacro{\mytest}{y2d("-tdtmpez")}	
   \pgfmathsetmacro@td@FPU{\pgfutil@tmpa}{sqrt(pow(x2d("-tdtmpo")-x2d("-tdtmpez"),2)+pow(y2d("-tdtmpo")-y2d("-tdtmpez"),2))}%
   \pgfmathtruncatemacro{\itest}{(\pgfutil@tmpa>0.5?1:0)}%
   \ifnum\itest=0
	\draw[3d/visible] (0,0,0) circle[radius=R];
   \else
    \pgfmathtruncatemacro{\itest}{sign(screendepth(0,0,\pv{h}))+1}%
	\pgfmathsetmacro{\sdtip}{screendepth(0,0,\pv{h})}%
	\pgfmathsetmacro{\aspectangle}{atan2(\sdtip,\pgfutil@tmpa/1cm)}%
	\path[overlay] (0,0,{tan(\aspectangle)}) coordinate (-tdtmpex);
	\begin{scope}[x={(-tdtmpex)},y={(-tdtmpey)}]
	 \ifcase\itest\relax
      % "lower" circle visible
	  \draw[3d/hidden] (-tdtmpez)+(0,\pv{r})
	  	arc[start angle=90,end angle=-90,radius=\pv{r}];
	  \draw[3d/visible]  (0,\pv{R}) 
	   -- ($(-tdtmpez)+(0,\pv{r})$) 
	   arc[start angle=90,end angle=270,radius=\pv{r}]
	   -- (0,-\pv{R})
	   (0,0) circle[radius=\pv{R}];
	 \or
      % no circle visible
	  \draw[3d/visible]  (0,\pv{R}) 
	   -- ($(-tdtmpez)+(0,\pv{r})$) 
	   -- ($(-tdtmpez)+(0,-\pv{r})$) -- (0,-\pv{R}) -- cycle;
	 \or
      % "upper" circle visible
	  \draw[3d/hidden] (0,\pv{R})
	  	arc[start angle=90,end angle=-90,radius=\pv{R}];
	  \draw[3d/visible] (-tdtmpez)+ (0,\pv{r}) 
	   -- (0,\pv{R})
	   arc[start angle=90,end angle=270,radius=\pv{R}]
	   -- ($(-tdtmpez)+(0,-\pv{r})$) 
	   (-tdtmpez) circle[radius=\pv{r}];
	 \fi
	\end{scope} 
   \fi
  \else
   \pgfmathsetmacro{\myH}{(\pv{R}*\pv{h}/(\pv{R}-\pv{r}))}%
   \pgfmathsetmacro{\sdtip}{screendepth(0,0,\myH)}%
   \pgfmathsetmacro{\aspectangle}{atan2(\sdtip,sqrt(\myH*\myH-\sdtip*\sdtip))}%
   %\typeout{H=\myH,angle=\aspectangle}
   \path[overlay] (0,0,\myH) coordinate (-tip)
   (0,0,\pv{h}) coordinate (-upper base)
   (0,0,{tan(\aspectangle)}) coordinate (-tdtmpex)
   ($(0,0,0)!1cm!90:(0,0,\pv{h})$) coordinate (-tdtmpey);
   \begin{scope}[x={(-tdtmpex)},y={(-tdtmpey)}]
	   \pgfmathtruncatemacro{\itest}{abs(tan(\aspectangle)*\pv{R}/\myH)<1}
	   \path[local bounding box=pft] (-upper base) circle[radius=\pv{r}]
	    (0,0,0) circle[radius=\pv{R}];
	   \ifnum\itest=1
		\pgfmathsetmacro{\alphacrit}{acos(tan(\aspectangle)*\pv{R}/\myH)}
		\ifdim\sdtip pt>0pt\relax
		 \begin{scope}
		  \clip (-upper base) circle[radius=\pv{r}] ;
		  \path[/tikz/3d/hidden] (\alphacrit:\pv{R}) arc[start angle=\alphacrit,end
		  angle=-\alphacrit,radius=\pv{R}];
		  \path[/tikz/3d/hidden] ($(-upper base)+(\alphacrit:\pv{r})$)
		  --(\alphacrit:\pv{R}) 
		  arc[start angle=\alphacrit,end  angle=360-\alphacrit,radius=\pv{R}]
		  -- ($(-upper base)+(360-\alphacrit:\pv{r})$);
		 \end{scope}
		 \begin{scope}
		  \clip[even odd clip] (-upper base) circle[radius=\pv{r}]  [generous outside path];
		  \path[/tikz/3d/hidden] (\alphacrit:\pv{R}) arc[start angle=\alphacrit,end
		  angle=-\alphacrit,radius=\pv{R}];
		  \path[/tikz/3d/visible] ($(-upper base)+(\alphacrit:\pv{r})$)
		  --(\alphacrit:\pv{R}) 
		  arc[start angle=\alphacrit,end  angle=360-\alphacrit,radius=\pv{R}]
		  -- ($(-upper base)+(360-\alphacrit:\pv{r})$);
		 \end{scope}
		 \path[/tikz/3d/visible] (-upper base) circle[radius=\pv{r}];
		\else %\typeout{\sdtip<0}
		 \begin{scope}
		  \clip circle[radius=\pv{R}];
		  \path[/tikz/3d/hidden] ($(-upper base)+(\alphacrit:\pv{r})$)
		  --(\alphacrit:\pv{R}) 
		  ($(-upper base)+(360-\alphacrit:\pv{r})$)
		  --(360-\alphacrit:\pv{R});
		  \path[/tikz/3d/hidden] (-upper base) circle[radius=\pv{r}];
		 \end{scope}
% 		 % enlarge the bounding box
% 		 \path ($(-upper base)+(\alphacrit:\pv{r})$)
% 		 --(\alphacrit:\pv{R}) 
% 		 ($(-upper base)+(360-\alphacrit:\pv{r})$)
% 		 --(360-\alphacrit:\pv{R});
% 		 \path (-upper base) circle[radius=\pv{r}];
		 \begin{scope}
 		  \clip[even odd clip] circle[radius=\pv{R}] [generous outside path];
		  \path[/tikz/3d/hidden]  ($(-upper base)+(\alphacrit:\pv{r})$)
		  arc[start angle=\alphacrit,end  angle=-\alphacrit,radius=\pv{r}];
		  \path[/tikz/3d/visible] (\alphacrit:\pv{R}) --
		  ($(-upper base)+(\alphacrit:\pv{r})$)
		  arc[start angle=\alphacrit,end  angle=360-\alphacrit,radius=\pv{r}]
		  --(360-\alphacrit:\pv{R});
		 \end{scope}
		 \path[/tikz/3d/visible] circle[radius=\pv{R}];
		\fi
	   \else
		\path[/tikz/3d/visible] circle[radius=\pv{R}];	 
		\path[/tikz/3d/hidden] (-upper base) circle[radius=\pv{r}];
	   \fi
   \end{scope}
  \fi
}}}
%		
\pgfmathdeclarefunction{tddistance}{2}{%
\begingroup%
\pgfmathparse@td@FPU{sqrt(TD("#1-#2o#1-#2"))}%
\pgfmathsmuggle\pgfmathresult\endgroup%
}%
% intersection of three spheres (see https://stackoverflow.com/a/18654302)
% 
%     temp1 = P2-P1                                        
%     e_x = temp1/norm(temp1)                              
%     temp2 = P3-P1                                        
%     i = dot(e_x,temp2)                                   
%     temp3 = temp2 - i*e_x                                
%     e_y = temp3/norm(temp3)                              
%     e_z = cross(e_x,e_y)                                 
%     d = norm(P2-P1)                                      
%     j = dot(e_y,temp2)                                   
%     x = (r1*r1 - r2*r2 + d*d) / (2*d)                    
%     y = (r1*r1 - r3*r3 -2*i*x + i*i + j*j) / (2*j)       
%     temp4 = r1*r1 - x*x - y*y                            
%     if temp4<0:                                          
%         raise Exception("The three spheres do not intersect!");
%     z = sqrt(temp4)                                      
%     p_12_a = P1 + x*e_x + y*e_y + z*e_z                  
%     p_12_b = P1 + x*e_x + y*e_y - z*e_z                  
%     return p_12_a,p_12_b                       
\tikzset{3d/.cd,intersection of three spheres/.code={%
\tikzset{3d/aux keys/.cd,#1,/tikz/3d/define orthonormal dreibein}%
\pgfmathsetmacro\pgfutil@tmpA{TD("\pgfkeysvalueof{/tikz/3d/aux keys/A}")}%
\pgfmathsetmacro\pgfutil@tmpB{TD("\pgfkeysvalueof{/tikz/3d/aux keys/B}")}%
\pgfmathsetmacro\pgfutil@tmpC{TD("\pgfkeysvalueof{/tikz/3d/aux keys/C}")}%
\pgfmathsetmacro\pgfutil@tmpex{TD("\pgfkeysvalueof{/tikz/3d/aux keys/ex}")}%
\pgfmathsetmacro\pgfutil@tmpey{TD("\pgfkeysvalueof{/tikz/3d/aux keys/ey}")}%
\pgfmathsetmacro\pgfutil@tmpez{TD("\pgfkeysvalueof{/tikz/3d/aux keys/ez}")}%
\pgfmathsetmacro\pgfutil@tmpAB{TD("(\pgfutil@tmpB)-(\pgfutil@tmpA)")}%
\pgfmathsetmacro\pgfutil@tmpd{sqrt(TD("(\pgfutil@tmpAB)o(\pgfutil@tmpAB)"))}%
\ifdim\pgfutil@tmpd pt<0.1pt\relax
\PackageWarning{3dtools}{Points \pgfkeysvalueof{/tikz/3d/aux keys/A} and \pgfkeysvalueof{/tikz/3d/aux keys/B} are too close to each other.}%
\else
\pgfmathsetmacro\pgfutil@tmpAC{TD("(\pgfutil@tmpC)-(\pgfutil@tmpA)")}% temp2
%     i = dot(e_x,temp2)                                   
\pgfmathsetmacro\pgfutil@tmpi{TD("(\pgfutil@tmpex)o(\pgfutil@tmpAC)")}%
%     j = dot(e_y,temp2)                                   
\pgfmathsetmacro\pgfutil@tmpj{TD("(\pgfutil@tmpey)o(\pgfutil@tmpAC)")}%
\edef\pgfutil@tmprA{\pgfkeysvalueof{/tikz/3d/aux keys/rA}}%
\edef\pgfutil@tmprB{\pgfkeysvalueof{/tikz/3d/aux keys/rB}}%
\edef\pgfutil@tmprC{\pgfkeysvalueof{/tikz/3d/aux keys/rC}}%
%     x = (r1*r1 - r2*r2 + d*d) / (2*d)                    
\pgfmathsetmacro\pgfutil@tmpx{(pow(\pgfutil@tmprA,2)-pow(\pgfutil@tmprB,2)%
+pow(\pgfutil@tmpd,2))/(2*(\pgfutil@tmpd))}%
%     y = (r1*r1 - r3*r3 -2*i*x + i*i + j*j) / (2*j)       
\pgfmathsetmacro\pgfutil@tmpy{(\pgfutil@tmprA*\pgfutil@tmprA-\pgfutil@tmprC*\pgfutil@tmprC%
-2*(\pgfutil@tmpi)*(\pgfutil@tmpx)+(\pgfutil@tmpi)*(\pgfutil@tmpi)%
+(\pgfutil@tmpj)*(\pgfutil@tmpj))/(2*(\pgfutil@tmpj))}%
%     temp4 = r1*r1 - x*x - y*y                            
\pgfmathsetmacro\pgfutil@tmpc{\pgfutil@tmprA*\pgfutil@tmprA-pow(\pgfutil@tmpx,2)-pow(\pgfutil@tmpy,2)}%
\ifdim\pgfutil@tmpc pt<0pt\relax
\PackageWarning{3dtools}{Not all spheres intersect.}%
\else
\pgfmathsetmacro\pgfutil@tmpz{sqrt(\pgfutil@tmpc)}%
\pgfmathsetmacro\pgfutil@tmpd{TD("(\pgfutil@tmpA)+\pgfutil@tmpx*(\pgfutil@tmpex)%
+\pgfutil@tmpy*(\pgfutil@tmpey)+\pgfutil@tmpz*(\pgfutil@tmpez)")}%
\pgfmathsetmacro\pgfutil@tmpe{TD("(\pgfutil@tmpA)+\pgfutil@tmpx*(\pgfutil@tmpex)%
+\pgfutil@tmpy*(\pgfutil@tmpey)-\pgfutil@tmpz*(\pgfutil@tmpez)")}%
\tikzset{insert path={%
(\pgfutil@tmpd) coordinate(\pgfkeysvalueof{/tikz/3d/aux keys/i1}) 
(\pgfutil@tmpe) coordinate(\pgfkeysvalueof{/tikz/3d/aux keys/i2}) 
}}
\fi
\fi
}}%
%
\tikzset{3d/insphere center/.code={%
 \tikzset{3d/insphere/.cd,#1}%
 \pgfmathsetmacro{\pgfutil@tmpA}{TD("\pgfkeysvalueof{/tikz/3d/insphere/B}x\pgfkeysvalueof{/tikz/3d/insphere/C}")}%
 \pgfmathsetmacro{\pgfutil@tmpA}{sqrt(TD("(\pgfutil@tmpA)o(\pgfutil@tmpA)"))/2}%
 \pgfmathsetmacro{\pgfutil@tmpB}{TD("\pgfkeysvalueof{/tikz/3d/insphere/A}x\pgfkeysvalueof{/tikz/3d/insphere/C}")}%
 \pgfmathsetmacro{\pgfutil@tmpB}{sqrt(TD("(\pgfutil@tmpB)o(\pgfutil@tmpB)"))/2}%
 \pgfmathsetmacro{\pgfutil@tmpC}{TD("\pgfkeysvalueof{/tikz/3d/insphere/A}x\pgfkeysvalueof{/tikz/3d/insphere/B}")}%
 \pgfmathsetmacro{\pgfutil@tmpC}{sqrt(TD("(\pgfutil@tmpC)o(\pgfutil@tmpC)"))/2}%
 \pgfmathsetmacro{\pgfutil@tmpD}{TD("\pgfkeysvalueof{/tikz/3d/insphere/A}-\pgfkeysvalueof{/tikz/3d/insphere/B}x\pgfkeysvalueof{/tikz/3d/insphere/C}-\pgfkeysvalueof{/tikz/3d/insphere/B}")}%
 \pgfmathsetmacro{\pgfutil@tmpD}{sqrt(TD("(\pgfutil@tmpD)o(\pgfutil@tmpD)"))/2}%
 \pgfmathsetmacro{\pgfutil@tmps}{\pgfutil@tmpA+\pgfutil@tmpB+\pgfutil@tmpC+\pgfutil@tmpD}%
 \pgfmathsetmacro{\pgfutil@tmpA}{\pgfutil@tmpA/\pgfutil@tmps}%
 \pgfmathsetmacro{\pgfutil@tmpB}{\pgfutil@tmpB/\pgfutil@tmps}%
 \pgfmathsetmacro{\pgfutil@tmpC}{\pgfutil@tmpC/\pgfutil@tmps}%
 \pgfmathsetmacro{\pgfutil@tmpD}{\pgfutil@tmpD/\pgfutil@tmps}%
 \pgfmathsetmacro{\pgfutil@tmpI}{TD("\pgfutil@tmpA*\pgfkeysvalueof{/tikz/3d/insphere/A}+\pgfutil@tmpB*\pgfkeysvalueof{/tikz/3d/insphere/B}+\pgfutil@tmpC*\pgfkeysvalueof{/tikz/3d/insphere/C}+\pgfutil@tmpD*\pgfkeysvalueof{/tikz/3d/insphere/D}")}%
 \tikzset{insert path={(\pgfutil@tmpI)}}
},3d/insphere/.cd,A/.initial={(A)},B/.initial={(B)},
C/.initial={(C)},D/.initial={(D)}}%
%
\newif\if@tikz@td@complete@dashes
\@tikz@td@complete@dashesfalse
\tikzset{cheating dash/.code args={on #1 off #2}{% from https://tex.stackexchange.com/a/133357
        % Use csname so catcode of @ doesn't have do be changed.		
        \tikz@addoption{%
            \pgfgetpath\pgfutil@tmpc%
            \pgfprocessround{\pgfutil@tmpc}{\pgfutil@tmpc}%
            \pgf@decorate@parsesoftpath{\pgfutil@tmpc}{\pgfutil@tmpc}%
            \pgfmathsetmacro{\pgfutil@tmpa}{\pgf@decorate@totalpathlength-#1}%\let\rest=\pgfmathresult%
            \pgfmathsetmacro{\pgfutil@tmpb}{#1+#2}%\let\onoff=\pgfmathresult%
            \pgfmathsetmacro{\pgfutil@tmpd}{max(floor(\pgfutil@tmpa/\pgfutil@tmpb), 1)}%\let\nfullonoff=\pgfmathresult%
            \pgfmathsetmacro{\pgfutil@tmpe}{max((\pgfutil@tmpa-\pgfutil@tmpb*\pgfutil@tmpd)/\pgfutil@tmpd+#2,#2)}%\let\offexpand=\pgfmathresult%
            \pgfsetdash{{#1}{\pgfutil@tmpe}}{0pt}}%
    },cheating dash/.default={on 2pt off 2pt}}%
\tikzset{3d/.cd,% 
reset vertex counter/.code={\c@pgf@counta0\relax},
add vertex/.code={\advance\c@pgf@counta by1\relax
\path (#1) coordinate (\the\c@pgf@counta);},
define vertices/.code={\c@pgf@counta0\relax
\tikzset{3d/add vertex/.list={#1}}},%
append vertices/.code={\tikzset{3d/add vertex/.list={#1}}},%
}	
\tikzset{3d/.cd,polyhedron/.cd,
face edges/.style={},
edges have complete dashes/.is if=@tikz@td@complete@dashes,
edges have complete dashes/.default=true,
complete dashes/.code args={on #1 off #2}{\tikzset{%
/tikz/3d/polyhedron/edges have complete dashes=true,
/tikz/3d/polyhedron/face edges/.append style={cheating dash=on #1 off #2}}},
complete dashes/.default={on 2pt off 2pt},
draw face with corners/.code={\begingroup\c@pgf@counta0\relax
\pgfutil@for\pgfutil@tmpa:={#1}\do{%
\pgfmathsetmacro\pgfutil@tmpT{TD("\pgfutil@tmpa")}%
\ifcase\c@pgf@counta 
\pgfmathsetmacro\pgfutil@tmpA{TD("\pgfutil@tmpa")}%
\or
\pgfmathsetmacro\pgfutil@tmpB{TD("\pgfutil@tmpa")}%
\or
\pgfmathsetmacro\pgfutil@tmpC{TD("\pgfutil@tmpa")}%
\fi
\advance\c@pgf@counta by1\relax
\ifnum\c@pgf@counta=1\relax
\edef\pgfutil@tmpl{(\pgfutil@tmpT)}% regular list
\edef\pgfutil@tmplf{(\pgfutil@tmpT)}% first
\edef\pgfutil@tmple{(\pgfutil@tmpT)}% edge list
\else
\edef\pgfutil@tmpl{\pgfutil@tmpl -- (\pgfutil@tmpT)}%
\edef\pgfutil@tmple{\pgfutil@tmple\space edge (\pgfutil@tmpT)
(\pgfutil@tmpT)}%
\fi
}%
\ifnum\c@pgf@counta<3\relax
\PackageWarning{3dtools}{A face needs at least three vertices. However, only \the\c@pgf@counta\space vertices were specified.}%
\else
\edef\pgfutil@tmpO{\pgfkeysvalueof{/tikz/3d/polyhedron/O}}%
\pgfmathsetmacro\pgfutil@tmpO{TD("\pgfutil@tmpO")}%
\edef\pgfutil@tmpL{\pgfkeysvalueof{/tikz/3d/polyhedron/L}}%
\pgfmathsetmacro\pgfutil@tmpL{TD("\pgfutil@tmpL")}%
\pgfmathsetmacro{\pgfutil@tmpb}{TD("(\pgfutil@tmpB)-(\pgfutil@tmpA)x(\pgfutil@tmpC)-(\pgfutil@tmpA)")}% 
\pgfmathsetmacro{\pgfutil@tmpc}{TD("(\pgfutil@tmpA)-(\pgfutil@tmpO)")}% 
\pgfmathtruncatemacro{\pgfutil@tmpd}{sign(TD("(\pgfutil@tmpb)o(\pgfutil@tmpc)"))}%
\ifnum\pgfutil@tmpd=-1\relax
\pgfmathsetmacro{\pgfutil@tmpb}{TD("(\pgfutil@tmpB)-(\pgfutil@tmpA)x(\pgfutil@tmpA)-(\pgfutil@tmpC)")}% 
\fi
\pgfmathsetmacro{\pgfutil@tmpe}{screendepth(\pgfutil@tmpb)}%
\pgfmathsetmacro{\pgfutil@tmpf}{sqrt(TD("(\pgfutil@tmpb)o(\pgfutil@tmpb)"))}%
\pgfmathsetmacro{\pgfutil@tmpg}{sqrt(TD("(\pgfutil@tmpL)o(\pgfutil@tmpL)"))}%
\pgfmathsetmacro{\pgfutil@tmph}{TD("(\pgfutil@tmpL)o(\pgfutil@tmpb)")/\pgfutil@tmpf/\pgfutil@tmpg}%
\pgfmathtruncatemacro{\pgfutil@tmpi}{70+30*\pgfutil@tmph}%
\pgfmathtruncatemacro{\pgfutil@tmpi}{\pgfkeysvalueof{/tikz/3d/polyhedron/shading function}(\pgfutil@tmph)}%
\ifdim\pgfutil@tmpe pt<0pt\relax
\begin{pgfonlayer}{\pgfkeysvalueof{/tikz/3d/polyhedron/back layer}}
\tikzset{3d/polyhedron/before hidden,3d/polyhedron/back}%
\if@tikz@td@complete@dashes
\path[fill=tikz@td@face@color!\pgfutil@tmpi!black,3d/polyhedron/back,draw=none] 
	\pgfutil@tmpl -- cycle;
\edef\pgfutil@tmplg{\pgfutil@tmple\space edge \pgfutil@tmplf}%
\draw[3d/polyhedron/back,every edge/.append style={/tikz/3d/polyhedron/face edges}]
	\pgfutil@tmplg;
\else
\draw[fill=tikz@td@face@color!\pgfutil@tmpi!black,3d/polyhedron/back] \pgfutil@tmpl -- cycle;
\fi
\tikzset{3d/polyhedron/after hidden}%
\end{pgfonlayer}
\else
\begin{pgfonlayer}{\pgfkeysvalueof{/tikz/3d/polyhedron/fore layer}}
\tikzset{3d/polyhedron/before visible,3d/polyhedron/fore}%
\if@tikz@td@complete@dashes
\path[fill=tikz@td@face@color!\pgfutil@tmpi!black,3d/polyhedron/fore,draw=none]
 \pgfutil@tmpl -- cycle;
\edef\pgfutil@tmplg{\pgfutil@tmple\space edge \pgfutil@tmplf}%
\draw[3d/polyhedron/fore,every edge/.append style={/tikz/3d/polyhedron/face edges}]
	\pgfutil@tmplg;
\else
\draw[fill=tikz@td@face@color!\pgfutil@tmpi!black,3d/polyhedron/fore] \pgfutil@tmpl -- cycle;
\fi
\tikzset{3d/polyhedron/after visible}%
\end{pgfonlayer}
\fi
\fi
\endgroup
},
draw open face with corners/.code={\begingroup\c@pgf@counta0\relax
\pgfutil@for\pgfutil@tmpa:={#1}\do{%
\pgfmathsetmacro\pgfutil@tmpT{TD("\pgfutil@tmpa")}%
\ifcase\c@pgf@counta 
\pgfmathsetmacro\pgfutil@tmpA{TD("\pgfutil@tmpa")}%
\or
\pgfmathsetmacro\pgfutil@tmpB{TD("\pgfutil@tmpa")}%
\or
\pgfmathsetmacro\pgfutil@tmpC{TD("\pgfutil@tmpa")}%
\fi
\advance\c@pgf@counta by1\relax
\ifnum\c@pgf@counta=1\relax
\edef\pgfutil@tmpl{(\pgfutil@tmpT)}% regular list
\edef\pgfutil@tmplf{(\pgfutil@tmpT)}% first
\edef\pgfutil@tmple{(\pgfutil@tmpT)}% edge list
\else
\edef\pgfutil@tmpl{\pgfutil@tmpl -- (\pgfutil@tmpT)}%
\edef\pgfutil@tmple{\pgfutil@tmple\space edge (\pgfutil@tmpT)
(\pgfutil@tmpT)}%
\fi
}%
\ifnum\c@pgf@counta<3\relax
\PackageWarning{3dtools}{A face needs at least three vertices. However, only \the\c@pgf@counta\space vertices were specified.}%
\else
\edef\pgfutil@tmpO{\pgfkeysvalueof{/tikz/3d/polyhedron/O}}%
\pgfmathsetmacro\pgfutil@tmpO{TD("\pgfutil@tmpO")}%
\edef\pgfutil@tmpL{\pgfkeysvalueof{/tikz/3d/polyhedron/L}}%
\pgfmathsetmacro\pgfutil@tmpL{TD("\pgfutil@tmpL")}%
\pgfmathsetmacro{\pgfutil@tmpb}{TD("(\pgfutil@tmpB)-(\pgfutil@tmpA)x(\pgfutil@tmpC)-(\pgfutil@tmpA)")}% 
\pgfmathsetmacro{\pgfutil@tmpc}{TD("(\pgfutil@tmpA)-(\pgfutil@tmpO)")}% 
\pgfmathtruncatemacro{\pgfutil@tmpd}{sign(TD("(\pgfutil@tmpb)o(\pgfutil@tmpc)"))}%
\ifnum\pgfutil@tmpd=-1\relax
\pgfmathsetmacro{\pgfutil@tmpb}{TD("(\pgfutil@tmpB)-(\pgfutil@tmpA)x(\pgfutil@tmpA)-(\pgfutil@tmpC)")}% 
\fi
\pgfmathsetmacro{\pgfutil@tmpe}{screendepth(\pgfutil@tmpb)}%
\pgfmathsetmacro{\pgfutil@tmpf}{sqrt(TD("(\pgfutil@tmpb)o(\pgfutil@tmpb)"))}%
\pgfmathsetmacro{\pgfutil@tmpg}{sqrt(TD("(\pgfutil@tmpL)o(\pgfutil@tmpL)"))}%
\pgfmathsetmacro{\pgfutil@tmph}{TD("(\pgfutil@tmpL)o(\pgfutil@tmpb)")/\pgfutil@tmpf/\pgfutil@tmpg}%
\pgfmathtruncatemacro{\pgfutil@tmpi}{70+30*\pgfutil@tmph}%
\pgfmathtruncatemacro{\pgfutil@tmpi}{\pgfkeysvalueof{/tikz/3d/polyhedron/shading function}(\pgfutil@tmph)}%
\ifdim\pgfutil@tmpe pt<0pt\relax
\begin{pgfonlayer}{\pgfkeysvalueof{/tikz/3d/polyhedron/back layer}}
\tikzset{3d/polyhedron/before hidden,3d/polyhedron/back}%
\if@tikz@td@complete@dashes
\path[fill=tikz@td@face@color!\pgfutil@tmpi!black,3d/polyhedron/back,draw=none] 
	\pgfutil@tmpl;
\edef\pgfutil@tmplg{\pgfutil@tmple\space edge \pgfutil@tmplf}%
\draw[3d/polyhedron/back,every edge/.append style={/tikz/3d/polyhedron/face edges}]
	\pgfutil@tmplg;
\else
\draw[fill=tikz@td@face@color!\pgfutil@tmpi!black,3d/polyhedron/back] \pgfutil@tmpl ;
\fi
\tikzset{3d/polyhedron/after hidden}%
\end{pgfonlayer}
\else
\begin{pgfonlayer}{\pgfkeysvalueof{/tikz/3d/polyhedron/fore layer}}
\tikzset{3d/polyhedron/before visible,3d/polyhedron/fore}%
\if@tikz@td@complete@dashes
\path[fill=tikz@td@face@color!\pgfutil@tmpi!black,3d/polyhedron/fore,draw=none]
 \pgfutil@tmpl ;
\edef\pgfutil@tmplg{\pgfutil@tmple\space edge \pgfutil@tmplf}%
\draw[3d/polyhedron/fore,every edge/.append style={/tikz/3d/polyhedron/face edges}]
	\pgfutil@tmplg;
\else
\draw[fill=tikz@td@face@color!\pgfutil@tmpi!black,3d/polyhedron/fore] \pgfutil@tmpl -- cycle;
\fi
\tikzset{3d/polyhedron/after visible}%
\end{pgfonlayer}
\fi
\fi
\endgroup
},
color/.code={\colorlet{tikz@td@face@color}{#1}},color=yellow,
O/.initial={(0,0,0)},% point inside the polyhedron
L/.initial={(1,1,1)},% "light source",
fore/.style={draw,solid},fore layer/.initial=main,
back/.style={draw,dashed,fill opacity=0},back layer/.initial=main,
shading function/.initial={tikztdpolyhedronshade},
/tikz/declare function={tikztdpolyhedronshade(\x)=70+30*\x;},
before visible/.code={},after visible/.code={},
before hidden/.code={},after hidden/.code={},
create face from vertices/.code={\let\pgfutil@tmpa\relax%
\pgfutil@for\pgfutil@tmpb:={#1}\do{%
\ifx\pgfutil@tmpa\relax
\edef\pgfutil@tmpa{{(\pgfkeysvalueof{/tikz/name prefix}\pgfutil@tmpb)}}%
\else
\edef\pgfutil@tmpa{\pgfutil@tmpa,{(\pgfkeysvalueof{/tikz/name prefix}\pgfutil@tmpb)}}%
\fi
}%
\tikzset{3d/polyhedron/draw face with corners/.expanded=\pgfutil@tmpa}%
},%
create faces from vertex list/.style={/tikz/3d/polyhedron/create face from vertices/.list={#1}}%
}%
% draw named paths in some order
\tikzset{3d/draw named path behind/.code 2 args={% #1 object, #2 list of objects in front
   %\typeout{Draw #1 behind #2.}
   \tikzset{3d/current named path=#1,
   	3d/draw named path clipped against/.list={#2},
	3d/draw named path avoiding={#2}}
  },3d/draw named path clipped against/.code={% #1=clip path
  %\typeout{Clip \pgfkeysvalueof{/tikz/3d/current path} against #1.}
  \begin{scope}
   	\clip[use named path/.expanded=#1];
	\draw[3d/hidden,3d/ordered paths/\pgfkeysvalueof{/tikz/3d/current named path}/.try,
		use named path/.expanded=\pgfkeysvalueof{/tikz/3d/current named path}];
  \end{scope}},
  3d/draw named path avoiding/.code={% #1=list of paths to be avoided
  %\typeout{Draw \pgfkeysvalueof{/tikz/3d/current path} avoiding #1.}
  \begin{scope}
   \tikzset{3d/avoid named path/.list={#1}}%
   \draw[3d/visible,3d/ordered paths/\pgfkeysvalueof{/tikz/3d/current named path}/.try,
   	use named path/.expanded=\pgfkeysvalueof{/tikz/3d/current named path}];
  \end{scope}},3d/avoid named path/.code={%
  	\clip[even odd clip,use named path/.expanded=#1,generous outside path];
  },
  3d/current named path/.initial={},
  3d/draw ordered paths/.code={%
  \tikzset{3d/temporary list 1/.initial={#1},
  	3d/draw ordered path/.list={#1}}%  
  },3d/draw ordered path/.code={%
  % test if remaining list has only one element
  \expanded{\noexpand\pgfutil@in@{,}{\pgfkeysvalueof{/tikz/3d/temporary list 1}}}% 
  \tikzset{3d/temporary list 1/.remove item={#1}}
  \ifpgfutil@in@% 
	\tikzset{3d/draw named path behind/.expanded={#1}{\pgfkeysvalueof{/tikz/3d/temporary list 1}}} 
  \else
   \begin{scope}
	\draw[3d/visible,3d/ordered paths/#1/.try,
	use named path/.expanded=#1];
   \end{scope}	
  \fi  
  },3d/ordered paths/.unknown/.code={}}
% y cylinder
\tikzset{pics/ycylinder/.style={code={%
% old version
% \tikzset{3d/.cd,#1}
% \def\pv##1{\pgfkeysvalueof{/tikz/3d/##1}}
% \pgfmathsetmacro{\vmin}{atan2(sin(\pgfkeysvalueof{/tikz/3d/theta})*sin(\pgfkeysvalueof{/tikz/3d/phi}),%
% min(cos(\pgfkeysvalueof{/tikz/3d/phi}),-1/sqrt(2))*cos(\pgfkeysvalueof{/tikz/3d/theta}))}
% \pgfmathsetmacro{\vmax}{\vmin-180}
% \path[3d/cylinder/mantle]
%   let \p1=($(0,1,0)-(0,0,0)$),\n1={atan2(\y1,\x1)+180} in
%   [shading angle=\n1]
%   plot[variable=\t,domain=\vmin:\vmax,smooth]
%     ({\pv{r}*cos(\t)},0,{\pv{r}*sin(\t)})
%     -- 
%     plot[variable=\t,domain=\vmax:\vmin,smooth]
%     ({\pv{r}*cos(\t)},\pv{h},{\pv{r}*sin(\t)})
%     --cycle;
% \pgfmathtruncatemacro{\itest}{sign(cos(\pgfkeysvalueof{/tikz/3d/phi}))}
% \ifnum\itest=-1
%     \path[3d/cylinder/top] plot[variable=\t,domain=0:360,smooth cycle]
%     ({\pv{r}*cos(\t)},\pv{h},{\pv{r}*sin(\t)}) ;
% \fi
% \ifnum\itest=1
%     \path[3d/cylinder/top] plot[variable=\t,domain=0:360,smooth cycle]
%     ({\pv{r}*cos(\t)},0,{\pv{r}*sin(\t)}) ;
% \fi
% new version
\tikzset{3d/.cd,#1}%
%\def\pv##1{\pgfkeysvalueof{/tikz/3d/##1}}
\pgfmathsetmacro{\tikz@td@vmin}{-atan2(sin(\pgfkeysvalueof{/tikz/3d/phi})*sin(\pgfkeysvalueof{/tikz/3d/theta}),cos(\pgfkeysvalueof{/tikz/3d/theta}))}%
\pgfmathsetmacro{\tikz@td@vmax}{\tikz@td@vmin+180}%
\path[3d/cylinder/mantle]
  let \p1=($(0,1,0)-(0,0,0)$),\n1={atan2(\y1,\x1)+180} in
  [shading angle=\n1]
  plot[variable=\tikz@td@t,domain=\tikz@td@vmin:\tikz@td@vmax,smooth]
    ({\pgfkeysvalueof{/tikz/3d/r}*cos(\tikz@td@t)},0,{\pgfkeysvalueof{/tikz/3d/r}*sin(\tikz@td@t)})
    -- 
    plot[variable=\tikz@td@t,domain=\tikz@td@vmax:\tikz@td@vmin,smooth]
    ({\pgfkeysvalueof{/tikz/3d/r}*cos(\tikz@td@t)},\pgfkeysvalueof{/tikz/3d/h},{\pgfkeysvalueof{/tikz/3d/r}*sin(\tikz@td@t)})
    --cycle;
\pgfmathtruncatemacro{\tikz@td@i}{sign(cos(\pgfkeysvalueof{/tikz/3d/phi}))}%
\ifnum\tikz@td@i=-1\relax
\pgfmathtruncatemacro{\tikz@td@i}{sign(cos(\pgfkeysvalueof{/tikz/3d/phi}))}%
    \path[3d/cylinder/top] plot[variable=\tikz@td@t,domain=0:360,smooth cycle]
    ({\pgfkeysvalueof{/tikz/3d/r}*cos(\tikz@td@t)},\pgfkeysvalueof{/tikz/3d/h},{\pgfkeysvalueof{/tikz/3d/r}*sin(\tikz@td@t)}) ;
\fi
\ifnum\tikz@td@i=1\relax
    \path[3d/cylinder/top] plot[variable=\tikz@td@t,domain=0:360,smooth cycle]
    ({\pgfkeysvalueof{/tikz/3d/r}*cos(\tikz@td@t)},0,{\pgfkeysvalueof{/tikz/3d/r}*sin(\tikz@td@t)}) ;
\fi
}},pics/cylinder/.style={code={%
% arbitrary cylinder
\tikzset{3d/.cd,#1}%
\pgfmathsetmacro{\tikz@td@v}{TD("\pgfkeysvalueof{/tikz/3d/cylinder/axis}x(nscreenx,nscreeny,nscreenz)")}%
\pgfmathtruncatemacro{\tikz@td@i}{abs(TD("(\tikz@td@v)o(\tikz@td@v)"))>0.01?1:0}%
\ifnum\tikz@td@i=0\relax 
  \path[3d/cylinder/top] circle[radius=\pgfkeysvalueof{/tikz/3d/r}];
\else 
  \pgfmathsetmacro{\tikz@td@ex}{TDunit("\pgfkeysvalueof{/tikz/3d/cylinder/axis}x(nscreenx,nscreeny,nscreenz)")}%
  \pgfmathsetmacro{\tikz@td@ey}{TDunit("(\tikz@td@ex)x\pgfkeysvalueof{/tikz/3d/cylinder/axis}")}%
  \pgfmathtruncatemacro{\tikz@td@i}{TD("\pgfkeysvalueof{/tikz/3d/cylinder/axis}o(nscreenx,nscreeny,nscreenz)")>0?1:0}%
  \ifnum\tikz@td@i=1\relax 
    \pgfmathsetmacro{\tikz@td@ey}{TD("-1*(\tikz@td@ey)")}%
  \else
    %\pgfmathsetmacro{\tikz@td@ex}{TD("-1*(\tikz@td@ex)")}%
  \fi
  \pgfmathsetmacro{\tikz@td@ez}{TDunit("\pgfkeysvalueof{/tikz/3d/cylinder/axis}")}%
  \expanded{\noexpand\path[overlay,
	3d coordinate={\pgfkeysvalueof{/tikz/3d/aux keys/ex}=(\tikz@td@ex)},
	3d coordinate={\pgfkeysvalueof{/tikz/3d/aux keys/ey}=(\tikz@td@ey)},
	3d coordinate={\pgfkeysvalueof{/tikz/3d/aux keys/ez}=(\tikz@td@ez)}];}%
  \pgfmathtruncatemacro{\tikz@td@i}{TD("\pgfkeysvalueof{/tikz/3d/cylinder/axis}o(nscreenx,nscreeny,nscreenz)")>0?1:0}%
  \begin{scope}[x/.expanded={\pgfkeysvalueof{/tikz/3d/aux keys/ex}},
    y/.expanded={\pgfkeysvalueof{/tikz/3d/aux keys/ey}},
    z/.expanded={\pgfkeysvalueof{/tikz/3d/aux keys/ez}}]       
    \ifnum\tikz@td@i=1\relax 
      \draw[3d/hidden] (\pgfkeysvalueof{/tikz/3d/r},0,0) arc[start angle=0,end angle=180,radius=\pgfkeysvalueof{/tikz/3d/r}];
    \else 
      \draw[3d/hidden] (\pgfkeysvalueof{/tikz/3d/r},0,\pgfkeysvalueof{/tikz/3d/h}) arc[start angle=0,end angle=180,radius=\pgfkeysvalueof{/tikz/3d/r}];
    \fi
    \path[3d/cylinder/mantle]
      let \p1=($(0,1,0)-(0,0,0)$),\n1={atan2(\y1,\x1)+180} in
      [shading angle=\n1]
      (\pgfkeysvalueof{/tikz/3d/r},0,0) arc[start angle=0,end angle=-180,radius=\pgfkeysvalueof{/tikz/3d/r}]
        -- 
      ({-1*(\pgfkeysvalueof{/tikz/3d/r})},0,\pgfkeysvalueof{/tikz/3d/h}) arc[start angle=-180,end angle=0,radius=\pgfkeysvalueof{/tikz/3d/r}]
      -- cycle;
    \ifnum\tikz@td@i=1\relax 
      \path[3d/cylinder/top] (0,0,\pgfkeysvalueof{/tikz/3d/h}) circle[radius=\pgfkeysvalueof{/tikz/3d/r}];
    \else 
      \path[3d/cylinder/top] (0,0,0) circle[radius=\pgfkeysvalueof{/tikz/3d/r}];
    \fi
  \end{scope}  
\fi
}},%
3d/.cd,cylinder/.cd,
mantle/.style={draw},top/.style={draw}}
\tikzset{3d/.cd,visible/.style={draw,solid},
	hidden/.style={draw,very thin,cheating dash},
	r/.initial=1,h/.initial=1,R/.initial=2,
  cylinder/axis/.initial={(0,0,1)}}
%%
%% decorations
%% 
%% path restoration
\newcounter{tikz@td@recorded@point}
\pgfmathdeclarefunction{tikztdindexoflastcoordinate}{0}{%
\edef\pgfmathresult{\number\value{tikz@td@recorded@point}}%
}%

\tikzset{stored path/.cd,coordinate prefix/.initial={stored-},
	reset coordinate index/.code={\setcounter{tikz@td@recorded@point}{0}},
	restore path/.style={insert path/.expanded={\csname tikz@td@recorded@path@f@#1\endcsname}},%	
	restore reversed path/.style={insert path/.expanded={\csname tikz@td@recorded@path@r@#1\endcsname}},%	
	append path/.style={insert path/.expanded={-- \csname tikz@td@recorded@path@f@#1\endcsname}},%	
	append reversed path/.style={insert path/.expanded={-- \csname tikz@td@recorded@path@r@#1\endcsname}},%	
	first coordinate of/.style={insert path/.expanded={(\pgfkeysvalueof{/tikz/stored path/coordinate prefix}#1-0)}},%	
	last coordinate of/.style={insert path/.expanded={(\pgfkeysvalueof{/tikz/stored path/coordinate prefix}#1-\the\numexpr\value{tikz@td@recorded@point})}},%	
	coordinate with index/.style args={#1 of #2}{insert path/.expanded={(\pgfkeysvalueof{/tikz/stored path/coordinate prefix}#2-#1)}},%	
/tikz/extend stored path/.style={%
	%/utils/exec=\typeout{\arabic{tikz@td@recorded@point}},
    decorate,decoration={show path construction,
    moveto code={\def\tikz@td@prefix{\pgfkeysvalueof{/tikz/stored path/coordinate prefix}#1-}%
	\path (\tikzinputsegmentfirst) 
		coordinate (\tikz@td@prefix\the\numexpr\value{tikz@td@recorded@point});
    \ifnum\value{tikz@td@recorded@point}=0
	 \expandafter\xdef\csname tikz@td@recorded@path@f@#1\endcsname{% forward
	 	(\tikz@td@prefix\the\numexpr\value{tikz@td@recorded@point})}%
	 \expandafter\xdef\csname tikz@td@recorded@path@r@#1\endcsname{% reverse
	 	(\tikz@td@prefix\the\numexpr\value{tikz@td@recorded@point})}%
	\else
	 \expandafter\xdef\csname tikz@td@recorded@path@f@#1\endcsname{% forward
	 	\csname tikz@td@recorded@path@f@#1\endcsname
		(\tikz@td@prefix\the\numexpr\value{tikz@td@recorded@point})}%
	 \expandafter\xdef\csname tikz@td@recorded@path@r@#1\endcsname{% reverse
	 	(\tikz@td@prefix\the\numexpr\value{tikz@td@recorded@point}) 
		\csname tikz@td@recorded@path@r@#1\endcsname}%
	\fi
	\stepcounter{tikz@td@recorded@point}%	
    },
    lineto code={\def\tikz@td@prefix{\pgfkeysvalueof{/tikz/stored path/coordinate prefix}#1-}%
	\path (\tikzinputsegmentfirst) 
		coordinate (\tikz@td@prefix\the\numexpr\value{tikz@td@recorded@point})
		 (\tikzinputsegmentlast) 
		coordinate (\tikz@td@prefix\the\numexpr\value{tikz@td@recorded@point}+1);
    \ifnum\value{tikz@td@recorded@point}=0
	 \expandafter\xdef\csname tikz@td@recorded@path@f@#1\endcsname{% forward
	 	(\tikz@td@prefix\the\numexpr\value{tikz@td@recorded@point})
		--(\tikz@td@prefix\the\numexpr\value{tikz@td@recorded@point}+1)}%
	 \expandafter\xdef\csname tikz@td@recorded@path@r@#1\endcsname{% reverse
	 	(\tikz@td@prefix\the\numexpr\value{tikz@td@recorded@point}+1)
		--(\tikz@td@prefix\the\numexpr\value{tikz@td@recorded@point})}%
	\else
	 \expandafter\xdef\csname tikz@td@recorded@path@f@#1\endcsname{% forward
	 	\csname tikz@td@recorded@path@f@#1\endcsname
		--(\tikz@td@prefix\the\numexpr\value{tikz@td@recorded@point}+1)}%
	 \expandafter\xdef\csname tikz@td@recorded@path@r@#1\endcsname{% reverse
	 	(\tikz@td@prefix\the\numexpr\value{tikz@td@recorded@point}+1) --
		\csname tikz@td@recorded@path@r@#1\endcsname}%
	\fi
	\stepcounter{tikz@td@recorded@point}%	
    },
    curveto code={\def\tikz@td@prefix{\pgfkeysvalueof{/tikz/stored path/coordinate prefix}#1-}%
      \path (\tikzinputsegmentfirst)
	    coordinate (\tikz@td@prefix\the\numexpr\value{tikz@td@recorded@point})
        (\tikzinputsegmentsupporta) 
		coordinate (\tikz@td@prefix\the\numexpr\value{tikz@td@recorded@point}+1)
		(\tikzinputsegmentsupportb)
		coordinate (\tikz@td@prefix\the\numexpr\value{tikz@td@recorded@point}+2)
        (\tikzinputsegmentlast)
		coordinate (\tikz@td@prefix\the\numexpr\value{tikz@td@recorded@point}+3);
    \ifnum\value{tikz@td@recorded@point}=0
	 \expandafter\xdef\csname tikz@td@recorded@path@f@#1\endcsname{% forward
	 	(\tikz@td@prefix\the\numexpr\value{tikz@td@recorded@point})
		.. controls (\tikz@td@prefix\the\numexpr\value{tikz@td@recorded@point}+1)
		and (\tikz@td@prefix\the\numexpr\value{tikz@td@recorded@point}+2)
		.. (\tikz@td@prefix\the\numexpr\value{tikz@td@recorded@point}+3)}%
	 \expandafter\xdef\csname tikz@td@recorded@path@r@#1\endcsname{% reverse
	 	(\tikz@td@prefix\the\numexpr\value{tikz@td@recorded@point}+3)
		.. controls (\tikz@td@prefix\the\numexpr\value{tikz@td@recorded@point}+2)
		and (\tikz@td@prefix\the\numexpr\value{tikz@td@recorded@point}+1)
		.. (\tikz@td@prefix\the\numexpr\value{tikz@td@recorded@point})}%
	\else
	 \expandafter\xdef\csname tikz@td@recorded@path@f@#1\endcsname{% forward
	 	\csname tikz@td@recorded@path@f@#1\endcsname
		.. controls (\tikz@td@prefix\the\numexpr\value{tikz@td@recorded@point}+1)
		and (\tikz@td@prefix\the\numexpr\value{tikz@td@recorded@point}+2)
		.. (\tikz@td@prefix\the\numexpr\value{tikz@td@recorded@point}+3)}%
	 \expandafter\xdef\csname tikz@td@recorded@path@r@#1\endcsname{% reverse
	 	(\tikz@td@prefix\the\numexpr\value{tikz@td@recorded@point}+3)
		.. controls (\tikz@td@prefix\the\numexpr\value{tikz@td@recorded@point}+2)
		and (\tikz@td@prefix\the\numexpr\value{tikz@td@recorded@point}+1) ..
		\csname tikz@td@recorded@path@r@#1\endcsname}%
	\fi
	\stepcounter{tikz@td@recorded@point}%	
	\stepcounter{tikz@td@recorded@point}%	
	\stepcounter{tikz@td@recorded@point}%	
    },
    closepath code={\def\tikz@td@prefix{\pgfkeysvalueof{/tikz/stored path/coordinate prefix}#1-}%
	\path (\tikzinputsegmentfirst) 
		coordinate (\tikz@td@prefix\the\numexpr\value{tikz@td@recorded@point})
		 (\tikzinputsegmentlast) 
		coordinate (\tikz@td@prefix\the\numexpr\value{tikz@td@recorded@point}+1);
    \ifnum\value{tikz@td@recorded@point}=0
	 \expandafter\xdef\csname tikz@td@recorded@path@f@#1\endcsname{% forward
	 	(\tikz@td@prefix\the\numexpr\value{tikz@td@recorded@point})
		--(\tikz@td@prefix\the\numexpr\value{tikz@td@recorded@point}+1)}%
	 \expandafter\xdef\csname tikz@td@recorded@path@r@#1\endcsname{% reverse
	 	(\tikz@td@prefix\the\numexpr\value{tikz@td@recorded@point}+1)
		--(\tikz@td@prefix\the\numexpr\value{tikz@td@recorded@point})}%
	\else
	 \expandafter\xdef\csname tikz@td@recorded@path@f@#1\endcsname{% forward
	 	\csname tikz@td@recorded@path@f@#1\endcsname
		--(\tikz@td@prefix\the\numexpr\value{tikz@td@recorded@point}+1)}%
	 \expandafter\xdef\csname tikz@td@recorded@path@r@#1\endcsname{% reverse
	 	(\tikz@td@prefix\the\numexpr\value{tikz@td@recorded@point}+1) --
		\csname tikz@td@recorded@path@r@#1\endcsname}%
	\fi
	  } }},
/tikz/store path/.style={%	  
	  /tikz/stored path/reset coordinate index,%
	  /tikz/extend stored path=#1}
	  }
%% bounding box for animations
\def\tikz@td@bbox@store@aux#1#2{%
	\immediate\write\@mainaux{\string\expandafter\xdef\noexpand\csname pgfk@/tikz/3d/bbox/stored/#1\string\endcsname{#2}}%
	\expandafter\xdef\csname pgfk@/tikz/3d/bbox/stored/#1\endcsname{#2}}%
\def\tikz@td@bbox@@get@min@from@aux#1#2{%
	\ifcsname pgfk@/tikz/3d/bbox/stored/#1min\endcsname
	\edef#2{\csname pgfk@/tikz/3d/bbox/stored/#1min\endcsname}%
	\else
	\edef#2{16383.99999pt}%
	\expandafter\edef\csname pgfk@/tikz/3d/bbox/stored/#1min\endcsname{16383.99999pt}%
	\fi}
\def\tikz@td@bbox@@get@max@from@aux#1#2{%
	\ifcsname pgfk@/tikz/3d/bbox/stored/#1max\endcsname
	\edef#2{\csname pgfk@/tikz/3d/bbox/stored/#1max\endcsname}%
	\else
	\edef#2{-16383.99999pt}%
	\expandafter\edef\csname pgfk@/tikz/3d/bbox/stored/#1max\endcsname{-16383.99999pt}%
	\fi}
\tikzset{same bounding box/.style={%
execute at end picture={%
\tikz@td@bbox@@get@min@from@aux{#1x}\pgfutil@tmpa%
\tikz@td@bbox@@get@min@from@aux{#1y}\pgfutil@tmpb%
\tikz@td@bbox@@get@max@from@aux{#1x}\pgfutil@tmpc%
\tikz@td@bbox@@get@max@from@aux{#1y}\pgfutil@tmpd%
%\typeout{(\pgfutil@tmpa,\pgfutil@tmpb) (\pgfutil@tmpc,\pgfutil@tmpd)}%
\pgfmathsetmacro\pgfutil@tmpa{min(\pgfutil@tmpa,\pgf@picminx,\pgfkeysvalueof{/tikz/3d/bbox/stored/#1xmin})}%
\pgfmathsetmacro\pgfutil@tmpb{min(\pgfutil@tmpb,\pgf@picminy,\pgfkeysvalueof{/tikz/3d/bbox/stored/#1ymin})}%
\pgfmathsetmacro\pgfutil@tmpc{max(\pgfutil@tmpc,\pgf@picmaxx,\pgfkeysvalueof{/tikz/3d/bbox/stored/#1xmax})}%
\pgfmathsetmacro\pgfutil@tmpd{max(\pgfutil@tmpd,\pgf@picmaxy,\pgfkeysvalueof{/tikz/3d/bbox/stored/#1ymax})}%
%\typeout{(\pgfutil@tmpa,\pgfutil@tmpb) (\pgfutil@tmpc,\pgfutil@tmpd)}%
\tikz@td@bbox@store@aux{#1xmin}{\pgfutil@tmpa}%
\tikz@td@bbox@store@aux{#1ymin}{\pgfutil@tmpb}%
\tikz@td@bbox@store@aux{#1xmax}{\pgfutil@tmpc}%
\tikz@td@bbox@store@aux{#1ymax}{\pgfutil@tmpd}%
\ifdim\pgfutil@tmpa pt<16383.99999pt\relax
\path (\pgfutil@tmpa pt,\pgfutil@tmpb pt) (\pgfutil@tmpc pt,\pgfutil@tmpd pt);
\fi
}},same bounding box/.default=A} 	  
%% list management
\newif\if@pgf@list@first@item
\pgfkeys{/handlers/.add item/.code=\pgfkeys{\pgfkeyscurrentpath/.append={,#1}},
/handlers/.remove item/.code={%
\edef\pgfutil@tmpa{\pgfkeysvalueof{\pgfkeyscurrentpath}}%
\edef\pgfutil@tmpb{#1}%
\edef\pgfutil@tmpc{\noexpand\@removeelement{\pgfutil@tmpb}{\pgfutil@tmpa}{\noexpand\pgfutil@tmpa}}%
\pgfutil@tmpc
\pgfkeyssetvalue{\pgfkeyscurrentpath}{\pgfutil@tmpa}},% maybe test if the list is now empty?
/handlers/.count/.code={\begingroup%
\edef\pgfutil@tmpl{\pgfkeysvalueof{\pgfkeyscurrentpath}}%
\c@pgf@counta0\relax
\pgfkeys{/list management/step count/.list/.expanded={\pgfutil@tmpl}}%
\edef#1{\the\c@pgf@counta}%
\pgfmathsmuggle#1\endgroup},%
/handlers/.print list/.code={\begingroup%
\@pgf@list@first@itemtrue
\edef\pgfutil@tmpl{\pgfkeysvalueof{\pgfkeyscurrentpath}}%
\pgfkeys{/list management/print item in list/.list/.expanded={\pgfutil@tmpl}}%
\endgroup},
/handlers/.is array/.code={\pgfkeysifdefined{\pgfkeyscurrentpath}{%
\typeout{The key `\pgfkeyscurrentpath` is already in use, and won't get overwritten.}}{%
\pgfkeysifdefined{\pgfkeyscurrentpath/dim}{%
\typeout{The key `\pgfkeyscurrentpath` is already in use, and won't get overwritten.}}{%
\c@pgf@counta=0\relax
\pgfkeyssetevalue{/list management/current array}{\pgfkeyscurrentpath}%
\pgfkeys{/list management/store array entry/.list/.expanded={#1}}%
\pgfkeys{\pgfkeysvalueof{/list management/current array}/dim/.initial=\the\c@pgf@counta}%
\pgfkeys{\pgfkeysvalueof{/list management/current array}/content/.initial={#1}}%
}}},
/handlers/.sort numeric list/.code 2 args={\begingroup%
\edef\pgfutil@tmpl{\pgfkeysvalueof{\pgfkeyscurrentpath}}%
\edef\pgfutil@tmpa{0}%
\pgfutil@for\pgfutil@tmpb:={\pgfutil@tmpl}\do{% build an indexed array and 
\edef\pgfutil@tmpa{\the\numexpr\pgfutil@tmpa+1}% precompute expressions used in comparison
\ifcase\pgfutil@tmpa
\or
\or
\edef\pgfutil@tmph{2}%
\else
\edef\pgfutil@tmph{\pgfutil@tmph,\pgfutil@tmpa}%
\fi
\pgfkeys{/list management/sort map=\pgfutil@tmpb}%
\expandafter\edef\csname pgfutil@tmpd@\pgfutil@tmpa\endcsname{\pgfmathresult}%
\expandafter\edef\csname pgfutil@tmpf@\pgfutil@tmpa\endcsname{\pgfutil@tmpa}%
}%
\edef\pgfutil@tmps{\pgfkeysvalueof{/list management/sort comparison}}%
\pgfutil@loop
\edef\pgfutil@tmpi{1}%
\pgfutil@for\pgfutil@tmpb:={\pgfutil@tmph}\do{%
\edef\pgfutil@tmpx{\@nameuse{pgfutil@tmpd@\pgfutil@tmpb}}%
\edef\pgfutil@tmpc{\the\numexpr\pgfutil@tmpb-1}%
\edef\pgfutil@tmpy{\@nameuse{pgfutil@tmpd@\pgfutil@tmpc}}%
\edef\pgfutil@tmpr{(\pgfutil@tmpx\pgfutil@tmps\pgfutil@tmpy?1:0)}%
\pgfmathtruncatemacro\pgfutil@tmpj{\pgfutil@tmpr}%
\ifnum\pgfutil@tmpj=0\relax
\edef\pgfutil@tmpi{0}%
\edef\pgfutil@tmpu{\@nameuse{pgfutil@tmpf@\pgfutil@tmpb}}%
\edef\pgfutil@tmpv{\@nameuse{pgfutil@tmpf@\pgfutil@tmpc}}%
%\typeout{swap (\pgfutil@tmpu<->\pgfutil@tmpv) and (\pgfutil@tmpx<->\pgfutil@tmpy)}%
\expandafter\edef\csname pgfutil@tmpd@\pgfutil@tmpb\endcsname{\pgfutil@tmpy}%
\expandafter\edef\csname pgfutil@tmpd@\pgfutil@tmpc\endcsname{\pgfutil@tmpx}%
\expandafter\edef\csname pgfutil@tmpf@\pgfutil@tmpb\endcsname{\pgfutil@tmpv}%
\expandafter\edef\csname pgfutil@tmpf@\pgfutil@tmpc\endcsname{\pgfutil@tmpu}%
\fi
}%
\ifnum\pgfutil@tmpi=0\relax
\pgfutil@repeat
\edef\pgfutil@tmpa{\@nameuse{pgfutil@tmpf@1}}%
\edef\pgfutil@tmpc{\@nameuse{pgfutil@tmpd@1}}%
\pgfutil@for\pgfutil@tmpb:={\pgfutil@tmph}\do{%
\edef\pgfutil@tmpa{\pgfutil@tmpa,\@nameuse{pgfutil@tmpf@\pgfutil@tmpb}}%
\edef\pgfutil@tmpc{\pgfutil@tmpc,\@nameuse{pgfutil@tmpd@\pgfutil@tmpb}}}%
\edef\pgfutil@tmpb{\noexpand\edef\noexpand#1{\pgfutil@tmpc}\noexpand\edef\noexpand#2{\pgfutil@tmpa}}%
\pgfmathsmuggle\pgfutil@tmpb\endgroup\pgfutil@tmpb},
/list management/.cd,print item/.code={#1},
print item in list/.code={%
\if@pgf@list@first@item
 \pgfkeys{/list management/print item={#1}}%
 \@pgf@list@first@itemfalse
\else
 \pgfkeys{/list management/print item={%
  \pgfkeysvalueof{/list management/list separator}#1}}%
\fi},
list separator/.initial={,\space},
step count/.code={\advance\c@pgf@counta by1\relax},
sort comparison/.initial={>=},
sort map/.code={\pgfmathparse{#1}},
current array/.initial={},
store array entry/.code={\advance\c@pgf@counta by1\relax
\pgfkeyssetevalue{\pgfkeysvalueof{/list management/current array}/\the\c@pgf@counta}{#1}}
}%
%% coil
\newif\ifcoil@closed%
\pgfkeys{%%
/pgf/decoration/.cd,%
3d coil color/.initial=black,%
3d coil width/.initial=0.4pt,%
3d coil dist/.initial=0.6pt,%
3d coil opacity/.initial=1,%
3d coil closed/.code=\coil@closedtrue%
}%
% https://tex.stackexchange.com/a/219088/121799%
% \tikzset{get stroke color/.code={%%
%     \expandafter\global% Jump over, now we have \global%
%     \expandafter\let% Jump over now we have \global\let%
%     \expandafter\pgfsavedstrokecolor% Jump we have \global\let\pgf...%
%     \csname\string\color@pgfstrokecolor\endcsname% Finally expand this and put it at the end %
% 	\typeout{\pgfsavedstrokecolor}%
% 	\pgfutil@namelet{\string\color@pgfstrokecolor}{pgf@strokecolor@global}%
%     },                                           % \global\let\pgf...{} in expanded form %
%     restore stroke color/.code={\pgf@setstrokecolor#1},%
% }%
\def\pgfpoint@onthreedcoil#1#2#3{%%
  \pgf@x=#1\pgfdecorationsegmentamplitude%%
  \pgf@x=\pgfdecorationsegmentaspect\pgf@x%%
  \pgf@y=#2\pgfdecorationsegmentamplitude%%
  \pgf@xa=0.083333333333\pgfdecorationsegmentlength%%
  \advance\pgf@x by#3\pgf@xa%%
  \advance\pgf@x by-\generaloffset pt%%
}%
% coil decoration%
%%
% Parameters: \pgfdecorationsegmentamplitude, \pgfdecorationsegmentlength,%
\pgfdeclaredecoration{3d complete coil}{initial}%
{ %
    \state{initial}[width=0.5*\pgfdecorationsegmentlength,%
    next state=coil, persistent precomputation={% from https://tex.stackexchange.com/a/25689/121799%
    \pgfmathsetmacro\matchinglength{\pgfdecoratedinputsegmentlength / int(\pgfdecoratedinputsegmentlength/\pgfdecorationsegmentlength)}%
    \setlength{\pgfdecorationsegmentlength}{\matchinglength pt}%
    %\tikzset{get stroke color}%
    \pgfmathsetmacro{\generaloffset}{\pgfdecorationsegmentlength}%
    \pgfmathsetmacro{\initialoffset}{1.5*\pgfdecorationsegmentlength}%
    \pgfmathsetmacro{\auxoffset}{2.5*\pgfdecorationsegmentlength}%
  }]    { %
    % line in the back%
    %%
	\edef\TDCoilColor{\pgfkeysvalueof{/pgf/decoration/3d coil color}}%
	\edef\TDCoilOpacity{\pgfkeysvalueof{/pgf/decoration/3d coil opacity}}%
	\edef\TDCoilWidth{\pgfkeysvalueof{/pgf/decoration/3d coil width}}%
	\edef\TDCoilDist{\pgfkeysvalueof{/pgf/decoration/3d coil dist}}%
    \pgfsetstrokecolor{\pgfkeysvalueof{/pgf/decoration/3d coil color}}%
    \pgfsetfillcolor{\pgfkeysvalueof{/pgf/decoration/3d coil color}}%
    \pgfsetstrokeopacity{\pgfkeysvalueof{/pgf/decoration/3d coil opacity}}%
    \pgfsetlinewidth{\pgfkeysvalueof{/pgf/decoration/3d coil width}}     %
    \ifcoil@closed%
     \begingroup%
      \def\generaloffset{\auxoffset}%
      \pgfpathmoveto{\pgfpoint@onthreedcoil{1    }{ 1    }{15}}%
      \pgfpathcurveto%
      {\pgfpoint@onthreedcoil{1.555}{ 1    }{16}}%
      {\pgfpoint@onthreedcoil{2    }{ 0.555}{17}}%
      {\pgfpoint@onthreedcoil{2    }{ 0    }{18}}%
      \pgfcoordinate{TD@coilast}{\pgfpoint@onthreedcoil{2    }{ 0    }{18}}%
      \pgfcoordinate{TD@coilfirst}{\pgfpoint@onthreedcoil{1    }{ 1    }{15}}%
      \pgfusepath{stroke} %
      \pgfsetstrokecolor{\pgfkeysvalueof{/pgf/decoration/3d coil color}}%
     \endgroup%
    \fi%
    \begingroup %%
    \def\generaloffset{\initialoffset}%
    \ifcoil@closed%
     \pgfpathmoveto{\pgfpointanchor{TD@coilast}{center}}%
    \else%
     \pgfpathmoveto{\pgfpointorigin}%
    \fi%
    \pgfpathcurveto%
    {\pgfpoint@onthreedcoil{2    }{-0.555}{7}}%
    {\pgfpoint@onthreedcoil{1.555}{-1    }{8}}%
    {\pgfpoint@onthreedcoil{1    }{-1    }{9}}%
    \pgfusepath{stroke} %
    %%
    % white background for front thick part%
    %%
    \pgfsetstrokeopacity{1}%
    \pgfsetstrokecolor{white}%
    \pgfsetfillcolor{white}%
    \pgfsetlinewidth{1.5*\pgfkeysvalueof{/pgf/decoration/3d coil width}+1.5*\pgfkeysvalueof{/pgf/decoration/3d coil dist}}%
    \pgfpathmoveto{\pgfpoint@onthreedcoil{1    }{-1    }{9}}%
    % draw forward%
    \pgfpathcurveto%
    {\pgfpoint@onthreedcoil{0.445}{-1    }{10}}%
    {\pgfpoint@onthreedcoil{0    }{-0.555}{11.25}}%
    {\pgfpoint@onthreedcoil{0    }{ 0    }{12.5}}%
    \pgfpathcurveto%
    {\pgfpoint@onthreedcoil{0    }{ 0.555}{13.25}}%
    {\pgfpoint@onthreedcoil{0.445}{ 1    }{14.25}}%
    {\pgfpoint@onthreedcoil{1    }{ 1    }{15}}%
    % draw the curve back%
    \pgfpathcurveto%
    {\pgfpoint@onthreedcoil{0.445}{ 1    }{14}}%
    {\pgfpoint@onthreedcoil{0    }{ 0.555}{12.75}}%
    {\pgfpoint@onthreedcoil{0    }{ 0    }{11.5}}%
    \pgfpathcurveto%
    {\pgfpoint@onthreedcoil{0    }{-0.555}{10.75}}%
    {\pgfpoint@onthreedcoil{0.445}{-1    }{10}}%
    {\pgfpoint@onthreedcoil{1    }{-1    }{9}}%
    \pgfusepath{stroke,fill} %
    % %
    % draw the thick foreground path%
    %%
    \pgfsetstrokecolor{\pgfkeysvalueof{/pgf/decoration/3d coil color}}%
    \pgfsetfillcolor{\pgfkeysvalueof{/pgf/decoration/3d coil color}}%
    \pgfsetstrokeopacity{\pgfkeysvalueof{/pgf/decoration/3d coil opacity}}%
    \pgfpathmoveto{\pgfpoint@onthreedcoil{1    }{ 1    }{3}}%
    \pgfsetlinewidth{\pgfkeysvalueof{/pgf/decoration/3d coil width}} %
    % forward shifted +%
    \pgfpathmoveto{\pgfpoint@onthreedcoil{1    }{-1    }{9}}%
    \pgfpathcurveto%
    {\pgfpoint@onthreedcoil{0.445}{-1    }{10}}%
    {\pgfpoint@onthreedcoil{0    }{-0.555}{11.25}}%
    {\pgfpoint@onthreedcoil{0    }{ 0    }{12.5}}%
    \pgfpathcurveto%
    {\pgfpoint@onthreedcoil{0    }{ 0.555}{13.25}}%
    {\pgfpoint@onthreedcoil{0.445}{ 1    }{14.25}}%
    {\pgfpoint@onthreedcoil{1    }{ 1    }{15}}%
    % draw the curve back shfted -%
    \pgfpathcurveto%
    {\pgfpoint@onthreedcoil{0.445}{ 1    }{14}}%
    {\pgfpoint@onthreedcoil{0    }{ 0.555}{12.75}}%
    {\pgfpoint@onthreedcoil{0    }{ 0    }{11.5}}%
    \pgfpathcurveto%
    {\pgfpoint@onthreedcoil{0    }{-0.555}{10.75}}%
    {\pgfpoint@onthreedcoil{0.445}{-1    }{10}}%
    {\pgfpoint@onthreedcoil{1    }{-1    }{9}}%
    \pgfusepath{stroke,fill} %
    \pgfpathmoveto{\pgfpoint@onthreedcoil{1    }{ 1    }{15}}%
    \pgfpathcurveto%
    {\pgfpoint@onthreedcoil{1.555}{ 1    }{16}}%
    {\pgfpoint@onthreedcoil{2    }{ 0.555}{17}}%
    {\pgfpoint@onthreedcoil{2    }{ 0    }{18}}%
    \pgfcoordinate{TD@coilast}{\pgfpoint@onthreedcoil{2    }{ 0    }{18}} %
    \pgfusepath{stroke}     %
    \endgroup%
  }%
  \state{coil}[switch if less than=%%
    1.9*\pgfdecorationsegmentlength  to last,%
               width=+\pgfdecorationsegmentlength]%
    { % line in the back%
    %%
    \pgfsetstrokecolor{\pgfkeysvalueof{/pgf/decoration/3d coil color}}%
    \pgfsetfillcolor{\pgfkeysvalueof{/pgf/decoration/3d coil color}}%
    \pgfsetstrokeopacity{\pgfkeysvalueof{/pgf/decoration/3d coil opacity}}%
    \pgfpathmoveto{\pgfpointanchor{TD@coilast}{center}}%
    \pgfsetlinewidth{\pgfkeysvalueof{/pgf/decoration/3d coil width}} %
    \pgfpathcurveto%
    {\pgfpoint@onthreedcoil{2    }{-0.555}{7}}%
    {\pgfpoint@onthreedcoil{1.555}{-1    }{8}}%
    {\pgfpoint@onthreedcoil{1    }{-1    }{9}}%
    \pgfusepath{stroke} %
    %%
    % white background for front thick part%
    %%
    \pgfsetstrokeopacity{1}%
    \pgfsetstrokecolor{white}%
    \pgfsetfillcolor{white}%
    \pgfsetlinewidth{1.5*\pgfkeysvalueof{/pgf/decoration/3d coil width}+1.5*\pgfkeysvalueof{/pgf/decoration/3d coil dist}}%
    \pgfpathmoveto{\pgfpoint@onthreedcoil{1    }{ 1    }{3}}%
    \pgfpathmoveto{\pgfpoint@onthreedcoil{1    }{-1    }{9}}%
    % draw forward%
    \pgfpathcurveto%
    {\pgfpoint@onthreedcoil{0.445}{-1    }{10}}%
    {\pgfpoint@onthreedcoil{0    }{-0.555}{11.25}}%
    {\pgfpoint@onthreedcoil{0    }{ 0    }{12.5}}%
    \pgfpathcurveto%
    {\pgfpoint@onthreedcoil{0    }{ 0.555}{13.25}}%
    {\pgfpoint@onthreedcoil{0.445}{ 1    }{14.25}}%
    {\pgfpoint@onthreedcoil{1    }{ 1    }{15}}%
    % draw the curve back%
    \pgfpathcurveto%
    {\pgfpoint@onthreedcoil{0.445}{ 1    }{14}}%
    {\pgfpoint@onthreedcoil{0    }{ 0.555}{12.75}}%
    {\pgfpoint@onthreedcoil{0    }{ 0    }{11.5}}%
    \pgfpathcurveto%
    {\pgfpoint@onthreedcoil{0    }{-0.555}{10.75}}%
    {\pgfpoint@onthreedcoil{0.445}{-1    }{10}}%
    {\pgfpoint@onthreedcoil{1    }{-1    }{9}}%
    \pgfusepath{stroke,fill} %
    % %
    % draw the thick foreground path%
    %%
    \pgfsetstrokecolor{\pgfkeysvalueof{/pgf/decoration/3d coil color}}%
    \pgfsetfillcolor{\pgfkeysvalueof{/pgf/decoration/3d coil color}}%
    \pgfsetstrokeopacity{\pgfkeysvalueof{/pgf/decoration/3d coil opacity}}%
    \pgfpathmoveto{\pgfpoint@onthreedcoil{1    }{ 1    }{3}}%
    \pgfsetlinewidth{\pgfkeysvalueof{/pgf/decoration/3d coil width}} %
    % forward shifted +%
    \pgfpathmoveto{\pgfpoint@onthreedcoil{1    }{-1    }{9}}%
    \pgfpathcurveto%
    {\pgfpoint@onthreedcoil{0.445}{-1    }{10}}%
    {\pgfpoint@onthreedcoil{0    }{-0.555}{11.25}}%
    {\pgfpoint@onthreedcoil{0    }{ 0    }{12.5}}%
    \pgfpathcurveto%
    {\pgfpoint@onthreedcoil{0    }{ 0.555}{13.25}}%
    {\pgfpoint@onthreedcoil{0.445}{ 1    }{14.25}}%
    {\pgfpoint@onthreedcoil{1    }{ 1    }{15}}%
    % draw the curve back shfted -%
    \pgfpathcurveto%
    {\pgfpoint@onthreedcoil{0.445}{ 1    }{14}}%
    {\pgfpoint@onthreedcoil{0    }{ 0.555}{12.75}}%
    {\pgfpoint@onthreedcoil{0    }{ 0    }{11.5}}%
    \pgfpathcurveto%
    {\pgfpoint@onthreedcoil{0    }{-0.555}{10.75}}%
    {\pgfpoint@onthreedcoil{0.445}{-1    }{10}}%
    {\pgfpoint@onthreedcoil{1    }{-1    }{9}}%
    \pgfusepath{stroke,fill} %
    \pgfpathmoveto{\pgfpoint@onthreedcoil{1    }{ 1    }{15}}%
    \pgfpathcurveto%
    {\pgfpoint@onthreedcoil{1.555}{ 1    }{16}}%
    {\pgfpoint@onthreedcoil{2    }{ 0.555}{17}}%
    {\pgfpoint@onthreedcoil{2    }{ 0    }{18}}%
    \pgfusepath{stroke} %
    \pgfcoordinate{TD@coilast}{\pgfpoint@onthreedcoil{2    }{ 0    }{18}} %
  }%
  \state{last}[next state=final]%
    { % line in the back%
    %%
    \pgfsetstrokecolor{\pgfkeysvalueof{/pgf/decoration/3d coil color}}%
    \pgfsetfillcolor{\pgfkeysvalueof{/pgf/decoration/3d coil color}}%
    \pgfsetstrokeopacity{\pgfkeysvalueof{/pgf/decoration/3d coil opacity}}%
    \pgfpathmoveto{\pgfpointanchor{TD@coilast}{center}}%
    \pgfsetlinewidth{\pgfkeysvalueof{/pgf/decoration/3d coil width}} %
    \pgfpathcurveto%
    {\pgfpoint@onthreedcoil{2    }{-0.555}{7}}%
    {\pgfpoint@onthreedcoil{1.555}{-1    }{8}}%
    {\pgfpoint@onthreedcoil{1    }{-1    }{9}}%
    \pgfusepath{stroke} %
    % %
    % draw the thick foreground path%
    %%
    \ifcoil@closed %\pgfpointanchor{TD@coilfirst}{center}%
     %%
     % white background for front thick part%
     %%
     \pgfsetstrokeopacity{1}%
     \pgfsetstrokecolor{white}%
     \pgfsetfillcolor{white}%
     \pgfsetlinewidth{1.5*\pgfkeysvalueof{/pgf/decoration/3d coil width}+1.5*\pgfkeysvalueof{/pgf/decoration/3d coil dist}}%
     \pgfpathmoveto{\pgfpoint@onthreedcoil{1    }{ 1    }{3}}%
     \pgfpathmoveto{\pgfpoint@onthreedcoil{1    }{-1    }{9}}%
     % draw forward%
     \pgfpathcurveto%
     {\pgfpoint@onthreedcoil{0.445}{-1    }{10}}%
     {\pgfpoint@onthreedcoil{0    }{-0.555}{11.25}}%
     {\pgfpoint@onthreedcoil{0    }{ 0    }{12.5}}%
     \pgfpathcurveto%
     {\pgfpoint@onthreedcoil{0    }{ 0.555}{13.25}}%
     {\pgfpoint@onthreedcoil{0.445}{ 1    }{14.25}}%
     {\pgfpointanchor{TD@coilfirst}{center}}%
     % draw the curve back%
     \pgfpathcurveto%
     {\pgfpoint@onthreedcoil{0.445}{ 1    }{14}}%
     {\pgfpoint@onthreedcoil{0    }{ 0.555}{12.75}}%
     {\pgfpoint@onthreedcoil{0    }{ 0    }{11.5}}%
     \pgfpathcurveto%
     {\pgfpoint@onthreedcoil{0    }{-0.555}{10.75}}%
     {\pgfpoint@onthreedcoil{0.445}{-1    }{10}}%
     {\pgfpoint@onthreedcoil{1    }{-1    }{9}}%
     \pgfusepath{stroke,fill} %
     \pgfsetstrokecolor{\pgfkeysvalueof{/pgf/decoration/3d coil color}}%
     \pgfsetfillcolor{\pgfkeysvalueof{/pgf/decoration/3d coil color}}%
     \pgfsetstrokeopacity{\pgfkeysvalueof{/pgf/decoration/3d coil opacity}}%
     \pgfpathmoveto{\pgfpoint@onthreedcoil{1    }{ 1    }{3}}%
     \pgfsetlinewidth{\pgfkeysvalueof{/pgf/decoration/3d coil width}} %
     % forward shifted +%
     \pgfpathmoveto{\pgfpoint@onthreedcoil{1    }{-1    }{9}}%
     \pgfpathcurveto%
     {\pgfpoint@onthreedcoil{0.445}{-1    }{10}}%
     {\pgfpoint@onthreedcoil{0    }{-0.555}{11.25}}%
     {\pgfpoint@onthreedcoil{0    }{ 0    }{12.5}}%
     \pgfpathcurveto%
     {\pgfpoint@onthreedcoil{0    }{ 0.555}{13.25}}%
     {\pgfpoint@onthreedcoil{0.445}{ 1    }{14.25}}%
     {\pgfpointanchor{TD@coilfirst}{center}}%
     % draw the curve back shifted %
     \pgfpathcurveto%
     {\pgfpoint@onthreedcoil{0.445}{ 1    }{14}}%
     {\pgfpoint@onthreedcoil{0    }{ 0.555}{12.75}}%
     {\pgfpoint@onthreedcoil{0    }{ 0    }{11.5}}%
     \pgfpathcurveto%
     {\pgfpoint@onthreedcoil{0    }{-0.555}{10.75}}%
     {\pgfpoint@onthreedcoil{0.445}{-1    }{10}}%
     {\pgfpoint@onthreedcoil{1    }{-1    }{9}}%
     \pgfusepath{stroke,fill} %
    \else%
     %%
     % white background for front thick part%
     %%
     \pgfsetstrokeopacity{1}%
     \pgfsetstrokecolor{white}%
     \pgfsetfillcolor{white}%
     \pgfsetlinewidth{1.5*\pgfkeysvalueof{/pgf/decoration/3d coil width}+1.5*\pgfkeysvalueof{/pgf/decoration/3d coil dist}}%
     \pgfpathmoveto{\pgfpoint@onthreedcoil{1}{1}{3}}%
     \pgfpathmoveto{\pgfpoint@onthreedcoil{1}{-1}{9}}%
     % draw forward%
     \pgfpathcurveto%
     {\pgfpoint@onthreedcoil{0.445}{-1    }{10}}%
     {\pgfpoint@onthreedcoil{0    }{-0.555}{11.25}}%
     {\pgfpoint@onthreedcoil{0    }{ 0    }{12.5}}%
     \pgfpathcurveto%
     {\pgfpoint@onthreedcoil{0    }{ 0.555}{13.25}}%
     {\pgfpoint@onthreedcoil{0.445}{ 1    }{14.25}}%
     {\pgfpoint@onthreedcoil{1    }{ 1    }{15}}%
     % draw the curve back%
     \pgfpathcurveto%
     {\pgfpoint@onthreedcoil{0.445}{ 1    }{14}}%
     {\pgfpoint@onthreedcoil{0    }{ 0.555}{12.75}}%
     {\pgfpoint@onthreedcoil{0    }{ 0    }{11.5}}%
     \pgfpathcurveto%
     {\pgfpoint@onthreedcoil{0    }{-0.555}{10.75}}%
     {\pgfpoint@onthreedcoil{0.445}{-1    }{10}}%
     {\pgfpoint@onthreedcoil{1    }{-1    }{9}}%
     \pgfusepath{stroke,fill} %
     \pgfsetstrokecolor{\pgfkeysvalueof{/pgf/decoration/3d coil color}}%
     \pgfsetfillcolor{\pgfkeysvalueof{/pgf/decoration/3d coil color}}%
     \pgfsetstrokeopacity{\pgfkeysvalueof{/pgf/decoration/3d coil opacity}}%
     \pgfpathmoveto{\pgfpoint@onthreedcoil{1}{1}{3}}%
     \pgfsetlinewidth{\pgfkeysvalueof{/pgf/decoration/3d coil width}} %
     % forward shifted +%
     \pgfpathmoveto{\pgfpoint@onthreedcoil{1}{-1}{9}}%
     \pgfpathcurveto%
     {\pgfpoint@onthreedcoil{0.445}{-1    }{10}}%
     {\pgfpoint@onthreedcoil{0    }{-0.555}{11.25}}%
     {\pgfpoint@onthreedcoil{0    }{ 0    }{12.5}}%
     \pgfpathcurveto%
     {\pgfpoint@onthreedcoil{0    }{ 0.555}{13.25}}%
     {\pgfpoint@onthreedcoil{0.445}{ 1    }{14.25}}%
     {\pgfpoint@onthreedcoil{1    }{ 1    }{15}}%
     % draw the curve back shifted %
     \pgfpathcurveto%
     {\pgfpoint@onthreedcoil{0.445}{ 1    }{14}}%
     {\pgfpoint@onthreedcoil{0    }{ 0.555}{12.75}}%
     {\pgfpoint@onthreedcoil{0    }{ 0    }{11.5}}%
     \pgfpathcurveto%
     {\pgfpoint@onthreedcoil{0    }{-0.555}{10.75}}%
     {\pgfpoint@onthreedcoil{0.445}{-1    }{10}}%
     {\pgfpoint@onthreedcoil{1    }{-1    }{9}}%
     \pgfusepath{stroke,fill} %
    \fi%
    \pgfpathmoveto{\pgfpoint@onthreedcoil{1    }{ 1    }{15}}%
    \ifcoil@closed %TD@coilfirst%
    \else%
     \pgfpathcurveto%
     {\pgfpoint@onthreedcoil{1.555}{ 1    }{16}}%
     {\pgfpoint@onthreedcoil{2    }{ 0.555}{17}}%
     {\pgfpoint@onthreedcoil{2    }{ 0    }{18}}%
    \fi%
    \pgfusepath{stroke} %
    %\pgfcoordinate{TD@coilast}{\pgfpoint@onthreedcoil{2    }{ 0    }{18}} %
  }%
  \state{final}%
  {%
    \pgfpathmoveto{\pgfpointdecoratedpathlast}%
	\pgfutil@namelet{\string\color@pgfstrokecolor}{pgf@strokecolor@global}%
    %\tikzset{restore stroke color/.expand once=\pgfsavedstrokecolor}%
  }%
}%
% cone shading
% based on https://tex.stackexchange.com/a/333409/238301
\newcounter{tikz@td@cone@shading}
% x and y run from -25 to 25, alpha is an angle
\tikzset{3d/cone/shading/.cd,x/.initial=0,y/.initial=0,alpha/.initial=0,
brightness/.initial=0.5,
create shading/.code={%
\stepcounter{tikz@td@cone@shading}%
\tikzset{3d/cone/shading/.cd,#1}%
\pgfdeclarefunctionalshading{simple cone \number\value{tikz@td@cone@shading}}{\pgfpoint{-25bp}{-25bp}}{\pgfpoint{25bp}{25bp}}{}{
    % x y
	\pgfkeysvalueof{/tikz/3d/cone/shading/y} -1 mul add % shift y by the offset
	exch % swap x and y
	\pgfkeysvalueof{/tikz/3d/cone/shading/x} -1 mul add % shift x by the offset
	exch % swap y and x (reverse above swap)
    atan   % theta
	\pgfkeysvalueof{/tikz/3d/cone/shading/alpha} add % 
    sin         % cos(theta)
	1 add       % 1 + sin(theta)
    \pgfkeysvalueof{/tikz/3d/cone/shading/brightness} mul     % brightness*(1 + sin(theta))
    dup mul     % [f*(1 + sin(theta))]^2
	2 mul
	dup dup		% important so that it gets three color components
}}}
\tikzset{3d/cone shading/.style={3d/cone/shading/create shading={#1},
 shading=simple cone \number\value{tikz@td@cone@shading}}}
\makeatother
\endinput

